Multiple testing with persistent homology

In this paper we propose a computationally efficient multiple hypothesis testing procedure for persistent homology. The computational efficiency of our procedure is based on the observation that one can empirically simulate a null distribution that is universal across many hypothesis testing applications involving persistence homology. Our observation suggests that one can simulate the null distribution efficiently based on a small number of summaries of the collected data and use this null in the same way that p-value tables were used in classical statistics. To illustrate the efficiency and utility of the null distribution we provide procedures for rejecting acyclicity with both control of the Family-Wise Error Rate (FWER) and the False Discovery Rate (FDR). We will argue that the empirical null we propose is very general conditional on a few summaries of the data based on simulations and limit theorems for persistent homology for point processes.

==> arXiv submission multiple hypothesis/long-table.tex <==
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1,0.1)}} & ell.L1 & 0.07/0.17/0.22  & 0.18/0.38/0.43  & 0.00/0.05/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.12/0.25/0.27  & 0.00/0.32/0.48  & 0.00/0.05/0.08 \\ 
 & ell.L2.1 & 0.00/0.02/0.10  & 0.00/0.00/0.07  & 0.00/0.05/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.13  & 0.05/0.25/0.42  & 0.00/0.03/0.05 \\ 
 & ell.Linf.1 & 0.00/0.03/0.10  & 0.00/0.00/0.08  & 0.05/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.17/0.22  & 1.00/1.00/1.00  & 0.00/0.03/0.08 \\ 
 & L1.0 & 0.02/0.05/0.17  & 1.00/1.00/1.00  & 0.00/0.08/0.15 \\ 
 & L1.1 & 0.07/0.17/0.22  & 0.18/0.38/0.43  & 0.00/0.05/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.12/0.23/0.28  & 1.00/1.00/1.00  & 0.00/0.00/0.05 \\ 
 & L2.0 & 0.02/0.03/0.12  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.12/0.25/0.27  & 0.00/0.32/0.48  & 0.00/0.05/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.05  & 0.27/0.50/0.68  & 0.00/0.02/0.05 \\ 
 & Linf.0 & 0.00/0.03/0.12  & 0.28/0.57/0.68  & 0.00/0.00/0.08 \\ 
 & Linf.1 & 0.00/0.02/0.13  & 0.05/0.25/0.42  & 0.00/0.03/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.07/0.17/0.22  & 0.18/0.38/0.43  & 0.00/0.05/0.12 \\ 
 & pi.L1.1 & 0.07/0.18/0.30  & 0.02/0.15/0.28  & 0.05/0.15/0.25 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.12/0.25/0.27  & 0.00/0.32/0.48  & 0.00/0.05/0.08 \\ 
 & pi.L2.1 & 0.10/0.15/0.25  & 0.00/0.10/0.27  & 0.05/0.17/0.25 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.13  & 0.05/0.25/0.42  & 0.00/0.03/0.05 \\ 
 & pi.Linf.1 & 0.00/0.05/0.15  & 0.00/0.02/0.08  & 0.00/0.05/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1,1)}} & ell.L1 & 0.00/0.05/0.15  & 0.10/0.17/0.30  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.07/0.18  & 0.05/0.22/0.35  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.02/0.03 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.02/0.07  & 0.95/0.97/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.03  & 0.95/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.05/0.15  & 0.10/0.17/0.30  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.10  & 0.92/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.02/0.05  & 0.95/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.07/0.18  & 0.05/0.22/0.35  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.15/0.15  & 0.02/0.12/0.18  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.05/0.17/0.20  & 0.02/0.13/0.22  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.05/0.15  & 0.10/0.17/0.30  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.10  & 0.00/0.00/0.03  & 0.00/0.00/0.03 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.07/0.18  & 0.05/0.22/0.35  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.02/0.10  & 0.00/0.00/0.03  & 0.00/0.00/0.03 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.13  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.05/0.08  & 0.05/0.05/0.05  & 0.05/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.03/0.05  & 0.00/0.02/0.03  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.02/0.07  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.82/0.97/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.05/0.13  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.07  & 0.33/0.38/0.55  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.05/0.08/0.10  & 0.40/0.40/0.58  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.07/0.13  & 0.00/0.07/0.12  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.05/0.05/0.12  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.02/0.03/0.05  & 0.00/0.02/0.03  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.13  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.03/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.07  & 0.00/0.03/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.03/0.05  & 0.00/0.02/0.03  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.02/0.05/0.05  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1)}} & ell.L1 & 0.00/0.03/0.12  & 0.05/0.10/0.18  & 0.05/0.07/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.05/0.08  & 0.10/0.17/0.18  & 0.00/0.13/0.15 \\ 
 & ell.L2.1 & 0.00/0.00/0.12  & 0.00/0.02/0.12  & 0.10/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.03/0.10 \\ 
 & ell.Linf.1 & 0.05/0.08/0.15  & 0.00/0.02/0.13  & 0.10/0.12/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.03/0.05  & 0.40/0.70/0.82  & 0.05/0.10/0.22 \\ 
 & L1.0 & 0.00/0.00/0.12  & 0.70/0.83/0.90  & 0.05/0.17/0.28 \\ 
 & L1.1 & 0.00/0.03/0.12  & 0.05/0.10/0.18  & 0.05/0.07/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.07/0.10  & 0.45/0.83/0.88  & 0.00/0.10/0.23 \\ 
 & L2.0 & 0.00/0.05/0.08  & 0.85/0.85/0.87  & 0.02/0.10/0.15 \\ 
 & L2.1 & 0.00/0.05/0.08  & 0.10/0.17/0.18  & 0.00/0.13/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.05/0.08  & 0.05/0.10/0.13  & 0.03/0.05/0.07 \\ 
 & Linf.0 & 0.05/0.05/0.10  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & Linf.1 & 0.00/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.03/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.12  & 0.05/0.10/0.18  & 0.05/0.07/0.12 \\ 
 & pi.L1.1 & 0.00/0.03/0.08  & 0.00/0.05/0.08  & 0.00/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.05/0.08  & 0.10/0.17/0.18  & 0.00/0.13/0.15 \\ 
 & pi.L2.1 & 0.00/0.03/0.08  & 0.00/0.07/0.10  & 0.00/0.02/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.03/0.10 \\ 
 & pi.Linf.1 & 0.00/0.00/0.10  & 0.00/0.03/0.07  & 0.00/0.00/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,1,1)}} & ell.L1 & 0.00/0.03/0.15  & 0.05/0.15/0.23  & 0.00/0.00/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.13  & 0.07/0.12/0.15  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.08/0.12  & 0.00/0.03/0.17  & 0.07/0.17/0.20 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.02  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.03/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.07/0.12  & 0.97/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L1.0 & 0.05/0.08/0.17  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.03/0.15  & 0.05/0.15/0.23  & 0.00/0.00/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.05/0.15  & 0.97/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.07/0.15/0.18  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.02/0.13  & 0.07/0.12/0.15  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.08/0.10  & 0.05/0.27/0.35  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.02/0.12/0.15  & 0.03/0.25/0.38  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.02  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.15  & 0.05/0.15/0.23  & 0.00/0.00/0.05 \\ 
 & pi.L1.1 & 0.00/0.03/0.08  & 0.05/0.07/0.12  & 0.05/0.12/0.23 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.13  & 0.07/0.12/0.15  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.02/0.13  & 0.05/0.08/0.13  & 0.05/0.18/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.02  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.00  & 0.00/0.02/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,1,10)}} & ell.L1 & 0.00/0.00/0.02  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.02  & 0.02/0.10/0.15  & 0.02/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.02  & 0.00/0.00/0.07  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.12/0.15  & 0.03/0.15/0.25  & 0.02/0.05/0.05 \\ 
 & ell.Linf.1 & 0.00/0.03/0.05  & 0.02/0.05/0.05  & 0.00/0.02/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.78/1.00/1.00  & 0.00/0.03/0.05 \\ 
 & L1.0 & 0.00/0.00/0.08  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.05/0.07  & 0.65/0.92/0.98  & 0.02/0.05/0.05 \\ 
 & L2.0 & 0.00/0.07/0.12  & 0.80/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.02  & 0.02/0.10/0.15  & 0.02/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.12/0.27  & 0.02/0.10/0.30  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.02/0.15/0.28  & 0.02/0.08/0.20  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.12/0.15  & 0.03/0.15/0.25  & 0.02/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.02  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.20/0.30/0.37 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.02  & 0.02/0.10/0.15  & 0.02/0.05/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.20/0.30/0.37 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.12/0.15  & 0.03/0.15/0.25  & 0.02/0.05/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.03/0.08  & 0.05/0.10/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,1)}} & ell.L1 & 0.00/0.02/0.10  & 0.05/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.12  & 0.05/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & ell.L2.1 & 0.00/0.03/0.17  & 0.02/0.05/0.12  & 0.00/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.02/0.02/0.05  & 0.05/0.05/0.08 \\ 
 & ell.Linf.1 & 0.00/0.05/0.10  & 0.00/0.05/0.08  & 0.00/0.07/0.15 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.07/0.13  & 0.27/0.62/0.83  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.02/0.10/0.17  & 0.50/0.85/0.88  & 0.05/0.05/0.05 \\ 
 & L1.1 & 0.00/0.02/0.10  & 0.05/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.07/0.13/0.18  & 0.18/0.45/0.57  & 0.05/0.05/0.05 \\ 
 & L2.0 & 0.10/0.15/0.15  & 0.33/0.58/0.65  & 0.05/0.05/0.05 \\ 
 & L2.1 & 0.00/0.02/0.12  & 0.05/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.10/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & Linf.0 & 0.05/0.10/0.10  & 0.10/0.10/0.10  & 0.00/0.10/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.02/0.02/0.05  & 0.05/0.05/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.10  & 0.05/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & pi.L1.1 & 0.00/0.03/0.13  & 0.05/0.05/0.05  & 0.00/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.12  & 0.05/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & pi.L2.1 & 0.00/0.03/0.13  & 0.05/0.05/0.07  & 0.00/0.07/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.02/0.02/0.05  & 0.05/0.05/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.03  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,10,10)}} & ell.L1 & 0.10/0.10/0.13  & 0.17/0.30/0.38  & 0.05/0.07/0.20 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.15/0.15/0.18  & 0.12/0.20/0.33  & 0.07/0.15/0.18 \\ 
 & ell.L2.1 & 0.05/0.05/0.07  & 0.05/0.08/0.12  & 0.05/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.08/0.10  & 0.05/0.12/0.20  & 0.00/0.00/0.08 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.05/0.05/0.05  & 0.02/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.15/0.23/0.25  & 0.93/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.10/0.17/0.20  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.10/0.13  & 0.17/0.30/0.38  & 0.05/0.07/0.20 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.17/0.25/0.25  & 0.87/0.97/0.98  & 0.00/0.10/0.15 \\ 
 & L2.0 & 0.10/0.17/0.23  & 0.95/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.15/0.15/0.18  & 0.12/0.20/0.33  & 0.07/0.15/0.18 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.07/0.17/0.20  & 0.17/0.25/0.43  & 0.00/0.03/0.12 \\ 
 & Linf.0 & 0.15/0.15/0.20  & 0.13/0.25/0.42  & 0.02/0.07/0.12 \\ 
 & Linf.1 & 0.02/0.08/0.10  & 0.05/0.12/0.20  & 0.00/0.00/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.10/0.13  & 0.17/0.30/0.38  & 0.05/0.07/0.20 \\ 
 & pi.L1.1 & 0.10/0.10/0.15  & 0.05/0.08/0.17  & 0.12/0.23/0.45 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.15/0.15/0.18  & 0.12/0.20/0.33  & 0.07/0.15/0.18 \\ 
 & pi.L2.1 & 0.10/0.10/0.12  & 0.05/0.10/0.15  & 0.12/0.23/0.42 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.08/0.10  & 0.05/0.12/0.20  & 0.00/0.00/0.08 \\ 
 & pi.Linf.1 & 0.02/0.10/0.10  & 0.05/0.05/0.12  & 0.05/0.10/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,10)}} & ell.L1 & 0.02/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.02/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.02/0.02/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.02/0.05  & 0.00/0.02/0.05  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.03/0.05  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.05/0.07  & 0.55/0.65/0.77  & 0.00/0.00/0.02 \\ 
 & L1.0 & 0.00/0.02/0.03  & 0.52/0.68/0.80  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.02/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.02/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.07/0.07/0.15  & 0.10/0.17/0.25  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.05/0.05/0.10  & 0.05/0.15/0.20  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.02/0.02/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.13/0.22  & 0.00/0.12/0.18  & 0.00/0.02/0.10 \\ 
 & Linf.0 & 0.05/0.13/0.18  & 0.00/0.12/0.18  & 0.00/0.03/0.10 \\ 
 & Linf.1 & 0.00/0.03/0.05  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.02/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.02/0.05 \\ 
 & pi.L1.1 & 0.00/0.03/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.02/0.02/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.03/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.03/0.05  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,1,1)}} & ell.L1 & 0.02/0.07/0.10  & 0.05/0.22/0.32  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.02/0.07/0.12  & 0.15/0.27/0.38  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.05/0.05/0.05  & 0.00/0.05/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.10/0.12  & 0.10/0.25/0.45  & 0.00/0.05/0.05 \\ 
 & ell.Linf.1 & 0.05/0.05/0.12  & 0.05/0.12/0.15  & 0.05/0.08/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.05/0.07  & 1.00/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L1.0 & 0.00/0.03/0.07  & 1.00/1.00/1.00  & 0.02/0.05/0.05 \\ 
 & L1.1 & 0.02/0.07/0.10  & 0.05/0.22/0.32  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.05/0.08  & 1.00/1.00/1.00  & 0.00/0.00/0.02 \\ 
 & L2.0 & 0.00/0.00/0.02  & 1.00/1.00/1.00  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.02/0.07/0.12  & 0.15/0.27/0.38  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.07/0.13  & 0.23/0.45/0.57  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.05/0.08/0.15  & 0.22/0.40/0.53  & 0.00/0.05/0.05 \\ 
 & Linf.1 & 0.00/0.10/0.12  & 0.10/0.25/0.45  & 0.00/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.02/0.07/0.10  & 0.05/0.22/0.32  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.02/0.05/0.10  & 0.05/0.05/0.05  & 0.00/0.05/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.02/0.07/0.12  & 0.15/0.27/0.38  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.02/0.05/0.12  & 0.05/0.05/0.05  & 0.00/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.10/0.12  & 0.10/0.25/0.45  & 0.00/0.05/0.05 \\ 
 & pi.Linf.1 & 0.05/0.05/0.08  & 0.00/0.10/0.20  & 0.05/0.05/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,1,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.08/0.18  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.00/0.00/0.03  & 0.00/0.00/0.02 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.10/0.15  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.03  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.93/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.05  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.05  & 0.78/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.03/0.07  & 0.85/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.08/0.18  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.10/0.20  & 0.05/0.08/0.22  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.08/0.15  & 0.05/0.10/0.17  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.02/0.10/0.15  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.08/0.18  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.10/0.15  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.02/0.05  & 0.00/0.00/0.03  & 0.00/0.00/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,1)}} & ell.L1 & 0.00/0.00/0.02  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.08/0.12  & 0.00/0.05/0.10  & 0.02/0.08/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.13  & 0.00/0.00/0.08 \\ 
 & ell.Linf.1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 0.62/0.77/0.90  & 0.00/0.08/0.13 \\ 
 & L1.0 & 0.00/0.05/0.10  & 0.70/0.88/0.92  & 0.05/0.12/0.32 \\ 
 & L1.1 & 0.00/0.00/0.02  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.48/0.72/0.83  & 0.00/0.03/0.12 \\ 
 & L2.0 & 0.00/0.02/0.05  & 0.70/0.85/0.88  & 0.05/0.17/0.20 \\ 
 & L2.1 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.08/0.13/0.15  & 0.20/0.22/0.35  & 0.07/0.20/0.22 \\ 
 & Linf.0 & 0.10/0.13/0.18  & 0.22/0.33/0.43  & 0.07/0.23/0.25 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.00/0.05/0.13  & 0.00/0.00/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.02  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.13  & 0.00/0.00/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,10,10)}} & ell.L1 & 0.05/0.05/0.05  & 0.05/0.08/0.13  & 0.05/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.05/0.15/0.20  & 0.05/0.05/0.05 \\ 
 & ell.L2.1 & 0.02/0.05/0.12  & 0.05/0.05/0.07  & 0.05/0.08/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.10/0.10  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & ell.Linf.1 & 0.00/0.00/0.05  & 0.05/0.05/0.08  & 0.00/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.07  & 1.00/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.02/0.08  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.05/0.08/0.13  & 0.05/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.08  & 0.95/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L2.0 & 0.00/0.02/0.10  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.05/0.15/0.20  & 0.05/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.05/0.10  & 0.17/0.20/0.27  & 0.00/0.02/0.05 \\ 
 & Linf.0 & 0.00/0.02/0.12  & 0.13/0.18/0.32  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.02/0.10/0.10  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.05/0.08/0.13  & 0.05/0.05/0.05 \\ 
 & pi.L1.1 & 0.02/0.02/0.07  & 0.00/0.05/0.07  & 0.10/0.17/0.20 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.05/0.15/0.20  & 0.05/0.05/0.05 \\ 
 & pi.L2.1 & 0.02/0.02/0.07  & 0.00/0.02/0.08  & 0.10/0.15/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.10/0.10  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & pi.Linf.1 & 0.05/0.05/0.08  & 0.00/0.00/0.07  & 0.05/0.08/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,10)}} & ell.L1 & 0.00/0.02/0.08  & 0.00/0.08/0.20  & 0.02/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.05/0.08  & 0.00/0.13/0.17  & 0.00/0.02/0.12 \\ 
 & ell.L2.1 & 0.05/0.15/0.20  & 0.00/0.13/0.20  & 0.10/0.13/0.25 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & ell.Linf.1 & 0.17/0.20/0.25  & 0.00/0.05/0.17  & 0.17/0.20/0.22 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.05  & 0.38/0.55/0.72  & 0.02/0.08/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.55/0.72/0.88  & 0.05/0.08/0.10 \\ 
 & L1.1 & 0.00/0.02/0.08  & 0.00/0.08/0.20  & 0.02/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.03/0.07  & 0.18/0.50/0.62  & 0.00/0.02/0.05 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.37/0.60/0.77  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.00/0.05/0.08  & 0.00/0.13/0.17  & 0.00/0.02/0.12 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.07/0.13  & 0.08/0.12/0.17  & 0.00/0.03/0.08 \\ 
 & Linf.0 & 0.00/0.02/0.10  & 0.00/0.02/0.12  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.05/0.05/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.08  & 0.00/0.08/0.20  & 0.02/0.05/0.07 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.07/0.15  & 0.05/0.10/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.05/0.08  & 0.00/0.13/0.17  & 0.00/0.02/0.12 \\ 
 & pi.L2.1 & 0.00/0.02/0.07  & 0.00/0.03/0.18  & 0.05/0.10/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & pi.Linf.1 & 0.05/0.05/0.07  & 0.00/0.03/0.12  & 0.02/0.05/0.08 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(10,10,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.17/0.32  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.05  & 0.07/0.23/0.40  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.12/0.17  & 0.05/0.08/0.17  & 0.07/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.03/0.18  & 0.12/0.30/0.48  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.05/0.10/0.13  & 0.05/0.08/0.13  & 0.05/0.10/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.05/0.05  & 0.97/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.05/0.07/0.10  & 1.00/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.17/0.32  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.07  & 0.98/1.00/1.00  & 0.02/0.03/0.05 \\ 
 & L2.0 & 0.00/0.02/0.05  & 1.00/1.00/1.00  & 0.02/0.05/0.05 \\ 
 & L2.1 & 0.00/0.02/0.05  & 0.07/0.23/0.40  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.08/0.12  & 0.12/0.48/0.65  & 0.02/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.05/0.07  & 0.22/0.38/0.57  & 0.05/0.05/0.05 \\ 
 & Linf.1 & 0.00/0.03/0.18  & 0.12/0.30/0.48  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.17/0.32  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.07  & 0.00/0.03/0.05  & 0.00/0.07/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.05  & 0.07/0.23/0.40  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.03/0.08  & 0.00/0.03/0.05  & 0.00/0.05/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.03/0.18  & 0.12/0.30/0.48  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.00/0.02/0.07  & 0.00/0.08/0.10  & 0.00/0.05/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(10,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.08/0.18  & 0.00/0.08/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.12  & 0.07/0.17/0.25  & 0.02/0.13/0.25 \\ 
 & ell.L2.1 & 0.05/0.08/0.15  & 0.05/0.13/0.20  & 0.12/0.15/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.07/0.20/0.33  & 0.13/0.25/0.35  & 0.07/0.20/0.30 \\ 
 & ell.Linf.1 & 0.07/0.15/0.15  & 0.05/0.12/0.22  & 0.00/0.08/0.18 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.30/0.53/0.73  & 0.00/0.08/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.55/0.77/0.87  & 0.05/0.05/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.08/0.18  & 0.00/0.08/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.38/0.62/0.78  & 0.00/0.12/0.17 \\ 
 & L2.0 & 0.00/0.00/0.07  & 0.70/0.78/0.83  & 0.05/0.05/0.18 \\ 
 & L2.1 & 0.00/0.03/0.12  & 0.07/0.17/0.25  & 0.02/0.13/0.25 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.18/0.30  & 0.10/0.22/0.38  & 0.03/0.12/0.27 \\ 
 & Linf.0 & 0.02/0.10/0.20  & 0.07/0.17/0.28  & 0.00/0.03/0.08 \\ 
 & Linf.1 & 0.07/0.20/0.33  & 0.13/0.25/0.35  & 0.07/0.20/0.30 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.08/0.18  & 0.00/0.08/0.10 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.03/0.15  & 0.02/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.12  & 0.07/0.17/0.25  & 0.02/0.13/0.25 \\ 
 & pi.L2.1 & 0.00/0.05/0.07  & 0.00/0.10/0.18  & 0.07/0.10/0.25 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.07/0.20/0.33  & 0.13/0.25/0.35  & 0.07/0.20/0.30 \\ 
 & pi.Linf.1 & 0.08/0.25/0.28  & 0.08/0.17/0.20  & 0.10/0.20/0.32 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(2)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.12/0.20  & 0.00/0.00/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.02/0.15  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.07/0.12  & 0.00/0.03/0.10  & 0.02/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.03  & 0.07/0.15/0.20  & 0.00/0.02/0.10 \\ 
 & ell.Linf.1 & 0.00/0.00/0.03  & 0.05/0.05/0.05  & 0.00/0.00/0.07 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.67/0.93/1.00  & 0.05/0.05/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.90/1.00/1.00  & 0.05/0.10/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.12/0.20  & 0.00/0.00/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.72/0.88/0.95  & 0.00/0.03/0.08 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.90/0.92/0.95  & 0.00/0.03/0.07 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.02/0.15  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.03/0.17/0.25  & 0.00/0.00/0.03 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.05/0.10/0.18  & 0.00/0.00/0.07 \\ 
 & Linf.1 & 0.00/0.00/0.03  & 0.07/0.15/0.20  & 0.00/0.02/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.12/0.20  & 0.00/0.00/0.05 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.05/0.08  & 0.00/0.07/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.02/0.15  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.10  & 0.00/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.03  & 0.07/0.15/0.20  & 0.00/0.02/0.10 \\ 
 & pi.Linf.1 & 0.03/0.13/0.18  & 0.00/0.18/0.20  & 0.05/0.08/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(3)}} & ell.L1 & 0.05/0.05/0.05  & 0.20/0.40/0.48  & 0.00/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.10  & 0.25/0.43/0.55  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.10  & 0.00/0.05/0.10  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.07/0.12  & 0.10/0.32/0.52  & 0.05/0.10/0.10 \\ 
 & ell.Linf.1 & 0.00/0.00/0.07  & 0.00/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.97/1.00/1.00  & 0.00/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.20/0.40/0.48  & 0.00/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.05  & 0.98/1.00/1.00  & 0.00/0.05/0.05 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.10  & 0.25/0.43/0.55  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.08  & 0.27/0.42/0.55  & 0.02/0.05/0.08 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.23/0.38/0.40  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.00/0.07/0.12  & 0.10/0.32/0.52  & 0.05/0.10/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.20/0.40/0.48  & 0.00/0.05/0.05 \\ 
 & pi.L1.1 & 0.05/0.05/0.12  & 0.00/0.10/0.12  & 0.05/0.10/0.17 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.10  & 0.25/0.43/0.55  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.05/0.07/0.18  & 0.00/0.10/0.22  & 0.05/0.05/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.07/0.12  & 0.10/0.32/0.52  & 0.05/0.10/0.10 \\ 
 & pi.Linf.1 & 0.00/0.13/0.23  & 0.05/0.10/0.18  & 0.05/0.12/0.18 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(4)}} & ell.L1 & 0.00/0.00/0.00  & 0.45/0.63/0.83  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.52/0.72/0.88  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.03/0.10/0.12  & 0.05/0.10/0.17  & 0.05/0.10/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.33/0.65/0.78  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.08  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.45/0.63/0.83  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.52/0.72/0.88  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.50/0.80/0.87  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.43/0.75/0.85  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.33/0.65/0.78  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.45/0.63/0.83  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.15  & 0.00/0.00/0.02  & 0.00/0.00/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.52/0.72/0.88  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.00/0.02  & 0.00/0.00/0.03 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.33/0.65/0.78  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.05  & 0.00/0.03/0.12  & 0.00/0.00/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(5)}} & ell.L1 & 0.00/0.02/0.05  & 0.75/0.90/0.98  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.07  & 0.80/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.13  & 0.00/0.02/0.10  & 0.00/0.02/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.05  & 0.57/0.83/0.97  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.07  & 0.00/0.03/0.05  & 0.00/0.02/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.75/0.90/0.98  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.07  & 0.80/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.02  & 0.85/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.92/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.02/0.05  & 0.57/0.83/0.97  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.75/0.90/0.98  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.10/0.13/0.18  & 0.05/0.13/0.17  & 0.02/0.10/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.07  & 0.80/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.10/0.13/0.17  & 0.05/0.15/0.17  & 0.02/0.10/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.05  & 0.57/0.83/0.97  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.08/0.13  & 0.00/0.03/0.10  & 0.02/0.05/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1,0.1)}} & ell.L1 & 0.00/0.00/0.00  & 0.10/0.25/0.35  & 0.00/0.03/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.20/0.27/0.38  & 0.00/0.00/0.02 \\ 
 & ell.L2.1 & 0.02/0.10/0.20  & 0.05/0.07/0.13  & 0.05/0.07/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.07/0.22/0.35  & 0.00/0.00/0.05 \\ 
 & ell.Linf.1 & 0.05/0.12/0.20  & 0.10/0.10/0.18  & 0.00/0.10/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.95/0.97/0.98  & 0.00/0.00/0.02 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/0.97/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.10/0.25/0.35  & 0.00/0.03/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.02 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.20/0.27/0.38  & 0.00/0.00/0.02 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.25/0.45/0.70  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.28/0.52/0.65  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.07/0.22/0.35  & 0.00/0.00/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.10/0.25/0.35  & 0.00/0.03/0.05 \\ 
 & pi.L1.1 & 0.00/0.08/0.13  & 0.00/0.05/0.08  & 0.00/0.03/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.20/0.27/0.38  & 0.00/0.00/0.02 \\ 
 & pi.L2.1 & 0.00/0.07/0.13  & 0.00/0.05/0.08  & 0.00/0.03/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.07/0.22/0.35  & 0.00/0.00/0.05 \\ 
 & pi.Linf.1 & 0.05/0.13/0.15  & 0.03/0.10/0.18  & 0.05/0.08/0.17 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.23/0.38  & 0.00/0.02/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.10/0.28/0.45  & 0.00/0.02/0.08 \\ 
 & ell.L2.1 & 0.00/0.02/0.05  & 0.00/0.02/0.02  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.05/0.05  & 0.10/0.12/0.28  & 0.00/0.02/0.10 \\ 
 & ell.Linf.1 & 0.02/0.05/0.05  & 0.00/0.00/0.05  & 0.00/0.02/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.92/1.00/1.00  & 0.00/0.05/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.05/0.08 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.23/0.38  & 0.00/0.02/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.03/0.05  & 0.77/0.98/1.00  & 0.00/0.02/0.02 \\ 
 & L2.0 & 0.05/0.05/0.05  & 0.90/0.98/1.00  & 0.00/0.02/0.07 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.10/0.28/0.45  & 0.00/0.02/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.32/0.52/0.65  & 0.22/0.33/0.40  & 0.00/0.02/0.20 \\ 
 & Linf.0 & 0.40/0.60/0.60  & 0.17/0.23/0.37  & 0.00/0.17/0.25 \\ 
 & Linf.1 & 0.00/0.05/0.05  & 0.10/0.12/0.28  & 0.00/0.02/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.23/0.38  & 0.00/0.02/0.08 \\ 
 & pi.L1.1 & 0.10/0.12/0.17  & 0.05/0.10/0.18  & 0.05/0.05/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.10/0.28/0.45  & 0.00/0.02/0.08 \\ 
 & pi.L2.1 & 0.10/0.12/0.15  & 0.05/0.10/0.18  & 0.05/0.05/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.05/0.05  & 0.10/0.12/0.28  & 0.00/0.02/0.10 \\ 
 & pi.Linf.1 & 0.08/0.08/0.12  & 0.05/0.08/0.15  & 0.07/0.08/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1,10)}} & ell.L1 & 0.05/0.05/0.05  & 0.12/0.22/0.23  & 0.10/0.15/0.18 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.12/0.18/0.22  & 0.10/0.15/0.18 \\ 
 & ell.L2.1 & 0.05/0.05/0.05  & 0.00/0.02/0.05  & 0.02/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.75/0.75/0.75  & 0.95/0.97/1.00  & 0.55/0.65/0.70 \\ 
 & L1.0 & 0.75/0.75/0.75  & 0.95/0.97/1.00  & 0.62/0.65/0.70 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.12/0.22/0.23  & 0.10/0.15/0.18 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 0.67/0.85/0.93  & 0.38/0.63/0.75 \\ 
 & L2.0 & 1.00/1.00/1.00  & 0.65/0.83/0.97  & 0.42/0.67/0.78 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.12/0.18/0.22  & 0.10/0.15/0.18 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.65/0.80/0.80  & 0.27/0.47/0.55  & 0.12/0.30/0.45 \\ 
 & Linf.0 & 0.65/0.80/0.80  & 0.32/0.50/0.57  & 0.12/0.33/0.45 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.12/0.22/0.23  & 0.10/0.15/0.18 \\ 
 & pi.L1.1 & 0.07/0.22/0.25  & 0.05/0.07/0.17  & 0.00/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.12/0.18/0.22  & 0.10/0.15/0.18 \\ 
 & pi.L2.1 & 0.07/0.18/0.23  & 0.05/0.07/0.13  & 0.00/0.07/0.17 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1)}} & ell.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.03/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.05  & 0.05/0.17/0.22  & 0.00/0.00/0.05 \\ 
 & ell.L2.1 & 0.07/0.08/0.15  & 0.05/0.08/0.13  & 0.05/0.10/0.18 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.05/0.05  & 0.00/0.02/0.08  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.03/0.05  & 0.00/0.05/0.08  & 0.00/0.00/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.33/0.73/0.80  & 0.00/0.12/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.68/0.80/0.90  & 0.10/0.12/0.17 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.03/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.05  & 0.52/0.80/0.87  & 0.00/0.05/0.10 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.82/0.87/0.95  & 0.05/0.12/0.13 \\ 
 & L2.1 & 0.00/0.03/0.05  & 0.05/0.17/0.22  & 0.00/0.00/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.02  & 0.00/0.05/0.15  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.00/0.17/0.27  & 0.00/0.03/0.07 \\ 
 & Linf.1 & 0.00/0.05/0.05  & 0.00/0.02/0.08  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.03/0.07 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.05  & 0.05/0.17/0.22  & 0.00/0.00/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.02 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.05/0.05  & 0.00/0.02/0.08  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.12  & 0.00/0.00/0.07  & 0.00/0.00/0.03 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.13/0.28/0.38  & 0.00/0.03/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.03  & 0.12/0.17/0.30  & 0.00/0.00/0.10 \\ 
 & ell.L2.1 & 0.00/0.05/0.18  & 0.05/0.17/0.27  & 0.05/0.07/0.25 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.15/0.23/0.32  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.08/0.10/0.13  & 0.00/0.15/0.22  & 0.02/0.05/0.18 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.90/0.97/0.98  & 0.00/0.02/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.13/0.28/0.38  & 0.00/0.03/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.90/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.95/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.03  & 0.12/0.17/0.30  & 0.00/0.00/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.02  & 0.15/0.28/0.37  & 0.02/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.03/0.05  & 0.12/0.22/0.37  & 0.02/0.05/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.15/0.23/0.32  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.13/0.28/0.38  & 0.00/0.03/0.12 \\ 
 & pi.L1.1 & 0.10/0.15/0.15  & 0.02/0.05/0.18  & 0.00/0.10/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.03  & 0.12/0.17/0.30  & 0.00/0.00/0.10 \\ 
 & pi.L2.1 & 0.10/0.13/0.15  & 0.00/0.07/0.13  & 0.00/0.05/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.15/0.23/0.32  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.03/0.15  & 0.00/0.00/0.07 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,1,10)}} & ell.L1 & 0.05/0.05/0.05  & 0.07/0.12/0.25  & 0.05/0.10/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & ell.L2.1 & 0.02/0.12/0.18  & 0.10/0.12/0.15  & 0.07/0.13/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.07  & 0.05/0.07/0.10  & 0.05/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.95/1.00/1.00  & 0.15/0.20/0.22 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.10/0.17/0.23 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.07/0.12/0.25  & 0.05/0.10/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.15/0.18/0.23  & 0.80/0.88/0.97  & 0.22/0.30/0.40 \\ 
 & L2.0 & 0.15/0.18/0.23  & 0.80/0.92/1.00  & 0.17/0.35/0.40 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.45/0.45/0.45  & 0.17/0.27/0.43  & 0.03/0.18/0.25 \\ 
 & Linf.0 & 0.45/0.45/0.45  & 0.18/0.30/0.52  & 0.05/0.23/0.27 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.07/0.12/0.25  & 0.05/0.10/0.12 \\ 
 & pi.L1.1 & 0.05/0.08/0.10  & 0.05/0.08/0.10  & 0.05/0.05/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & pi.L2.1 & 0.05/0.08/0.10  & 0.05/0.08/0.10  & 0.05/0.05/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.03/0.05  & 0.05/0.05/0.07  & 0.00/0.03/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,1)}} & ell.L1 & 0.00/0.02/0.05  & 0.00/0.10/0.17  & 0.02/0.07/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.03  & 0.00/0.02/0.12  & 0.00/0.00/0.08 \\ 
 & ell.L2.1 & 0.05/0.07/0.10  & 0.00/0.07/0.10  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.05  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.37/0.62/0.73  & 0.02/0.10/0.18 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.70/0.72/0.80  & 0.05/0.12/0.22 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.00/0.10/0.17  & 0.02/0.07/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.03/0.22/0.50  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.20/0.52/0.82  & 0.00/0.00/0.05 \\ 
 & L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.12  & 0.00/0.00/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.20/0.25/0.25  & 0.05/0.12/0.12  & 0.00/0.02/0.10 \\ 
 & Linf.0 & 0.22/0.25/0.25  & 0.05/0.12/0.13  & 0.00/0.03/0.13 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.00/0.10/0.17  & 0.02/0.07/0.12 \\ 
 & pi.L1.1 & 0.02/0.05/0.07  & 0.00/0.05/0.10  & 0.02/0.07/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.03  & 0.00/0.02/0.12  & 0.00/0.00/0.08 \\ 
 & pi.L2.1 & 0.02/0.05/0.07  & 0.00/0.05/0.10  & 0.00/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.02/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,10,10)}} & ell.L1 & 0.00/0.00/0.05  & 0.07/0.27/0.40  & 0.05/0.07/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.12/0.23/0.38  & 0.00/0.05/0.10 \\ 
 & ell.L2.1 & 0.05/0.05/0.08  & 0.02/0.07/0.17  & 0.07/0.12/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & ell.Linf.1 & 0.00/0.08/0.10  & 0.00/0.00/0.05  & 0.00/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.80/0.95/0.98  & 0.10/0.15/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.05/0.10/0.15 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.07/0.27/0.40  & 0.05/0.07/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.85/1.00/1.00  & 0.12/0.22/0.27 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.15/0.23/0.33 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.12/0.23/0.38  & 0.00/0.05/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.08/0.10/0.10  & 0.20/0.42/0.47  & 0.05/0.12/0.12 \\ 
 & Linf.0 & 0.10/0.10/0.12  & 0.25/0.42/0.53  & 0.05/0.12/0.18 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.07/0.27/0.40  & 0.05/0.07/0.13 \\ 
 & pi.L1.1 & 0.00/0.05/0.10  & 0.02/0.05/0.10  & 0.05/0.07/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.12/0.23/0.38  & 0.00/0.05/0.10 \\ 
 & pi.L2.1 & 0.00/0.03/0.08  & 0.02/0.05/0.08  & 0.02/0.07/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.03 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,10)}} & ell.L1 & 0.05/0.08/0.10  & 0.05/0.05/0.10  & 0.00/0.13/0.20 \\ 
 & ell.L1.1 & 0.00/0.03/0.03  & 0.00/0.00/0.00  & 0.00/0.02/0.05 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.08/0.10  & 0.05/0.05/0.07  & 0.00/0.10/0.13 \\ 
 & ell.L2.1 & 0.02/0.05/0.08  & 0.00/0.05/0.05  & 0.00/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.97/1.00/1.00  & 0.80/0.80/0.82  & 0.68/0.80/0.80 \\ 
 & L1.0 & 1.00/1.00/1.00  & 0.80/0.85/0.88  & 0.77/0.80/0.80 \\ 
 & L1.1 & 0.05/0.08/0.10  & 0.05/0.05/0.10  & 0.00/0.13/0.20 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.83/0.97/1.00  & 0.55/0.68/0.78  & 0.35/0.55/0.78 \\ 
 & L2.0 & 0.83/0.97/1.00  & 0.55/0.72/0.82  & 0.37/0.62/0.85 \\ 
 & L2.1 & 0.05/0.08/0.10  & 0.05/0.05/0.07  & 0.00/0.10/0.13 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.55/0.60/0.63  & 0.17/0.37/0.45  & 0.15/0.25/0.38 \\ 
 & Linf.0 & 0.55/0.60/0.63  & 0.17/0.38/0.48  & 0.15/0.28/0.45 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.08/0.10  & 0.05/0.05/0.10  & 0.00/0.13/0.20 \\ 
 & pi.L1.1 & 0.10/0.13/0.17  & 0.05/0.05/0.10  & 0.05/0.15/0.17 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.08/0.10  & 0.05/0.05/0.07  & 0.00/0.10/0.13 \\ 
 & pi.L2.1 & 0.10/0.13/0.17  & 0.05/0.05/0.10  & 0.05/0.15/0.17 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.00/0.02/0.03  & 0.00/0.02/0.02  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.07/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.08  & 0.00/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.12/0.18/0.28  & 0.00/0.00/0.03 \\ 
 & ell.Linf.1 & 0.00/0.00/0.02  & 0.05/0.05/0.07  & 0.03/0.05/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.02/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.07/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.32/0.45/0.55  & 0.00/0.02/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.32/0.50/0.60  & 0.00/0.03/0.07 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.12/0.18/0.28  & 0.00/0.00/0.03 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.07/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.12/0.18/0.28  & 0.00/0.00/0.03 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.07  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,1,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.20  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.13/0.25  & 0.05/0.18/0.23  & 0.07/0.10/0.27 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.08/0.15  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.05/0.10/0.10  & 0.00/0.00/0.03  & 0.00/0.02/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.87/0.95/1.00  & 0.00/0.00/0.02 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.87/1.00/1.00  & 0.00/0.02/0.17 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.10/0.20  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.40/0.52/0.62  & 0.20/0.43/0.58  & 0.00/0.03/0.07 \\ 
 & Linf.0 & 0.40/0.55/0.63  & 0.20/0.47/0.63  & 0.00/0.03/0.13 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.08/0.15  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.02/0.05/0.05  & 0.00/0.00/0.05  & 0.00/0.03/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.20  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.02/0.05/0.05  & 0.00/0.00/0.05  & 0.00/0.02/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.08/0.15  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.00/0.02/0.05  & 0.00/0.02/0.05  & 0.00/0.00/0.03 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.07/0.13  & 0.00/0.05/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.17  & 0.00/0.05/0.10 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.13/0.15  & 0.00/0.02/0.08 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.45/0.65/0.77  & 0.05/0.15/0.17 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.67/0.73/0.85  & 0.05/0.13/0.22 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.07/0.13  & 0.00/0.05/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.58/0.87/0.97  & 0.00/0.07/0.12 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/0.95/0.98  & 0.00/0.07/0.25 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.05/0.13/0.17  & 0.00/0.05/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.05/0.22/0.40  & 0.00/0.05/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.05/0.18/0.33  & 0.00/0.12/0.15 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.13/0.15  & 0.00/0.02/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.07/0.13  & 0.00/0.05/0.08 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.02/0.08  & 0.00/0.03/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.17  & 0.00/0.05/0.10 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.05/0.12  & 0.00/0.05/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.13/0.15  & 0.00/0.02/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.07  & 0.00/0.02/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,10,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.25/0.35  & 0.05/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.10/0.23/0.33  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.02/0.05/0.10  & 0.00/0.03/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.05/0.10/0.17  & 0.05/0.05/0.05 \\ 
 & ell.Linf.1 & 0.02/0.05/0.07  & 0.05/0.05/0.05  & 0.05/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.03/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.25/0.35  & 0.05/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.93/0.97/1.00  & 0.00/0.08/0.10 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.00/0.05/0.05 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.10/0.23/0.33  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.08/0.12  & 0.23/0.33/0.43  & 0.05/0.15/0.20 \\ 
 & Linf.0 & 0.02/0.13/0.18  & 0.30/0.45/0.52  & 0.07/0.12/0.25 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.05/0.10/0.17  & 0.05/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.25/0.35  & 0.05/0.05/0.05 \\ 
 & pi.L1.1 & 0.02/0.08/0.15  & 0.00/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.10/0.23/0.33  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.02/0.10/0.15  & 0.00/0.10/0.13  & 0.05/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.05/0.10/0.17  & 0.05/0.05/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.07  & 0.00/0.02/0.10  & 0.00/0.05/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,10)}} & ell.L1 & 0.00/0.03/0.05  & 0.00/0.02/0.15  & 0.00/0.00/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.05  & 0.00/0.03/0.15  & 0.00/0.05/0.15 \\ 
 & ell.L2.1 & 0.05/0.20/0.27  & 0.12/0.18/0.20  & 0.08/0.15/0.27 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.00/0.02/0.10  & 0.03/0.08/0.13 \\ 
 & ell.Linf.1 & 0.02/0.08/0.10  & 0.02/0.03/0.05  & 0.10/0.10/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.43/0.73/0.75  & 0.05/0.07/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.70/0.75/0.77  & 0.05/0.10/0.18 \\ 
 & L1.1 & 0.00/0.03/0.05  & 0.00/0.02/0.15  & 0.00/0.00/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.07/0.08  & 0.13/0.38/0.58  & 0.02/0.03/0.10 \\ 
 & L2.0 & 0.05/0.05/0.05  & 0.18/0.53/0.73  & 0.02/0.05/0.17 \\ 
 & L2.1 & 0.00/0.03/0.05  & 0.00/0.03/0.15  & 0.00/0.05/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.20/0.27/0.35  & 0.07/0.18/0.28  & 0.03/0.10/0.20 \\ 
 & Linf.0 & 0.20/0.30/0.35  & 0.07/0.22/0.28  & 0.00/0.05/0.17 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.00/0.02/0.10  & 0.03/0.08/0.13 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.05  & 0.00/0.02/0.15  & 0.00/0.00/0.08 \\ 
 & pi.L1.1 & 0.08/0.10/0.13  & 0.00/0.00/0.12  & 0.00/0.08/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.05  & 0.00/0.03/0.15  & 0.00/0.05/0.15 \\ 
 & pi.L2.1 & 0.05/0.07/0.12  & 0.00/0.02/0.07  & 0.00/0.07/0.18 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.00/0.02/0.10  & 0.03/0.08/0.13 \\ 
 & pi.Linf.1 & 0.00/0.07/0.10  & 0.05/0.07/0.10  & 0.10/0.10/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(10,10,10)}} & ell.L1 & 0.00/0.00/0.03  & 0.15/0.27/0.33  & 0.00/0.00/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.17/0.27/0.37  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.03/0.10/0.10  & 0.00/0.07/0.10  & 0.00/0.08/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.10/0.17/0.32  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.00/0.05/0.05  & 0.00/0.03/0.05  & 0.00/0.05/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.03  & 0.15/0.27/0.33  & 0.00/0.00/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.17/0.27/0.37  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.12/0.37/0.57  & 0.00/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.15/0.43/0.58  & 0.00/0.05/0.07 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.10/0.17/0.32  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.03  & 0.15/0.27/0.33  & 0.00/0.00/0.07 \\ 
 & pi.L1.1 & 0.00/0.08/0.10  & 0.00/0.02/0.05  & 0.00/0.05/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.17/0.27/0.37  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.05/0.10  & 0.00/0.02/0.07  & 0.00/0.05/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.10/0.17/0.32  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.02/0.05/0.13  & 0.00/0.08/0.13  & 0.00/0.05/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(10,10)}} & ell.L1 & 0.00/0.00/0.03  & 0.05/0.08/0.12  & 0.00/0.02/0.03 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.03  & 0.05/0.08/0.10  & 0.00/0.03/0.08 \\ 
 & ell.L2.1 & 0.05/0.05/0.07  & 0.05/0.05/0.07  & 0.05/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.05/0.12/0.15  & 0.00/0.07/0.08 \\ 
 & ell.Linf.1 & 0.02/0.10/0.10  & 0.10/0.10/0.10  & 0.05/0.07/0.15 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.37/0.67/0.77  & 0.00/0.02/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.58/0.80/0.87  & 0.00/0.05/0.20 \\ 
 & L1.1 & 0.00/0.00/0.03  & 0.05/0.08/0.12  & 0.00/0.02/0.03 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.40/0.68/0.78  & 0.03/0.10/0.17 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.63/0.80/0.88  & 0.10/0.10/0.13 \\ 
 & L2.1 & 0.00/0.02/0.03  & 0.05/0.08/0.10  & 0.00/0.03/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.08/0.17/0.25  & 0.00/0.08/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.03/0.15/0.27  & 0.02/0.08/0.17 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.05/0.12/0.15  & 0.00/0.07/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.03  & 0.05/0.08/0.12  & 0.00/0.02/0.03 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.05/0.07/0.12  & 0.00/0.02/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.03  & 0.05/0.08/0.10  & 0.00/0.03/0.08 \\ 
 & pi.L2.1 & 0.00/0.03/0.07  & 0.05/0.07/0.10  & 0.05/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.05/0.12/0.15  & 0.00/0.07/0.08 \\ 
 & pi.Linf.1 & 0.00/0.05/0.10  & 0.00/0.07/0.12  & 0.05/0.05/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(10,5,25)}} & ell.L1 & 0.00/0.02/0.05  & 0.67/0.90/0.97  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.05/0.05  & 0.67/0.88/1.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.02/0.05/0.05  & 0.02/0.05/0.07  & 0.00/0.00/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.48/0.80/0.85  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.08/0.17  & 0.00/0.02/0.05  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.67/0.90/0.97  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.02/0.02  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.05/0.05  & 0.67/0.88/1.00  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.02  & 0.88/0.93/0.97  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.02/0.05  & 0.85/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.48/0.80/0.85  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.67/0.90/0.97  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.07/0.13  & 0.05/0.10/0.10  & 0.00/0.07/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.05/0.05  & 0.67/0.88/1.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.12/0.15  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.48/0.80/0.85  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.07/0.13  & 0.00/0.12/0.15  & 0.00/0.07/0.17 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(3,3,75)}} & ell.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.38  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.27/0.48  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.02  & 0.00/0.05/0.05  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.07/0.10  & 0.10/0.23/0.32  & 0.07/0.10/0.10 \\ 
 & ell.Linf.1 & 0.02/0.05/0.10  & 0.02/0.05/0.07  & 0.02/0.10/0.12 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.02/0.17/0.38  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.27/0.48  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.05/0.08  & 0.35/0.57/0.60  & 0.03/0.07/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.28/0.52/0.70  & 0.00/0.02/0.07 \\ 
 & Linf.1 & 0.00/0.07/0.10  & 0.10/0.23/0.32  & 0.07/0.10/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.38  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.27/0.48  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.07/0.10  & 0.10/0.23/0.32  & 0.07/0.10/0.10 \\ 
 & pi.Linf.1 & 0.00/0.02/0.17  & 0.05/0.10/0.12  & 0.07/0.13/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(4,4,25)}} & ell.L1 & 0.05/0.05/0.05  & 0.63/0.77/0.87  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.57/0.83/0.87  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.05/0.12  & 0.00/0.05/0.13  & 0.00/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.02  & 0.35/0.45/0.53  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.02/0.03/0.08  & 0.00/0.02/0.07  & 0.00/0.00/0.07 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.03/0.05/0.05  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.63/0.77/0.87  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.02/0.05/0.05  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.57/0.83/0.87  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.77/0.88/0.95  & 0.00/0.00/0.02 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.78/0.90/0.95  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.02  & 0.35/0.45/0.53  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.63/0.77/0.87  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.07/0.10/0.12  & 0.05/0.07/0.12  & 0.02/0.05/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.57/0.83/0.87  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.05/0.10/0.15  & 0.05/0.10/0.12  & 0.02/0.05/0.08 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.02  & 0.35/0.45/0.53  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.00/0.15/0.23  & 0.00/0.03/0.13  & 0.00/0.10/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(5,2,25)}} & ell.L1 & 0.05/0.05/0.07  & 0.10/0.17/0.18  & 0.05/0.10/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.10  & 0.10/0.13/0.17  & 0.10/0.12/0.20 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.00/0.03/0.07  & 0.05/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.13  & 0.10/0.12/0.13  & 0.05/0.05/0.10 \\ 
 & ell.Linf.1 & 0.05/0.05/0.07  & 0.00/0.05/0.12  & 0.02/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.52/0.85/0.90  & 0.05/0.07/0.12 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.77/0.90/0.92  & 0.00/0.02/0.08 \\ 
 & L1.1 & 0.05/0.05/0.07  & 0.10/0.17/0.18  & 0.05/0.10/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.07  & 0.78/0.88/0.98  & 0.05/0.10/0.13 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/0.92/0.98  & 0.00/0.02/0.07 \\ 
 & L2.1 & 0.05/0.05/0.10  & 0.10/0.13/0.17  & 0.10/0.12/0.20 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.05/0.05  & 0.10/0.17/0.28  & 0.00/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.05  & 0.05/0.20/0.37  & 0.00/0.00/0.08 \\ 
 & Linf.1 & 0.05/0.05/0.13  & 0.10/0.12/0.13  & 0.05/0.05/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.07  & 0.10/0.17/0.18  & 0.05/0.10/0.13 \\ 
 & pi.L1.1 & 0.05/0.05/0.12  & 0.02/0.05/0.12  & 0.00/0.07/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.10  & 0.10/0.13/0.17  & 0.10/0.12/0.20 \\ 
 & pi.L2.1 & 0.05/0.05/0.12  & 0.02/0.07/0.10  & 0.07/0.07/0.18 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.13  & 0.10/0.12/0.13  & 0.05/0.05/0.10 \\ 
 & pi.Linf.1 & 0.05/0.10/0.10  & 0.02/0.05/0.10  & 0.00/0.07/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(6,4,25)}} & ell.L1 & 0.00/0.00/0.00  & 0.35/0.52/0.67  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.40/0.53/0.67  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.03/0.05  & 0.00/0.05/0.17  & 0.00/0.02/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.10/0.30/0.43  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.07  & 0.00/0.02/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.35/0.52/0.67  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.40/0.53/0.67  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.62/0.72/0.83  & 0.00/0.00/0.02 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.65/0.82/0.93  & 0.00/0.02/0.05 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.10/0.30/0.43  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.35/0.52/0.67  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.05/0.05/0.05  & 0.05/0.05/0.05  & 0.05/0.05/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.40/0.53/0.67  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.05/0.05/0.05  & 0.05/0.05/0.05  & 0.05/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.10/0.30/0.43  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.07  & 0.00/0.05/0.07  & 0.00/0.02/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(8,3,100)}} & ell.L1 & 0.00/0.02/0.05  & 0.20/0.40/0.55  & 0.05/0.05/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.17/0.35/0.50  & 0.05/0.07/0.10 \\ 
 & ell.L2.1 & 0.00/0.00/0.07  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.03  & 0.13/0.25/0.38  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.00/0.05/0.13  & 0.00/0.00/0.00  & 0.00/0.00/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 0.97/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.20/0.40/0.55  & 0.05/0.05/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.02/0.05/0.05  & 1.00/1.00/1.00  & 0.05/0.05/0.08 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.17/0.35/0.50  & 0.05/0.07/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.23/0.47/0.63  & 0.00/0.00/0.02 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.28/0.45/0.63  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.00/0.02/0.03  & 0.13/0.25/0.38  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.20/0.40/0.55  & 0.05/0.05/0.10 \\ 
 & pi.L1.1 & 0.10/0.12/0.15  & 0.10/0.13/0.18  & 0.10/0.15/0.17 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.17/0.35/0.50  & 0.05/0.07/0.10 \\ 
 & pi.L2.1 & 0.10/0.15/0.15  & 0.10/0.12/0.17  & 0.10/0.15/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.03  & 0.13/0.25/0.38  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.05/0.05/0.10  & 0.00/0.03/0.08  & 0.05/0.10/0.12 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(1,2,100)}} & ell.L1 & 0.00/0.00/0.05  & 0.03/0.10/0.23  & 0.02/0.08/0.15 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.07/0.13 \\ 
 & ell.L2.1 & 0.00/0.02/0.05  & 0.00/0.10/0.13  & 0.00/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & ell.Linf.1 & 0.00/0.05/0.10  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.63/0.90/1.00  & 0.02/0.05/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.85/0.98/1.00  & 0.00/0.00/0.12 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.03/0.10/0.23  & 0.02/0.08/0.15 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.53/0.93/1.00  & 0.00/0.05/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/1.00/1.00  & 0.05/0.15/0.22 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.07/0.13 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.07  & 0.07/0.13/0.23  & 0.00/0.10/0.12 \\ 
 & Linf.0 & 0.00/0.07/0.12  & 0.10/0.20/0.38  & 0.10/0.10/0.15 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.03/0.10/0.23  & 0.02/0.08/0.15 \\ 
 & pi.L1.1 & 0.05/0.05/0.05  & 0.00/0.05/0.10  & 0.00/0.05/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.07/0.13 \\ 
 & pi.L2.1 & 0.05/0.05/0.05  & 0.00/0.08/0.10  & 0.00/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & pi.Linf.1 & 0.00/0.05/0.10  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(10,4,75)}} & ell.L1 & 0.00/0.00/0.00  & 0.30/0.42/0.55  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.27/0.48/0.63  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.02/0.07/0.23  & 0.00/0.00/0.15  & 0.00/0.02/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.10/0.23/0.47  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.05/0.07/0.13  & 0.05/0.07/0.10  & 0.05/0.10/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.30/0.42/0.55  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.27/0.48/0.63  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.47/0.77/0.90  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.50/0.83/0.90  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.10/0.23/0.47  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.30/0.42/0.55  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.12  & 0.03/0.13/0.15  & 0.03/0.10/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.27/0.48/0.63  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.07/0.13  & 0.02/0.13/0.15  & 0.03/0.12/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.10/0.23/0.47  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.02/0.05  & 0.00/0.02/0.12  & 0.00/0.10/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(2,2,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.08  & 0.00/0.05/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.08 \\ 
 & ell.L2.1 & 0.00/0.05/0.13  & 0.00/0.07/0.22  & 0.00/0.05/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.02  & 0.03/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & ell.Linf.1 & 0.00/0.03/0.10  & 0.00/0.07/0.10  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.32/0.65/0.92  & 0.00/0.12/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.63/0.93/0.95  & 0.05/0.10/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.07/0.08  & 0.00/0.05/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.38/0.85/0.88  & 0.00/0.03/0.08 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.82/0.90/0.95  & 0.05/0.10/0.15 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.02/0.12/0.22  & 0.05/0.07/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.05  & 0.05/0.15/0.32  & 0.07/0.10/0.12 \\ 
 & Linf.1 & 0.00/0.00/0.02  & 0.03/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.08  & 0.00/0.05/0.10 \\ 
 & pi.L1.1 & 0.02/0.05/0.15  & 0.00/0.05/0.13  & 0.05/0.05/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.08 \\ 
 & pi.L2.1 & 0.02/0.07/0.12  & 0.00/0.05/0.10  & 0.05/0.07/0.08 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.02  & 0.03/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & pi.Linf.1 & 0.00/0.05/0.05  & 0.02/0.05/0.10  & 0.00/0.03/0.08 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(3,3,75)}} & ell.L1 & 0.00/0.00/0.00  & 0.15/0.27/0.32  & 0.00/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.12/0.27/0.32  & 0.00/0.02/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.13  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.02/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.15/0.27/0.32  & 0.00/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.12/0.27/0.32  & 0.00/0.02/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.22/0.38/0.50  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.27/0.45/0.57  & 0.00/0.05/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.02/0.13  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.15/0.27/0.32  & 0.00/0.05/0.05 \\ 
 & pi.L1.1 & 0.00/0.10/0.15  & 0.00/0.07/0.12  & 0.00/0.13/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.12/0.27/0.32  & 0.00/0.02/0.05 \\ 
 & pi.L2.1 & 0.00/0.07/0.15  & 0.05/0.05/0.10  & 0.02/0.08/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.13  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(4,3,25)}} & ell.L1 & 0.02/0.07/0.12  & 0.25/0.28/0.42  & 0.00/0.07/0.15 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.08/0.13  & 0.25/0.28/0.40  & 0.05/0.10/0.10 \\ 
 & ell.L2.1 & 0.05/0.08/0.15  & 0.05/0.07/0.08  & 0.05/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.10/0.12  & 0.18/0.25/0.32  & 0.10/0.15/0.15 \\ 
 & ell.Linf.1 & 0.02/0.03/0.05  & 0.00/0.05/0.05  & 0.00/0.03/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.05/0.07  & 1.00/1.00/1.00  & 0.00/0.03/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.02/0.07/0.12  & 0.25/0.28/0.42  & 0.00/0.07/0.15 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.08/0.10  & 1.00/1.00/1.00  & 0.05/0.08/0.10 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.08/0.13  & 0.25/0.28/0.40  & 0.05/0.10/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.08/0.08  & 0.37/0.45/0.53  & 0.05/0.12/0.15 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.22/0.33/0.53  & 0.00/0.00/0.03 \\ 
 & Linf.1 & 0.05/0.10/0.12  & 0.18/0.25/0.32  & 0.10/0.15/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.02/0.07/0.12  & 0.25/0.28/0.42  & 0.00/0.07/0.15 \\ 
 & pi.L1.1 & 0.17/0.20/0.20  & 0.10/0.17/0.23  & 0.12/0.20/0.30 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.08/0.13  & 0.25/0.28/0.40  & 0.05/0.10/0.10 \\ 
 & pi.L2.1 & 0.17/0.20/0.22  & 0.10/0.17/0.23  & 0.12/0.20/0.30 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.10/0.12  & 0.18/0.25/0.32  & 0.10/0.15/0.15 \\ 
 & pi.Linf.1 & 0.10/0.13/0.15  & 0.10/0.12/0.15  & 0.05/0.12/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(5,2,75)}} & ell.L1 & 0.00/0.05/0.10  & 0.12/0.22/0.33  & 0.05/0.08/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.13  & 0.20/0.22/0.28  & 0.05/0.08/0.17 \\ 
 & ell.L2.1 & 0.00/0.05/0.08  & 0.00/0.05/0.07  & 0.00/0.05/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.07/0.12/0.13  & 0.07/0.10/0.15  & 0.02/0.05/0.17 \\ 
 & ell.Linf.1 & 0.00/0.05/0.23  & 0.05/0.07/0.15  & 0.00/0.08/0.12 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.02/0.07  & 0.70/0.95/0.98  & 0.08/0.18/0.22 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.90/0.98/1.00  & 0.05/0.12/0.17 \\ 
 & L1.1 & 0.00/0.05/0.10  & 0.12/0.22/0.33  & 0.05/0.08/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.07  & 0.87/0.95/0.95  & 0.05/0.10/0.20 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.92/0.95/0.98  & 0.05/0.12/0.20 \\ 
 & L2.1 & 0.00/0.03/0.13  & 0.20/0.22/0.28  & 0.05/0.08/0.17 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.12/0.18  & 0.15/0.22/0.22  & 0.05/0.05/0.17 \\ 
 & Linf.0 & 0.00/0.07/0.10  & 0.10/0.13/0.32  & 0.05/0.07/0.13 \\ 
 & Linf.1 & 0.07/0.12/0.13  & 0.07/0.10/0.15  & 0.02/0.05/0.17 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.05/0.10  & 0.12/0.22/0.33  & 0.05/0.08/0.13 \\ 
 & pi.L1.1 & 0.00/0.13/0.22  & 0.10/0.15/0.23  & 0.05/0.07/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.13  & 0.20/0.22/0.28  & 0.05/0.08/0.17 \\ 
 & pi.L2.1 & 0.05/0.12/0.27  & 0.12/0.18/0.25  & 0.05/0.08/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.07/0.12/0.13  & 0.07/0.10/0.15  & 0.02/0.05/0.17 \\ 
 & pi.Linf.1 & 0.10/0.13/0.18  & 0.05/0.05/0.12  & 0.05/0.12/0.17 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(6,2,100)}} & ell.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.05  & 0.00/0.08/0.12  & 0.00/0.00/0.05 \\ 
 & ell.L2.1 & 0.00/0.07/0.10  & 0.00/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.05/0.05  & 0.05/0.08/0.12  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.55/0.87/0.92  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.85/0.95/0.95  & 0.00/0.00/0.13 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.02  & 0.48/0.83/0.92  & 0.00/0.02/0.03 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.72/0.90/1.00  & 0.00/0.02/0.17 \\ 
 & L2.1 & 0.00/0.00/0.05  & 0.00/0.08/0.12  & 0.00/0.00/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.03/0.05  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.02/0.05 \\ 
 & Linf.1 & 0.02/0.05/0.05  & 0.05/0.08/0.12  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.02/0.05  & 0.00/0.00/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.05  & 0.00/0.08/0.12  & 0.00/0.00/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.00/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.05/0.05  & 0.05/0.08/0.12  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.00/0.02/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(8,3,50)}} & ell.L1 & 0.00/0.00/0.00  & 0.25/0.38/0.57  & 0.00/0.00/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.25/0.47/0.52  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.10/0.10  & 0.08/0.15/0.18  & 0.05/0.07/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.07  & 0.10/0.17/0.23  & 0.00/0.03/0.05 \\ 
 & ell.Linf.1 & 0.05/0.05/0.05  & 0.05/0.05/0.05  & 0.00/0.03/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.98/1.00/1.00  & 0.00/0.02/0.03 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.02/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.25/0.38/0.57  & 0.00/0.00/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.25/0.47/0.52  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.33/0.43/0.68  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.25/0.53/0.75  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.07  & 0.10/0.17/0.23  & 0.00/0.03/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.25/0.38/0.57  & 0.00/0.00/0.05 \\ 
 & pi.L1.1 & 0.00/0.10/0.25  & 0.05/0.10/0.25  & 0.07/0.17/0.22 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.25/0.47/0.52  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.05/0.10/0.23  & 0.00/0.07/0.18  & 0.02/0.17/0.18 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.07  & 0.10/0.17/0.23  & 0.00/0.03/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.08  & 0.00/0.02/0.10  & 0.00/0.05/0.07 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(9,2,10)}} & ell.L1 & 0.00/0.05/0.05  & 0.07/0.13/0.22  & 0.02/0.02/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.07/0.23  & 0.00/0.00/0.12 \\ 
 & ell.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.07  & 0.00/0.02/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.05/0.08/0.17  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.03  & 0.00/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.05  & 0.50/0.77/0.88  & 0.07/0.07/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.77/0.90/1.00  & 0.05/0.12/0.15 \\ 
 & L1.1 & 0.00/0.05/0.05  & 0.07/0.13/0.22  & 0.02/0.02/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.47/0.85/0.95  & 0.03/0.05/0.12 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.90/0.93/0.95  & 0.05/0.15/0.20 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.07/0.23  & 0.00/0.00/0.12 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.05/0.15/0.17  & 0.00/0.02/0.07 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.10/0.15/0.25  & 0.00/0.02/0.12 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.05/0.08/0.17  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.05/0.05  & 0.07/0.13/0.22  & 0.02/0.02/0.08 \\ 
 & pi.L1.1 & 0.00/0.07/0.07  & 0.00/0.02/0.10  & 0.00/0.02/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.07/0.23  & 0.00/0.00/0.12 \\ 
 & pi.L2.1 & 0.00/0.02/0.10  & 0.00/0.03/0.10  & 0.00/0.03/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.05/0.08/0.17  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.00/0.05/0.05  & 0.00/0.05/0.12  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.simplex(unit,2)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.03/0.18  & 0.02/0.03/0.10 \\ 
 & ell.L2.1 & 0.00/0.05/0.13  & 0.07/0.10/0.18  & 0.05/0.13/0.23 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.03/0.07 \\ 
 & ell.Linf.1 & 0.07/0.10/0.13  & 0.05/0.10/0.10  & 0.00/0.08/0.15 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.32/0.63/0.80  & 0.00/0.07/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.62/0.82/0.88  & 0.00/0.10/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.48/0.72/0.80  & 0.05/0.08/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.70/0.80/0.92  & 0.05/0.08/0.23 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.03/0.18  & 0.02/0.03/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.05  & 0.07/0.20/0.43  & 0.00/0.05/0.10 \\ 
 & Linf.0 & 0.00/0.05/0.07  & 0.10/0.25/0.43  & 0.00/0.07/0.13 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.03/0.07 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.05/0.05 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.03/0.05  & 0.02/0.05/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.03/0.18  & 0.02/0.03/0.10 \\ 
 & pi.L2.1 & 0.00/0.00/0.02  & 0.00/0.03/0.05  & 0.02/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.03/0.07 \\ 
 & pi.Linf.1 & 0.00/0.03/0.03  & 0.00/0.02/0.05  & 0.00/0.03/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.simplex(unit,3)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.18/0.30  & 0.00/0.03/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.30  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.03/0.07  & 0.00/0.05/0.08  & 0.05/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.07/0.08/0.10  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.03/0.05  & 0.05/0.05/0.08  & 0.02/0.07/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.90/0.98/1.00  & 0.03/0.07/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.05/0.10/0.15 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.18/0.30  & 0.00/0.03/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.02 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.02/0.07 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.05/0.13/0.30  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.15/0.20/0.25  & 0.05/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.12/0.22/0.32  & 0.05/0.05/0.05 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.07/0.08/0.10  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.18/0.30  & 0.00/0.03/0.05 \\ 
 & pi.L1.1 & 0.05/0.05/0.05  & 0.05/0.05/0.10  & 0.02/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.30  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.02/0.03/0.05  & 0.05/0.05/0.05  & 0.02/0.05/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.07/0.08/0.10  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.simplex(unit,4)}} & ell.L1 & 0.00/0.00/0.00  & 0.27/0.40/0.55  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.25/0.35/0.58  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.03/0.05  & 0.00/0.00/0.08  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.05/0.05/0.18  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.05/0.08  & 0.00/0.00/0.05  & 0.02/0.07/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.27/0.40/0.55  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.25/0.35/0.58  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.37/0.47/0.60  & 0.05/0.05/0.07 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.37/0.53/0.70  & 0.05/0.07/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.05/0.05/0.18  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.27/0.40/0.55  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.07  & 0.00/0.03/0.17  & 0.00/0.07/0.22 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.25/0.35/0.58  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.17  & 0.00/0.10/0.23 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.05/0.05/0.18  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.05/0.07  & 0.00/0.02/0.05  & 0.00/0.02/0.07 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(1.25).mvn.0.01}} & ell.L1 & 0.62/0.65/0.67  & 0.60/0.73/0.75  & 0.57/0.68/0.72 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.05  & 0.00/0.10/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.90/0.95/0.95  & 1.00/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & ell.Linf.1 & 0.48/0.50/0.58  & 0.45/0.52/0.60  & 0.42/0.47/0.58 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.60/0.62/0.65  & 0.60/0.70/0.73  & 0.57/0.68/0.68 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.17/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.62/0.65/0.67  & 0.60/0.73/0.75  & 0.57/0.68/0.72 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.17/0.22  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.90/0.95/0.95  & 0.97/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & Linf.0 & 0.05/0.05/0.05  & 0.05/0.10/0.22  & 0.05/0.07/0.08 \\ 
 & Linf.1 & 0.90/0.95/0.95  & 1.00/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.62/0.65/0.67  & 0.60/0.73/0.75  & 0.57/0.68/0.72 \\ 
 & pi.L1.1 & 0.70/0.87/0.90  & 0.62/0.88/0.95  & 0.63/0.88/0.97 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & pi.L2.1 & 0.85/0.88/0.93  & 0.87/0.95/0.95  & 0.82/0.93/0.98 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.90/0.95/0.95  & 1.00/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & pi.Linf.1 & 0.80/0.88/0.93  & 0.90/0.90/0.95  & 0.85/0.90/0.90 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(1.25).mvn.0.05}} & ell.L1 & 0.22/0.32/0.38  & 0.32/0.45/0.57  & 0.30/0.32/0.40 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.53/0.62/0.82  & 0.85/0.93/0.95  & 0.80/0.85/0.88 \\ 
 & ell.L2.1 & 0.10/0.12/0.20  & 0.02/0.12/0.15  & 0.05/0.13/0.18 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.65/0.73/0.83  & 0.85/0.85/0.85  & 0.70/0.90/0.92 \\ 
 & ell.Linf.1 & 0.43/0.45/0.50  & 0.40/0.45/0.52  & 0.45/0.48/0.52 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.22/0.32/0.33  & 0.33/0.43/0.58  & 0.30/0.30/0.33 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.25/0.33/0.45  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.22/0.32/0.38  & 0.32/0.45/0.57  & 0.30/0.32/0.40 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.52/0.60/0.68  & 0.85/0.95/0.97  & 0.80/0.83/0.83 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.30/0.45  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.53/0.62/0.82  & 0.85/0.93/0.95  & 0.80/0.85/0.88 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.60/0.68/0.77  & 0.80/0.83/0.85  & 0.70/0.78/0.90 \\ 
 & Linf.0 & 0.15/0.18/0.20  & 0.20/0.25/0.33  & 0.20/0.20/0.30 \\ 
 & Linf.1 & 0.65/0.73/0.83  & 0.85/0.85/0.85  & 0.70/0.90/0.92 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.22/0.32/0.38  & 0.32/0.45/0.57  & 0.30/0.32/0.40 \\ 
 & pi.L1.1 & 0.22/0.35/0.40  & 0.27/0.38/0.47  & 0.30/0.33/0.38 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.53/0.62/0.82  & 0.85/0.93/0.95  & 0.80/0.85/0.88 \\ 
 & pi.L2.1 & 0.33/0.63/0.78  & 0.45/0.68/0.77  & 0.35/0.57/0.80 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.65/0.73/0.83  & 0.85/0.85/0.85  & 0.70/0.90/0.92 \\ 
 & pi.Linf.1 & 0.68/0.77/0.80  & 0.70/0.73/0.77  & 0.65/0.75/0.85 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(1.25).mvn.0.1}} & ell.L1 & 0.05/0.10/0.15  & 0.00/0.20/0.25  & 0.10/0.12/0.18 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.13/0.23  & 0.10/0.32/0.35  & 0.10/0.18/0.27 \\ 
 & ell.L2.1 & 0.07/0.08/0.10  & 0.00/0.10/0.13  & 0.00/0.08/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.35/0.48/0.62  & 0.47/0.63/0.70  & 0.32/0.47/0.53 \\ 
 & ell.Linf.1 & 0.25/0.38/0.42  & 0.35/0.37/0.43  & 0.35/0.38/0.40 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.08/0.12  & 0.17/0.63/0.67  & 0.10/0.15/0.18 \\ 
 & L1.0 & 0.00/0.02/0.05  & 0.55/0.60/0.65  & 0.02/0.05/0.07 \\ 
 & L1.1 & 0.05/0.10/0.15  & 0.00/0.20/0.25  & 0.10/0.12/0.18 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.10/0.17  & 0.37/0.67/0.75  & 0.10/0.17/0.25 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.50/0.67/0.78  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.05/0.13/0.23  & 0.10/0.32/0.35  & 0.10/0.18/0.27 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.35/0.40/0.45  & 0.48/0.67/0.75  & 0.27/0.47/0.53 \\ 
 & Linf.0 & 0.20/0.27/0.30  & 0.35/0.35/0.38  & 0.30/0.32/0.35 \\ 
 & Linf.1 & 0.35/0.48/0.62  & 0.47/0.63/0.70  & 0.32/0.47/0.53 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.10/0.15  & 0.00/0.20/0.25  & 0.10/0.12/0.18 \\ 
 & pi.L1.1 & 0.05/0.15/0.23  & 0.00/0.17/0.20  & 0.10/0.10/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.13/0.23  & 0.10/0.32/0.35  & 0.10/0.18/0.27 \\ 
 & pi.L2.1 & 0.05/0.18/0.25  & 0.00/0.13/0.22  & 0.10/0.13/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.35/0.48/0.62  & 0.47/0.63/0.70  & 0.32/0.47/0.53 \\ 
 & pi.Linf.1 & 0.35/0.53/0.63  & 0.37/0.52/0.65  & 0.27/0.43/0.50 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(10).mvn.0.01}} & ell.L1 & 0.60/0.60/0.62  & 0.68/0.72/0.75  & 0.42/0.50/0.57 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.65/0.65/0.68  & 0.70/0.73/0.80  & 0.58/0.65/0.65 \\ 
 & ell.L2.1 & 0.38/0.70/0.80  & 0.40/0.53/0.77  & 0.47/0.65/0.72 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.60/0.63/0.67  & 0.68/0.73/0.78  & 0.55/0.60/0.65 \\ 
 & ell.Linf.1 & 0.70/0.70/0.75  & 0.70/0.70/0.77  & 0.62/0.68/0.72 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.60/0.60/0.60  & 0.67/0.75/0.80  & 0.42/0.50/0.50 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.02/0.15/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.60/0.60/0.62  & 0.68/0.72/0.75  & 0.42/0.50/0.57 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.65/0.65/0.65  & 0.88/0.95/1.00  & 0.58/0.65/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.45/0.50/0.50  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.65/0.65/0.68  & 0.70/0.73/0.80  & 0.58/0.65/0.65 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.78/0.95/0.98  & 1.00/1.00/1.00  & 0.75/0.75/0.75 \\ 
 & Linf.0 & 0.90/0.98/1.00  & 1.00/1.00/1.00  & 0.70/0.75/0.75 \\ 
 & Linf.1 & 0.60/0.63/0.67  & 0.68/0.73/0.78  & 0.55/0.60/0.65 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.60/0.60/0.62  & 0.68/0.72/0.75  & 0.42/0.50/0.57 \\ 
 & pi.L1.1 & 0.50/0.57/0.60  & 0.55/0.60/0.65  & 0.47/0.60/0.60 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.65/0.65/0.68  & 0.70/0.73/0.80  & 0.58/0.65/0.65 \\ 
 & pi.L2.1 & 0.60/0.60/0.60  & 0.60/0.65/0.67  & 0.57/0.60/0.63 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.60/0.63/0.67  & 0.68/0.73/0.78  & 0.55/0.60/0.65 \\ 
 & pi.Linf.1 & 0.52/0.58/0.60  & 0.60/0.60/0.63  & 0.55/0.58/0.63 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(10).mvn.0.05}} & ell.L1 & 0.25/0.37/0.55  & 0.35/0.47/0.53  & 0.22/0.30/0.40 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.70/0.73/0.77  & 0.75/0.80/0.87  & 0.60/0.63/0.70 \\ 
 & ell.L2.1 & 0.22/0.40/0.50  & 0.40/0.45/0.47  & 0.32/0.45/0.53 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.60/0.65/0.75  & 0.70/0.80/0.80  & 0.60/0.62/0.65 \\ 
 & ell.Linf.1 & 0.50/0.55/0.63  & 0.50/0.57/0.65  & 0.52/0.55/0.60 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.25/0.33/0.40  & 0.40/0.58/0.68  & 0.18/0.28/0.35 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.23/0.25  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.25/0.37/0.55  & 0.35/0.47/0.53  & 0.22/0.30/0.40 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.70/0.73/0.73  & 0.93/1.00/1.00  & 0.60/0.63/0.65 \\ 
 & L2.0 & 0.00/0.00/0.03  & 0.37/0.38/0.45  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.70/0.73/0.77  & 0.75/0.80/0.87  & 0.60/0.63/0.70 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.75/0.92/0.93  & 1.00/1.00/1.00  & 0.75/0.75/0.75 \\ 
 & Linf.0 & 0.85/0.95/1.00  & 1.00/1.00/1.00  & 0.75/0.75/0.75 \\ 
 & Linf.1 & 0.60/0.65/0.75  & 0.70/0.80/0.80  & 0.60/0.62/0.65 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.25/0.37/0.55  & 0.35/0.47/0.53  & 0.22/0.30/0.40 \\ 
 & pi.L1.1 & 0.15/0.20/0.37  & 0.10/0.27/0.40  & 0.12/0.23/0.30 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.70/0.73/0.77  & 0.75/0.80/0.87  & 0.60/0.63/0.70 \\ 
 & pi.L2.1 & 0.50/0.57/0.67  & 0.42/0.58/0.65  & 0.42/0.60/0.60 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.60/0.65/0.75  & 0.70/0.80/0.80  & 0.60/0.62/0.65 \\ 
 & pi.Linf.1 & 0.50/0.58/0.63  & 0.50/0.55/0.70  & 0.45/0.62/0.67 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(10).mvn.0.1}} & ell.L1 & 0.30/0.38/0.40  & 0.35/0.40/0.42  & 0.30/0.37/0.40 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.60/0.63/0.65  & 0.65/0.65/0.72  & 0.62/0.65/0.65 \\ 
 & ell.L2.1 & 0.00/0.05/0.15  & 0.05/0.10/0.12  & 0.00/0.05/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.60/0.63/0.65  & 0.65/0.65/0.67  & 0.62/0.65/0.65 \\ 
 & ell.Linf.1 & 0.40/0.50/0.50  & 0.43/0.55/0.55  & 0.50/0.53/0.55 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.30/0.37/0.38  & 0.35/0.42/0.52  & 0.30/0.37/0.37 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.05/0.12/0.18  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.30/0.38/0.40  & 0.35/0.40/0.42  & 0.30/0.37/0.40 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.60/0.67/0.70  & 0.73/0.92/0.97  & 0.62/0.65/0.65 \\ 
 & L2.0 & 0.05/0.05/0.05  & 0.37/0.45/0.50  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.60/0.63/0.65  & 0.65/0.65/0.72  & 0.62/0.65/0.65 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.83/0.85/0.87  & 1.00/1.00/1.00  & 0.75/0.75/0.80 \\ 
 & Linf.0 & 0.85/0.88/0.98  & 1.00/1.00/1.00  & 0.70/0.75/0.80 \\ 
 & Linf.1 & 0.60/0.63/0.65  & 0.65/0.65/0.67  & 0.62/0.65/0.65 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.30/0.38/0.40  & 0.35/0.40/0.42  & 0.30/0.37/0.40 \\ 
 & pi.L1.1 & 0.17/0.30/0.35  & 0.20/0.32/0.35  & 0.25/0.27/0.32 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.60/0.63/0.65  & 0.65/0.65/0.72  & 0.62/0.65/0.65 \\ 
 & pi.L2.1 & 0.50/0.58/0.62  & 0.50/0.57/0.60  & 0.50/0.58/0.62 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.60/0.63/0.65  & 0.65/0.65/0.67  & 0.62/0.65/0.65 \\ 
 & pi.Linf.1 & 0.55/0.55/0.55  & 0.52/0.58/0.60  & 0.55/0.60/0.60 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(2).mvn.0.01}} & ell.L1 & 0.20/0.20/0.30  & 0.17/0.42/0.58  & 0.20/0.25/0.33 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.50/0.55/0.67  & 0.52/0.68/0.83  & 0.45/0.52/0.67 \\ 
 & ell.L2.1 & 0.00/0.05/0.15  & 0.00/0.02/0.10  & 0.00/0.07/0.18 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.47/0.65/0.70  & 0.70/0.78/0.82  & 0.45/0.53/0.70 \\ 
 & ell.Linf.1 & 0.40/0.40/0.40  & 0.30/0.43/0.45  & 0.35/0.42/0.43 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.20/0.20/0.25  & 0.35/0.57/0.70  & 0.20/0.25/0.25 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.32/0.48/0.50  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.20/0.20/0.30  & 0.17/0.42/0.58  & 0.20/0.25/0.33 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.50/0.55/0.57  & 0.87/1.00/1.00  & 0.45/0.52/0.53 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.50/0.50/0.50  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.50/0.55/0.67  & 0.52/0.68/0.83  & 0.45/0.52/0.67 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.42/0.52/0.60  & 0.62/0.70/0.80  & 0.42/0.47/0.57 \\ 
 & Linf.0 & 0.25/0.25/0.25  & 0.27/0.33/0.57  & 0.25/0.28/0.30 \\ 
 & Linf.1 & 0.47/0.65/0.70  & 0.70/0.78/0.82  & 0.45/0.53/0.70 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.20/0.20/0.30  & 0.17/0.42/0.58  & 0.20/0.25/0.33 \\ 
 & pi.L1.1 & 0.05/0.08/0.17  & 0.07/0.10/0.12  & 0.05/0.10/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.50/0.55/0.67  & 0.52/0.68/0.83  & 0.45/0.52/0.67 \\ 
 & pi.L2.1 & 0.25/0.40/0.45  & 0.22/0.38/0.40  & 0.22/0.33/0.43 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.47/0.65/0.70  & 0.70/0.78/0.82  & 0.45/0.53/0.70 \\ 
 & pi.Linf.1 & 0.35/0.45/0.58  & 0.47/0.53/0.57  & 0.37/0.50/0.67 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(2).mvn.0.05}} & ell.L1 & 0.00/0.10/0.17  & 0.08/0.23/0.40  & 0.05/0.13/0.33 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.25/0.27/0.30  & 0.32/0.43/0.57  & 0.20/0.35/0.38 \\ 
 & ell.L2.1 & 0.00/0.07/0.13  & 0.05/0.05/0.12  & 0.05/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.30/0.30/0.33  & 0.37/0.37/0.40  & 0.25/0.32/0.38 \\ 
 & ell.Linf.1 & 0.25/0.25/0.30  & 0.22/0.28/0.30  & 0.20/0.27/0.30 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.07/0.12  & 0.32/0.62/0.72  & 0.00/0.10/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.55/0.70/0.73  & 0.00/0.00/0.05 \\ 
 & L1.1 & 0.00/0.10/0.17  & 0.08/0.23/0.40  & 0.05/0.13/0.33 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.20/0.25/0.28  & 0.52/0.88/1.00  & 0.20/0.33/0.37 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.65/0.72/0.75  & 0.00/0.00/0.02 \\ 
 & L2.1 & 0.25/0.27/0.30  & 0.32/0.43/0.57  & 0.20/0.35/0.38 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.30/0.30/0.30  & 0.32/0.32/0.40  & 0.25/0.28/0.32 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.00/0.08/0.25  & 0.00/0.10/0.22 \\ 
 & Linf.1 & 0.30/0.30/0.33  & 0.37/0.37/0.40  & 0.25/0.32/0.38 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.10/0.17  & 0.08/0.23/0.40  & 0.05/0.13/0.33 \\ 
 & pi.L1.1 & 0.00/0.17/0.25  & 0.00/0.02/0.10  & 0.00/0.15/0.27 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.25/0.27/0.30  & 0.32/0.43/0.57  & 0.20/0.35/0.38 \\ 
 & pi.L2.1 & 0.10/0.28/0.35  & 0.15/0.20/0.25  & 0.05/0.23/0.32 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.30/0.30/0.33  & 0.37/0.37/0.40  & 0.25/0.32/0.38 \\ 
 & pi.Linf.1 & 0.25/0.30/0.30  & 0.25/0.25/0.27  & 0.25/0.27/0.30 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(2).mvn.0.1}} & ell.L1 & 0.05/0.05/0.07  & 0.05/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.10  & 0.05/0.10/0.17  & 0.05/0.08/0.15 \\ 
 & ell.L2.1 & 0.00/0.10/0.13  & 0.00/0.10/0.20  & 0.05/0.07/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.07/0.22  & 0.07/0.23/0.38  & 0.08/0.23/0.33 \\ 
 & ell.Linf.1 & 0.10/0.12/0.17  & 0.10/0.10/0.15  & 0.10/0.10/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.40/0.57/0.67  & 0.05/0.10/0.10 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.62/0.65/0.70  & 0.05/0.05/0.12 \\ 
 & L1.1 & 0.05/0.05/0.07  & 0.05/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.07  & 0.57/0.77/0.90  & 0.05/0.08/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/0.95/0.95  & 0.00/0.03/0.15 \\ 
 & L2.1 & 0.05/0.05/0.10  & 0.05/0.10/0.17  & 0.05/0.08/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.08/0.18/0.33  & 0.37/0.58/0.70  & 0.18/0.40/0.47 \\ 
 & Linf.0 & 0.15/0.25/0.32  & 0.43/0.57/0.62  & 0.18/0.33/0.40 \\ 
 & Linf.1 & 0.00/0.07/0.22  & 0.07/0.23/0.38  & 0.08/0.23/0.33 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.07  & 0.05/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & pi.L1.1 & 0.05/0.05/0.10  & 0.05/0.05/0.05  & 0.00/0.03/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.10  & 0.05/0.10/0.17  & 0.05/0.08/0.15 \\ 
 & pi.L2.1 & 0.05/0.08/0.15  & 0.05/0.07/0.07  & 0.05/0.08/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.07/0.22  & 0.07/0.23/0.38  & 0.08/0.23/0.33 \\ 
 & pi.Linf.1 & 0.10/0.22/0.32  & 0.15/0.20/0.25  & 0.08/0.22/0.25 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(5).mvn.0.01}} & ell.L1 & 0.25/0.25/0.30  & 0.30/0.40/0.40  & 0.25/0.30/0.38 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.50/0.50/0.52  & 0.55/0.55/0.57  & 0.50/0.50/0.52 \\ 
 & ell.L2.1 & 0.17/0.30/0.35  & 0.25/0.25/0.33  & 0.20/0.22/0.25 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.50/0.52/0.55  & 0.55/0.55/0.55  & 0.52/0.55/0.55 \\ 
 & ell.Linf.1 & 0.47/0.53/0.60  & 0.55/0.58/0.60  & 0.43/0.52/0.58 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.25/0.25/0.27  & 0.32/0.50/0.58  & 0.25/0.30/0.32 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.15/0.18/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.25/0.25/0.30  & 0.30/0.40/0.40  & 0.25/0.30/0.38 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.50/0.50/0.50  & 0.78/0.88/0.90  & 0.50/0.50/0.50 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.40/0.40/0.40  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.50/0.50/0.52  & 0.55/0.55/0.57  & 0.50/0.50/0.52 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.75/0.78/0.82  & 0.95/1.00/1.00  & 0.68/0.73/0.75 \\ 
 & Linf.0 & 0.75/0.83/0.92  & 0.95/1.00/1.00  & 0.72/0.75/0.75 \\ 
 & Linf.1 & 0.50/0.52/0.55  & 0.55/0.55/0.55  & 0.52/0.55/0.55 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.25/0.25/0.30  & 0.30/0.40/0.40  & 0.25/0.30/0.38 \\ 
 & pi.L1.1 & 0.30/0.30/0.30  & 0.25/0.27/0.30  & 0.25/0.25/0.27 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.50/0.50/0.52  & 0.55/0.55/0.57  & 0.50/0.50/0.52 \\ 
 & pi.L2.1 & 0.45/0.45/0.45  & 0.45/0.45/0.47  & 0.37/0.45/0.45 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.50/0.52/0.55  & 0.55/0.55/0.55  & 0.52/0.55/0.55 \\ 
 & pi.Linf.1 & 0.45/0.50/0.53  & 0.48/0.52/0.55  & 0.45/0.45/0.48 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(5).mvn.0.05}} & ell.L1 & 0.10/0.15/0.23  & 0.15/0.30/0.38  & 0.10/0.20/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.55/0.62/0.65  & 0.55/0.65/0.70  & 0.60/0.60/0.65 \\ 
 & ell.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.10  & 0.00/0.02/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.53/0.60/0.67  & 0.60/0.67/0.70  & 0.50/0.57/0.63 \\ 
 & ell.Linf.1 & 0.52/0.55/0.63  & 0.50/0.50/0.55  & 0.50/0.52/0.57 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.15/0.17  & 0.20/0.40/0.52  & 0.10/0.15/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.20/0.22  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.15/0.23  & 0.15/0.30/0.38  & 0.10/0.20/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.53/0.62/0.65  & 0.73/0.90/0.95  & 0.60/0.60/0.60 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.30/0.37/0.42  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.55/0.62/0.65  & 0.55/0.65/0.70  & 0.60/0.60/0.65 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.65/0.72/0.78  & 0.77/0.90/0.93  & 0.63/0.67/0.75 \\ 
 & Linf.0 & 0.65/0.78/0.83  & 0.80/0.90/1.00  & 0.65/0.70/0.75 \\ 
 & Linf.1 & 0.53/0.60/0.67  & 0.60/0.67/0.70  & 0.50/0.57/0.63 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.15/0.23  & 0.15/0.30/0.38  & 0.10/0.20/0.25 \\ 
 & pi.L1.1 & 0.05/0.08/0.12  & 0.00/0.05/0.10  & 0.05/0.05/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.55/0.62/0.65  & 0.55/0.65/0.70  & 0.60/0.60/0.65 \\ 
 & pi.L2.1 & 0.25/0.33/0.45  & 0.22/0.40/0.53  & 0.20/0.35/0.48 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.53/0.60/0.67  & 0.60/0.67/0.70  & 0.50/0.57/0.63 \\ 
 & pi.Linf.1 & 0.35/0.50/0.58  & 0.45/0.50/0.53  & 0.37/0.48/0.53 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(5).mvn.0.1}} & ell.L1 & 0.07/0.13/0.22  & 0.25/0.25/0.33  & 0.17/0.23/0.27 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.53/0.53/0.60  & 0.55/0.58/0.63  & 0.55/0.55/0.60 \\ 
 & ell.L2.1 & 0.05/0.07/0.20  & 0.05/0.12/0.20  & 0.05/0.13/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.48/0.52/0.55  & 0.55/0.60/0.67  & 0.45/0.50/0.58 \\ 
 & ell.Linf.1 & 0.50/0.52/0.57  & 0.50/0.52/0.55  & 0.45/0.55/0.55 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.07/0.10/0.12  & 0.27/0.40/0.52  & 0.13/0.20/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.07/0.13/0.22  & 0.25/0.25/0.33  & 0.17/0.23/0.27 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.53/0.53/0.55  & 0.68/0.85/0.90  & 0.55/0.55/0.55 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.25/0.35/0.45  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.53/0.53/0.60  & 0.55/0.58/0.63  & 0.55/0.55/0.60 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.53/0.60/0.60  & 0.82/0.92/0.95  & 0.57/0.60/0.65 \\ 
 & Linf.0 & 0.55/0.58/0.67  & 0.90/0.93/0.95  & 0.60/0.65/0.77 \\ 
 & Linf.1 & 0.48/0.52/0.55  & 0.55/0.60/0.67  & 0.45/0.50/0.58 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.07/0.13/0.22  & 0.25/0.25/0.33  & 0.17/0.23/0.27 \\ 
 & pi.L1.1 & 0.00/0.08/0.10  & 0.05/0.10/0.10  & 0.02/0.10/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.53/0.53/0.60  & 0.55/0.58/0.63  & 0.55/0.55/0.60 \\ 
 & pi.L2.1 & 0.15/0.22/0.32  & 0.10/0.18/0.23  & 0.12/0.25/0.25 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.48/0.52/0.55  & 0.55/0.60/0.67  & 0.45/0.50/0.58 \\ 
 & pi.Linf.1 & 0.40/0.42/0.45  & 0.40/0.40/0.43  & 0.35/0.37/0.47 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.25).mvn.0.01}} & ell.L1 & 0.65/0.67/0.70  & 0.62/0.68/0.72  & 0.52/0.63/0.65 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.90/0.95/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & ell.L2.1 & 0.00/0.05/0.12  & 0.00/0.05/0.07  & 0.05/0.05/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.77/0.85/0.85  & 0.90/0.95/1.00  & 0.80/0.80/0.85 \\ 
 & ell.Linf.1 & 0.45/0.52/0.55  & 0.50/0.55/0.55  & 0.47/0.53/0.55 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.62/0.65/0.67  & 0.62/0.68/0.70  & 0.52/0.63/0.65 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.05/0.10/0.15  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.65/0.67/0.70  & 0.62/0.68/0.72  & 0.52/0.63/0.65 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.90/0.92/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.18/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.90/0.95/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.73/0.82/0.83  & 0.90/0.95/0.97  & 0.80/0.80/0.80 \\ 
 & Linf.0 & 0.00/0.00/0.05  & 0.12/0.25/0.40  & 0.02/0.10/0.10 \\ 
 & Linf.1 & 0.77/0.85/0.85  & 0.90/0.95/1.00  & 0.80/0.80/0.85 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.65/0.67/0.70  & 0.62/0.68/0.72  & 0.52/0.63/0.65 \\ 
 & pi.L1.1 & 0.50/0.52/0.58  & 0.37/0.50/0.58  & 0.40/0.55/0.60 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.90/0.95/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & pi.L2.1 & 0.75/0.77/0.80  & 0.70/0.77/0.80  & 0.70/0.77/0.80 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.77/0.85/0.85  & 0.90/0.95/1.00  & 0.80/0.80/0.85 \\ 
 & pi.Linf.1 & 0.70/0.70/0.75  & 0.63/0.77/0.80  & 0.70/0.72/0.77 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.25).mvn.0.05}} & ell.L1 & 0.10/0.10/0.17  & 0.20/0.25/0.30  & 0.15/0.17/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.50/0.53/0.55  & 0.60/0.75/0.85  & 0.62/0.67/0.68 \\ 
 & ell.L2.1 & 0.00/0.02/0.03  & 0.00/0.02/0.03  & 0.00/0.05/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.50/0.65/0.67  & 0.70/0.70/0.80  & 0.70/0.72/0.75 \\ 
 & ell.Linf.1 & 0.30/0.37/0.50  & 0.30/0.42/0.58  & 0.40/0.48/0.53 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.10/0.10  & 0.30/0.38/0.40  & 0.15/0.15/0.17 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.30/0.38  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.10/0.17  & 0.20/0.25/0.30  & 0.15/0.17/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.50/0.53/0.53  & 0.70/0.80/0.92  & 0.62/0.65/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.35/0.43/0.55  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.50/0.53/0.55  & 0.60/0.75/0.85  & 0.62/0.67/0.68 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.47/0.63/0.67  & 0.73/0.78/0.82  & 0.55/0.70/0.73 \\ 
 & Linf.0 & 0.15/0.23/0.25  & 0.35/0.43/0.47  & 0.25/0.27/0.30 \\ 
 & Linf.1 & 0.50/0.65/0.67  & 0.70/0.70/0.80  & 0.70/0.72/0.75 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.10/0.17  & 0.20/0.25/0.30  & 0.15/0.17/0.25 \\ 
 & pi.L1.1 & 0.10/0.23/0.30  & 0.05/0.15/0.23  & 0.10/0.13/0.28 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.50/0.53/0.55  & 0.60/0.75/0.85  & 0.62/0.67/0.68 \\ 
 & pi.L2.1 & 0.30/0.45/0.57  & 0.22/0.37/0.52  & 0.30/0.47/0.62 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.50/0.65/0.67  & 0.70/0.70/0.80  & 0.70/0.72/0.75 \\ 
 & pi.Linf.1 & 0.50/0.65/0.67  & 0.53/0.65/0.70  & 0.55/0.65/0.73 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.25).mvn.0.1}} & ell.L1 & 0.05/0.10/0.13  & 0.10/0.13/0.17  & 0.05/0.10/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.10/0.17  & 0.13/0.30/0.33  & 0.15/0.15/0.22 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.08  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.20/0.32/0.48  & 0.32/0.48/0.67  & 0.25/0.48/0.55 \\ 
 & ell.Linf.1 & 0.10/0.22/0.32  & 0.15/0.25/0.28  & 0.17/0.23/0.33 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.08/0.10  & 0.33/0.48/0.53  & 0.05/0.10/0.10 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.43/0.47/0.55  & 0.00/0.02/0.12 \\ 
 & L1.1 & 0.05/0.10/0.13  & 0.10/0.13/0.17  & 0.05/0.10/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.08/0.13  & 0.47/0.68/0.77  & 0.15/0.17/0.22 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.65/0.75/0.82  & 0.00/0.05/0.08 \\ 
 & L2.1 & 0.05/0.10/0.17  & 0.13/0.30/0.33  & 0.15/0.15/0.22 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.30/0.40/0.43  & 0.42/0.55/0.70  & 0.30/0.43/0.55 \\ 
 & Linf.0 & 0.25/0.27/0.30  & 0.30/0.38/0.45  & 0.25/0.30/0.37 \\ 
 & Linf.1 & 0.20/0.32/0.48  & 0.32/0.48/0.67  & 0.25/0.48/0.55 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.10/0.13  & 0.10/0.13/0.17  & 0.05/0.10/0.13 \\ 
 & pi.L1.1 & 0.07/0.12/0.15  & 0.05/0.10/0.10  & 0.05/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.10/0.17  & 0.13/0.30/0.33  & 0.15/0.15/0.22 \\ 
 & pi.L2.1 & 0.07/0.12/0.17  & 0.05/0.12/0.15  & 0.05/0.15/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.20/0.32/0.48  & 0.32/0.48/0.67  & 0.25/0.48/0.55 \\ 
 & pi.Linf.1 & 0.32/0.37/0.40  & 0.22/0.28/0.35  & 0.15/0.25/0.27 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.5).mvn.0.01}} & ell.L1 & 0.60/0.65/0.65  & 0.70/0.75/0.75  & 0.70/0.73/0.75 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.90/0.90/0.90  & 0.90/0.90/0.92  & 0.90/0.90/0.90 \\ 
 & ell.L2.1 & 0.00/0.02/0.08  & 0.00/0.07/0.10  & 0.02/0.05/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.90/0.90/0.90  & 0.87/0.87/0.88  & 0.83/0.83/0.83 \\ 
 & ell.Linf.1 & 0.32/0.45/0.53  & 0.30/0.43/0.55  & 0.37/0.45/0.48 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.60/0.65/0.65  & 0.70/0.78/0.80  & 0.70/0.73/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.07/0.17/0.25  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.60/0.65/0.65  & 0.70/0.75/0.75  & 0.70/0.73/0.75 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.90/0.90/0.90  & 1.00/1.00/1.00  & 0.90/0.90/0.90 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.15/0.20/0.20  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.90/0.90/0.90  & 0.90/0.90/0.92  & 0.90/0.90/0.90 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.92/0.95/0.95  & 0.97/0.97/0.97  & 0.83/0.88/0.90 \\ 
 & Linf.0 & 0.05/0.10/0.15  & 0.32/0.45/0.50  & 0.12/0.23/0.32 \\ 
 & Linf.1 & 0.90/0.90/0.90  & 0.87/0.87/0.88  & 0.83/0.83/0.83 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.60/0.65/0.65  & 0.70/0.75/0.75  & 0.70/0.73/0.75 \\ 
 & pi.L1.1 & 0.70/0.82/0.90  & 0.67/0.78/0.82  & 0.68/0.78/0.87 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.90/0.90/0.90  & 0.90/0.90/0.92  & 0.90/0.90/0.90 \\ 
 & pi.L2.1 & 0.80/0.85/0.90  & 0.83/0.85/0.87  & 0.83/0.85/0.88 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.90/0.90/0.90  & 0.87/0.87/0.88  & 0.83/0.83/0.83 \\ 
 & pi.Linf.1 & 0.58/0.68/0.85  & 0.65/0.72/0.72  & 0.53/0.72/0.78 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.5).mvn.0.05}} & ell.L1 & 0.10/0.17/0.30  & 0.25/0.35/0.40  & 0.05/0.10/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.42/0.55/0.62  & 0.57/0.65/0.72  & 0.47/0.53/0.63 \\ 
 & ell.L2.1 & 0.03/0.05/0.10  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.55/0.55/0.70  & 0.68/0.72/0.72  & 0.53/0.68/0.70 \\ 
 & ell.Linf.1 & 0.25/0.38/0.43  & 0.30/0.35/0.40  & 0.30/0.35/0.40 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.12/0.20  & 0.40/0.45/0.53  & 0.05/0.10/0.10 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.30/0.42/0.47  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.17/0.30  & 0.25/0.35/0.40  & 0.05/0.10/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.37/0.53/0.55  & 0.82/0.85/0.87  & 0.47/0.53/0.62 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.37/0.43/0.50  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.42/0.55/0.62  & 0.57/0.65/0.72  & 0.47/0.53/0.63 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.53/0.62/0.77  & 0.73/0.97/0.97  & 0.55/0.68/0.73 \\ 
 & Linf.0 & 0.07/0.33/0.42  & 0.38/0.57/0.62  & 0.30/0.32/0.40 \\ 
 & Linf.1 & 0.55/0.55/0.70  & 0.68/0.72/0.72  & 0.53/0.68/0.70 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.17/0.30  & 0.25/0.35/0.40  & 0.05/0.10/0.25 \\ 
 & pi.L1.1 & 0.17/0.28/0.33  & 0.12/0.18/0.33  & 0.05/0.07/0.20 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.42/0.55/0.62  & 0.57/0.65/0.72  & 0.47/0.53/0.63 \\ 
 & pi.L2.1 & 0.22/0.33/0.40  & 0.25/0.37/0.48  & 0.15/0.18/0.33 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.55/0.55/0.70  & 0.68/0.72/0.72  & 0.53/0.68/0.70 \\ 
 & pi.Linf.1 & 0.47/0.60/0.62  & 0.42/0.55/0.57  & 0.45/0.52/0.58 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.5).mvn.0.1}} & ell.L1 & 0.00/0.03/0.05  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.08  & 0.02/0.12/0.18  & 0.05/0.05/0.08 \\ 
 & ell.L2.1 & 0.00/0.00/0.07  & 0.00/0.05/0.07  & 0.05/0.05/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.17/0.23/0.33  & 0.30/0.37/0.57  & 0.25/0.33/0.37 \\ 
 & ell.Linf.1 & 0.22/0.30/0.33  & 0.20/0.33/0.42  & 0.30/0.35/0.38 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 0.18/0.50/0.55  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.48/0.52/0.57  & 0.00/0.00/0.05 \\ 
 & L1.1 & 0.00/0.03/0.05  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.03/0.07  & 0.40/0.72/0.77  & 0.05/0.12/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.70/0.75/0.77  & 0.00/0.08/0.13 \\ 
 & L2.1 & 0.00/0.03/0.08  & 0.02/0.12/0.18  & 0.05/0.05/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.28/0.30  & 0.27/0.37/0.57  & 0.25/0.30/0.37 \\ 
 & Linf.0 & 0.20/0.22/0.25  & 0.25/0.43/0.57  & 0.25/0.28/0.38 \\ 
 & Linf.1 & 0.17/0.23/0.33  & 0.30/0.37/0.57  & 0.25/0.33/0.37 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.05  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & pi.L1.1 & 0.00/0.08/0.15  & 0.02/0.08/0.10  & 0.05/0.08/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.08  & 0.02/0.12/0.18  & 0.05/0.05/0.08 \\ 
 & pi.L2.1 & 0.00/0.08/0.15  & 0.02/0.08/0.10  & 0.05/0.08/0.17 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.17/0.23/0.33  & 0.30/0.37/0.57  & 0.25/0.33/0.37 \\ 
 & pi.Linf.1 & 0.23/0.25/0.37  & 0.25/0.27/0.35  & 0.25/0.27/0.32 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1.5).mvn.0.01}} & ell.L1 & 0.70/0.75/0.78  & 0.80/0.93/0.95  & 0.80/0.80/0.92 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.85/0.93/0.95  & 0.95/0.98/1.00  & 0.85/0.95/0.98 \\ 
 & ell.L2.1 & 0.15/0.25/0.30  & 0.15/0.20/0.32  & 0.13/0.22/0.27 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.85/0.87/0.87  & 0.90/0.93/0.95  & 0.80/0.83/0.85 \\ 
 & ell.Linf.1 & 0.45/0.45/0.47  & 0.45/0.48/0.50  & 0.40/0.43/0.50 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.70/0.75/0.77  & 0.80/0.85/0.90  & 0.80/0.80/0.80 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.13/0.15  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.70/0.75/0.78  & 0.80/0.93/0.95  & 0.80/0.80/0.92 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.85/0.95/1.00  & 1.00/1.00/1.00  & 0.85/0.95/0.95 \\ 
 & L2.0 & 0.00/0.05/0.05  & 0.25/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.85/0.93/0.95  & 0.95/0.98/1.00  & 0.85/0.95/0.98 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.95/0.95/0.95  & 0.98/1.00/1.00  & 0.80/0.88/0.93 \\ 
 & Linf.0 & 0.10/0.12/0.20  & 0.17/0.32/0.45  & 0.07/0.15/0.20 \\ 
 & Linf.1 & 0.85/0.87/0.87  & 0.90/0.93/0.95  & 0.80/0.83/0.85 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.70/0.75/0.78  & 0.80/0.93/0.95  & 0.80/0.80/0.92 \\ 
 & pi.L1.1 & 0.80/0.88/0.90  & 0.80/0.87/0.90  & 0.80/0.85/0.88 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.85/0.93/0.95  & 0.95/0.98/1.00  & 0.85/0.95/0.98 \\ 
 & pi.L2.1 & 0.80/0.88/0.92  & 0.80/0.87/0.95  & 0.75/0.83/0.88 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.85/0.87/0.87  & 0.90/0.93/0.95  & 0.80/0.83/0.85 \\ 
 & pi.Linf.1 & 0.75/0.75/0.80  & 0.77/0.83/0.85  & 0.75/0.75/0.75 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1.5).mvn.0.05}} & ell.L1 & 0.42/0.50/0.55  & 0.50/0.65/0.65  & 0.50/0.57/0.67 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.85/0.85/0.85  & 0.87/0.90/0.93  & 0.75/0.78/0.88 \\ 
 & ell.L2.1 & 0.05/0.05/0.10  & 0.00/0.05/0.08  & 0.00/0.07/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.75/0.75/0.80  & 0.80/0.83/0.83  & 0.55/0.75/0.75 \\ 
 & ell.Linf.1 & 0.43/0.48/0.53  & 0.40/0.48/0.52  & 0.45/0.45/0.50 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.38/0.50/0.50  & 0.60/0.75/0.75  & 0.48/0.52/0.58 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.28/0.30  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.42/0.50/0.55  & 0.50/0.65/0.65  & 0.50/0.57/0.67 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.85/0.85/0.85  & 0.95/1.00/1.00  & 0.75/0.78/0.82 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.25/0.27/0.27  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.85/0.85/0.85  & 0.87/0.90/0.93  & 0.75/0.78/0.88 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.58/0.75/0.80  & 0.78/0.88/0.88  & 0.55/0.68/0.75 \\ 
 & Linf.0 & 0.05/0.10/0.10  & 0.20/0.25/0.27  & 0.15/0.15/0.15 \\ 
 & Linf.1 & 0.75/0.75/0.80  & 0.80/0.83/0.83  & 0.55/0.75/0.75 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.42/0.50/0.55  & 0.50/0.65/0.65  & 0.50/0.57/0.67 \\ 
 & pi.L1.1 & 0.37/0.50/0.60  & 0.25/0.53/0.58  & 0.42/0.53/0.65 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.85/0.85/0.85  & 0.87/0.90/0.93  & 0.75/0.78/0.88 \\ 
 & pi.L2.1 & 0.62/0.73/0.77  & 0.58/0.73/0.78  & 0.70/0.73/0.82 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.75/0.75/0.80  & 0.80/0.83/0.83  & 0.55/0.75/0.75 \\ 
 & pi.Linf.1 & 0.65/0.65/0.70  & 0.50/0.67/0.68  & 0.50/0.65/0.65 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1.5).mvn.0.1}} & ell.L1 & 0.18/0.27/0.35  & 0.20/0.30/0.38  & 0.10/0.23/0.28 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.57/0.65/0.65  & 0.65/0.75/0.75  & 0.50/0.65/0.68 \\ 
 & ell.L2.1 & 0.05/0.25/0.32  & 0.15/0.22/0.30  & 0.07/0.20/0.30 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.55/0.65/0.68  & 0.57/0.68/0.70  & 0.55/0.65/0.70 \\ 
 & ell.Linf.1 & 0.42/0.48/0.50  & 0.45/0.47/0.53  & 0.45/0.47/0.53 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.17/0.27/0.30  & 0.27/0.55/0.65  & 0.10/0.18/0.27 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.30/0.42/0.45  & 0.00/0.02/0.03 \\ 
 & L1.1 & 0.18/0.27/0.35  & 0.20/0.30/0.38  & 0.10/0.23/0.28 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.57/0.62/0.65  & 0.67/0.93/0.95  & 0.50/0.63/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.32/0.38/0.40  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.57/0.65/0.65  & 0.65/0.75/0.75  & 0.50/0.65/0.68 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.53/0.58/0.67  & 0.62/0.73/0.78  & 0.55/0.58/0.65 \\ 
 & Linf.0 & 0.12/0.15/0.17  & 0.30/0.43/0.53  & 0.15/0.20/0.23 \\ 
 & Linf.1 & 0.55/0.65/0.68  & 0.57/0.68/0.70  & 0.55/0.65/0.70 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.18/0.27/0.35  & 0.20/0.30/0.38  & 0.10/0.23/0.28 \\ 
 & pi.L1.1 & 0.12/0.20/0.20  & 0.10/0.20/0.22  & 0.08/0.20/0.22 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.57/0.65/0.65  & 0.65/0.75/0.75  & 0.50/0.65/0.68 \\ 
 & pi.L2.1 & 0.37/0.45/0.50  & 0.20/0.47/0.50  & 0.25/0.40/0.50 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.55/0.65/0.68  & 0.57/0.68/0.70  & 0.55/0.65/0.70 \\ 
 & pi.Linf.1 & 0.47/0.50/0.58  & 0.40/0.50/0.55  & 0.45/0.53/0.58 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1).mvn.0.01}} & ell.L1 & 0.65/0.68/0.72  & 0.65/0.70/0.90  & 0.60/0.67/0.72 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.85/0.92/0.95  & 0.88/0.92/1.00  & 0.80/0.92/0.95 \\ 
 & ell.L2.1 & 0.10/0.15/0.28  & 0.12/0.18/0.20  & 0.05/0.12/0.22 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.78/0.80/0.82  & 0.83/0.88/0.90  & 0.70/0.78/0.82 \\ 
 & ell.Linf.1 & 0.40/0.45/0.53  & 0.45/0.47/0.50  & 0.42/0.47/0.48 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.65/0.67/0.70  & 0.65/0.73/0.82  & 0.60/0.67/0.67 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.20/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.65/0.68/0.72  & 0.65/0.70/0.90  & 0.60/0.67/0.72 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.85/0.90/0.93  & 0.98/1.00/1.00  & 0.80/0.88/0.92 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.25/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.85/0.92/0.95  & 0.88/0.92/1.00  & 0.80/0.92/0.95 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.77/0.80/0.87  & 0.88/0.93/0.95  & 0.65/0.73/0.83 \\ 
 & Linf.0 & 0.15/0.20/0.23  & 0.15/0.30/0.45  & 0.02/0.10/0.17 \\ 
 & Linf.1 & 0.78/0.80/0.82  & 0.83/0.88/0.90  & 0.70/0.78/0.82 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.65/0.68/0.72  & 0.65/0.70/0.90  & 0.60/0.67/0.72 \\ 
 & pi.L1.1 & 0.75/0.78/0.80  & 0.75/0.80/0.80  & 0.70/0.82/0.87 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.85/0.92/0.95  & 0.88/0.92/1.00  & 0.80/0.92/0.95 \\ 
 & pi.L2.1 & 0.80/0.83/0.85  & 0.80/0.82/0.85  & 0.75/0.85/0.87 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.78/0.80/0.82  & 0.83/0.88/0.90  & 0.70/0.78/0.82 \\ 
 & pi.Linf.1 & 0.55/0.60/0.73  & 0.62/0.70/0.72  & 0.50/0.68/0.75 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1).mvn.0.05}} & ell.L1 & 0.32/0.40/0.42  & 0.42/0.52/0.58  & 0.37/0.45/0.52 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.62/0.70/0.70  & 0.77/0.80/0.88  & 0.63/0.78/0.83 \\ 
 & ell.L2.1 & 0.02/0.10/0.15  & 0.05/0.07/0.10  & 0.05/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.47/0.63/0.73  & 0.62/0.73/0.77  & 0.43/0.67/0.80 \\ 
 & ell.Linf.1 & 0.30/0.30/0.30  & 0.30/0.30/0.30  & 0.35/0.35/0.37 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.27/0.35/0.40  & 0.45/0.57/0.63  & 0.35/0.45/0.45 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.25/0.30/0.35  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.32/0.40/0.42  & 0.42/0.52/0.58  & 0.37/0.45/0.52 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.62/0.68/0.70  & 0.85/0.93/0.95  & 0.63/0.77/0.82 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.32/0.40/0.40  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.62/0.70/0.70  & 0.77/0.80/0.88  & 0.63/0.78/0.83 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.38/0.53/0.62  & 0.55/0.80/0.88  & 0.42/0.55/0.67 \\ 
 & Linf.0 & 0.00/0.10/0.15  & 0.10/0.28/0.37  & 0.15/0.15/0.18 \\ 
 & Linf.1 & 0.47/0.63/0.73  & 0.62/0.73/0.77  & 0.43/0.67/0.80 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.32/0.40/0.42  & 0.42/0.52/0.58  & 0.37/0.45/0.52 \\ 
 & pi.L1.1 & 0.15/0.30/0.42  & 0.20/0.30/0.47  & 0.17/0.35/0.47 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.62/0.70/0.70  & 0.77/0.80/0.88  & 0.63/0.78/0.83 \\ 
 & pi.L2.1 & 0.38/0.52/0.65  & 0.43/0.65/0.70  & 0.38/0.62/0.72 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.47/0.63/0.73  & 0.62/0.73/0.77  & 0.43/0.67/0.80 \\ 
 & pi.Linf.1 & 0.40/0.52/0.60  & 0.45/0.50/0.53  & 0.42/0.52/0.60 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1).mvn.0.1}} & ell.L1 & 0.00/0.07/0.17  & 0.02/0.18/0.23  & 0.00/0.03/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.03/0.12/0.18  & 0.08/0.28/0.33  & 0.00/0.17/0.23 \\ 
 & ell.L2.1 & 0.05/0.20/0.28  & 0.12/0.17/0.18  & 0.00/0.00/0.20 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.23/0.37/0.37  & 0.35/0.37/0.42  & 0.27/0.37/0.37 \\ 
 & ell.Linf.1 & 0.17/0.27/0.38  & 0.20/0.20/0.33  & 0.20/0.23/0.30 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.05/0.12  & 0.18/0.38/0.50  & 0.00/0.03/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.33/0.53/0.58  & 0.02/0.05/0.05 \\ 
 & L1.1 & 0.00/0.07/0.17  & 0.02/0.18/0.23  & 0.00/0.03/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.03/0.10/0.13  & 0.42/0.65/0.73  & 0.00/0.17/0.18 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.50/0.60/0.62  & 0.00/0.00/0.05 \\ 
 & L2.1 & 0.03/0.12/0.18  & 0.08/0.28/0.33  & 0.00/0.17/0.23 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.43/0.50  & 0.50/0.67/0.70  & 0.28/0.37/0.45 \\ 
 & Linf.0 & 0.20/0.20/0.38  & 0.52/0.62/0.67  & 0.20/0.28/0.45 \\ 
 & Linf.1 & 0.23/0.37/0.37  & 0.35/0.37/0.42  & 0.27/0.37/0.37 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.07/0.17  & 0.02/0.18/0.23  & 0.00/0.03/0.10 \\ 
 & pi.L1.1 & 0.00/0.05/0.17  & 0.00/0.08/0.17  & 0.02/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.03/0.12/0.18  & 0.08/0.28/0.33  & 0.00/0.17/0.23 \\ 
 & pi.L2.1 & 0.02/0.17/0.25  & 0.05/0.17/0.25  & 0.05/0.08/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.23/0.37/0.37  & 0.35/0.37/0.42  & 0.27/0.37/0.37 \\ 
 & pi.Linf.1 & 0.25/0.32/0.35  & 0.25/0.27/0.32  & 0.27/0.32/0.35 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(5).mvn.0.01}} & ell.L1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & ell.L2.1 & 0.10/0.10/0.15  & 0.10/0.10/0.10  & 0.05/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.92/0.95/0.95  & 0.87/0.90/0.90  & 0.85/0.85/0.88 \\ 
 & ell.Linf.1 & 0.30/0.32/0.35  & 0.30/0.30/0.30  & 0.30/0.33/0.35 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.10/0.15  & 0.00/0.00/0.00 \\ 
 & L2.1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.95/0.95/0.95  & 0.93/1.00/1.00  & 0.82/0.85/0.85 \\ 
 & Linf.0 & 0.05/0.07/0.15  & 0.25/0.38/0.48  & 0.00/0.00/0.05 \\ 
 & Linf.1 & 0.92/0.95/0.95  & 0.87/0.90/0.90  & 0.85/0.85/0.88 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & pi.L1.1 & 0.88/1.00/1.00  & 0.87/0.93/1.00  & 0.92/0.97/1.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & pi.L2.1 & 0.87/0.98/1.00  & 0.87/0.93/1.00  & 0.92/0.95/1.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.92/0.95/0.95  & 0.87/0.90/0.90  & 0.85/0.85/0.88 \\ 
 & pi.Linf.1 & 0.77/0.82/0.82  & 0.80/0.80/0.80  & 0.80/0.80/0.80 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(5).mvn.0.05}} & ell.L1 & 0.70/0.70/0.70  & 0.72/0.83/0.87  & 0.70/0.73/0.82 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & ell.L2.1 & 0.12/0.23/0.25  & 0.20/0.23/0.27  & 0.20/0.27/0.32 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.95/0.95/0.95  & 0.95/0.95/0.95  & 0.90/0.90/0.90 \\ 
 & ell.Linf.1 & 0.35/0.38/0.40  & 0.40/0.43/0.47  & 0.45/0.45/0.45 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.70/0.70/0.70  & 0.72/0.83/0.83  & 0.70/0.72/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.70/0.70/0.70  & 0.72/0.83/0.87  & 0.70/0.73/0.82 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.02/0.12/0.13  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.92/0.95/0.95  & 0.95/0.95/0.98  & 0.90/0.90/0.90 \\ 
 & Linf.0 & 0.00/0.02/0.07  & 0.10/0.15/0.30  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.95/0.95/0.95  & 0.95/0.95/0.95  & 0.90/0.90/0.90 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.70/0.70/0.70  & 0.72/0.83/0.87  & 0.70/0.73/0.82 \\ 
 & pi.L1.1 & 0.90/0.95/0.95  & 0.88/0.95/0.95  & 0.95/0.95/0.95 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & pi.L2.1 & 0.92/0.95/0.95  & 0.88/0.95/0.95  & 0.95/0.95/0.95 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.95/0.95/0.95  & 0.95/0.95/0.95  & 0.90/0.90/0.90 \\ 
 & pi.Linf.1 & 0.85/0.90/0.95  & 0.82/0.87/0.95  & 0.80/0.85/0.85 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(5).mvn.0.1}} & ell.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & ell.L2.1 & 0.00/0.07/0.15  & 0.00/0.05/0.12  & 0.00/0.03/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.87/0.90/0.95  & 0.83/0.87/0.88  & 0.85/0.88/0.97 \\ 
 & ell.Linf.1 & 0.40/0.42/0.45  & 0.37/0.43/0.50  & 0.35/0.40/0.47 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.00/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & L2.1 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.80/0.83/0.90  & 0.85/0.93/0.97  & 0.80/0.88/0.92 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.07/0.23/0.30  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.87/0.90/0.95  & 0.83/0.87/0.88  & 0.85/0.88/0.97 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & pi.L1.1 & 0.72/0.75/0.83  & 0.75/0.77/0.83  & 0.70/0.82/0.88 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & pi.L2.1 & 0.82/0.83/0.92  & 0.85/0.87/0.90  & 0.80/0.88/0.98 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.87/0.90/0.95  & 0.83/0.87/0.88  & 0.85/0.88/0.97 \\ 
 & pi.Linf.1 & 0.80/0.80/0.82  & 0.75/0.75/0.75  & 0.75/0.78/0.80 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(2).mvn.0.01}} & ell.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.18  & 0.05/0.13/0.25  & 0.03/0.10/0.23 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 1.00/1.00/1.00  & 0.85/0.85/0.85  & 0.90/0.93/0.95 \\ 
 & ell.Linf.1 & 0.52/0.60/0.60  & 0.55/0.60/0.60  & 0.50/0.55/0.60 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.05/0.12/0.17  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.17/0.20  & 0.00/0.00/0.00 \\ 
 & L2.1 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 1.00/1.00/1.00  & 0.90/0.90/0.93  & 0.90/0.93/0.95 \\ 
 & Linf.0 & 0.02/0.10/0.10  & 0.10/0.15/0.20  & 0.05/0.07/0.12 \\ 
 & Linf.1 & 1.00/1.00/1.00  & 0.85/0.85/0.85  & 0.90/0.93/0.95 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & pi.L1.1 & 0.70/0.83/0.85  & 0.80/0.80/0.80  & 0.70/0.77/0.80 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & pi.L2.1 & 0.95/1.00/1.00  & 1.00/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 1.00/1.00/1.00  & 0.85/0.85/0.85  & 0.90/0.93/0.95 \\ 
 & pi.Linf.1 & 0.90/0.95/1.00  & 0.80/0.80/0.85  & 0.85/0.88/0.93 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(2).mvn.0.05}} & ell.L1 & 0.10/0.17/0.20  & 0.13/0.27/0.32  & 0.10/0.18/0.28 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.40/0.52/0.58  & 0.67/0.75/0.78  & 0.55/0.63/0.77 \\ 
 & ell.L2.1 & 0.05/0.10/0.15  & 0.05/0.05/0.10  & 0.00/0.03/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.57/0.70/0.72  & 0.72/0.78/0.80  & 0.68/0.80/0.80 \\ 
 & ell.Linf.1 & 0.30/0.38/0.43  & 0.35/0.40/0.47  & 0.30/0.43/0.48 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.13/0.17  & 0.17/0.28/0.40  & 0.10/0.15/0.17 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.25/0.37/0.47  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.17/0.20  & 0.13/0.27/0.32  & 0.10/0.18/0.28 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.38/0.50/0.57  & 0.67/0.82/0.88  & 0.55/0.60/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.23/0.37/0.52  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.40/0.52/0.58  & 0.67/0.75/0.78  & 0.55/0.63/0.77 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.52/0.67/0.72  & 0.73/0.82/0.87  & 0.68/0.80/0.83 \\ 
 & Linf.0 & 0.10/0.17/0.23  & 0.30/0.33/0.48  & 0.22/0.28/0.35 \\ 
 & Linf.1 & 0.57/0.70/0.72  & 0.72/0.78/0.80  & 0.68/0.80/0.80 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.17/0.20  & 0.13/0.27/0.32  & 0.10/0.18/0.28 \\ 
 & pi.L1.1 & 0.10/0.25/0.33  & 0.20/0.23/0.32  & 0.22/0.25/0.27 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.40/0.52/0.58  & 0.67/0.75/0.78  & 0.55/0.63/0.77 \\ 
 & pi.L2.1 & 0.30/0.42/0.53  & 0.30/0.43/0.60  & 0.35/0.43/0.58 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.57/0.70/0.72  & 0.72/0.78/0.80  & 0.68/0.80/0.80 \\ 
 & pi.Linf.1 & 0.55/0.65/0.65  & 0.60/0.70/0.70  & 0.65/0.65/0.70 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(2).mvn.0.1}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.08  & 0.15/0.18/0.30  & 0.05/0.13/0.22 \\ 
 & ell.L2.1 & 0.07/0.13/0.20  & 0.00/0.02/0.10  & 0.00/0.12/0.20 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.12/0.17/0.27  & 0.28/0.53/0.58  & 0.28/0.37/0.47 \\ 
 & ell.Linf.1 & 0.27/0.32/0.38  & 0.25/0.30/0.33  & 0.20/0.25/0.38 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.38/0.62/0.65  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.58/0.67/0.70  & 0.00/0.00/0.03 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.02  & 0.75/0.87/0.90  & 0.08/0.15/0.30 \\ 
 & L2.0 & 0.00/0.02/0.05  & 0.70/0.85/0.85  & 0.05/0.20/0.27 \\ 
 & L2.1 & 0.00/0.02/0.08  & 0.15/0.18/0.30  & 0.05/0.13/0.22 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.37/0.37  & 0.50/0.63/0.75  & 0.28/0.38/0.57 \\ 
 & Linf.0 & 0.23/0.32/0.37  & 0.40/0.53/0.67  & 0.25/0.37/0.50 \\ 
 & Linf.1 & 0.12/0.17/0.27  & 0.28/0.53/0.58  & 0.28/0.37/0.47 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & pi.L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.00/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.08  & 0.15/0.18/0.30  & 0.05/0.13/0.22 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.00/0.05  & 0.00/0.02/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.12/0.17/0.27  & 0.28/0.53/0.58  & 0.28/0.37/0.47 \\ 
 & pi.Linf.1 & 0.25/0.40/0.43  & 0.25/0.35/0.42  & 0.27/0.33/0.40 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(3).mvn.0.01}} & ell.L1 & 0.25/0.38/0.53  & 0.53/0.62/0.75  & 0.05/0.22/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.18/0.38/0.57  & 0.63/0.68/0.82  & 0.05/0.13/0.23 \\ 
 & ell.L2.1 & 0.02/0.12/0.15  & 0.05/0.10/0.15  & 0.07/0.13/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.12/0.23/0.40  & 0.58/0.77/0.95  & 0.10/0.17/0.22 \\ 
 & ell.Linf.1 & 0.05/0.12/0.20  & 0.07/0.15/0.20  & 0.08/0.08/0.18 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.20/0.33/0.47  & 0.75/0.75/0.75  & 0.03/0.13/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.75/0.75/0.75  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.25/0.38/0.53  & 0.53/0.62/0.75  & 0.05/0.22/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.13/0.28/0.47  & 0.75/0.75/0.75  & 0.05/0.10/0.13 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.75/0.75/0.75  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.18/0.38/0.57  & 0.63/0.68/0.82  & 0.05/0.13/0.23 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.12/0.22/0.30  & 0.62/0.68/0.82  & 0.10/0.10/0.18 \\ 
 & Linf.0 & 0.02/0.05/0.05  & 0.33/0.43/0.48  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.12/0.23/0.40  & 0.58/0.77/0.95  & 0.10/0.17/0.22 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.25/0.38/0.53  & 0.53/0.62/0.75  & 0.05/0.22/0.25 \\ 
 & pi.L1.1 & 0.40/0.45/0.58  & 0.20/0.48/0.58  & 0.48/0.53/0.60 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.18/0.38/0.57  & 0.63/0.68/0.82  & 0.05/0.13/0.23 \\ 
 & pi.L2.1 & 0.35/0.45/0.58  & 0.20/0.43/0.58  & 0.48/0.53/0.60 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.12/0.23/0.40  & 0.58/0.77/0.95  & 0.10/0.17/0.22 \\ 
 & pi.Linf.1 & 0.13/0.40/0.58  & 0.17/0.37/0.52  & 0.25/0.37/0.57 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(3).mvn.0.05}} & ell.L1 & 0.10/0.15/0.15  & 0.45/0.47/0.58  & 0.03/0.10/0.18 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.08/0.10/0.13  & 0.43/0.53/0.62  & 0.00/0.08/0.15 \\ 
 & ell.L2.1 & 0.05/0.07/0.17  & 0.07/0.12/0.17  & 0.10/0.10/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.07  & 0.33/0.42/0.45  & 0.00/0.00/0.03 \\ 
 & ell.Linf.1 & 0.05/0.08/0.15  & 0.05/0.08/0.10  & 0.00/0.07/0.12 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.10/0.10  & 0.92/0.93/0.95  & 0.02/0.05/0.12 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/0.95/0.97  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.15/0.15  & 0.45/0.47/0.58  & 0.03/0.10/0.18 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.08/0.10/0.10  & 0.95/1.00/1.00  & 0.00/0.02/0.07 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.08/0.10/0.13  & 0.43/0.53/0.62  & 0.00/0.08/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.03/0.07/0.10  & 0.45/0.70/0.88  & 0.10/0.10/0.18 \\ 
 & Linf.0 & 0.05/0.05/0.05  & 0.38/0.63/0.80  & 0.12/0.18/0.23 \\ 
 & Linf.1 & 0.05/0.05/0.07  & 0.33/0.42/0.45  & 0.00/0.00/0.03 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.15/0.15  & 0.45/0.47/0.58  & 0.03/0.10/0.18 \\ 
 & pi.L1.1 & 0.15/0.27/0.37  & 0.12/0.18/0.37  & 0.15/0.28/0.38 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.08/0.10/0.13  & 0.43/0.53/0.62  & 0.00/0.08/0.15 \\ 
 & pi.L2.1 & 0.15/0.25/0.38  & 0.13/0.25/0.35  & 0.15/0.25/0.38 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.07  & 0.33/0.42/0.45  & 0.00/0.00/0.03 \\ 
 & pi.Linf.1 & 0.05/0.07/0.28  & 0.05/0.12/0.32  & 0.10/0.15/0.28 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(3).mvn.0.1}} & ell.L1 & 0.00/0.00/0.02  & 0.02/0.13/0.30  & 0.00/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.05  & 0.07/0.18/0.35  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.02/0.05/0.08  & 0.00/0.03/0.05  & 0.00/0.05/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.05  & 0.07/0.20/0.32  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.02/0.08  & 0.00/0.02/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.80/0.90/0.95  & 0.00/0.00/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.85/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.02  & 0.02/0.13/0.30  & 0.00/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.95/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.97/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.05  & 0.07/0.18/0.35  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.03  & 0.53/0.80/0.85  & 0.23/0.30/0.33 \\ 
 & Linf.0 & 0.00/0.02/0.07  & 0.60/0.80/0.95  & 0.25/0.33/0.33 \\ 
 & Linf.1 & 0.00/0.02/0.05  & 0.07/0.20/0.32  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.02  & 0.02/0.13/0.30  & 0.00/0.05/0.07 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.05/0.08  & 0.05/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.05  & 0.07/0.18/0.35  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.05/0.08  & 0.05/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.05  & 0.07/0.20/0.32  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.03/0.12  & 0.00/0.02/0.08 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.05)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.02/0.07  & 0.00/0.00/0.03  & 0.00/0.03/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.08 \\ 
 & ell.Linf.1 & 0.00/0.02/0.05  & 0.02/0.03/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.12/0.20/0.20  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.17/0.20/0.20  & 0.05/0.05/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.30/0.30/0.30  & 0.55/0.63/0.68  & 0.45/0.45/0.48 \\ 
 & L2.0 & 0.30/0.30/0.30  & 0.57/0.68/0.70  & 0.45/0.50/0.50 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.82/0.82/0.85  & 0.95/0.97/0.98  & 0.85/0.90/0.95 \\ 
 & Linf.0 & 0.82/0.90/0.95  & 0.95/0.98/1.00  & 0.90/0.92/1.00 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.1)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.02/0.05/0.05  & 0.05/0.05/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.12/0.17/0.20  & 0.10/0.18/0.23  & 0.10/0.13/0.15 \\ 
 & ell.Linf.1 & 0.03/0.05/0.08  & 0.02/0.10/0.10  & 0.00/0.03/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.08  & 0.25/0.27/0.28  & 0.10/0.17/0.20 \\ 
 & L1.0 & 0.07/0.08/0.10  & 0.25/0.27/0.37  & 0.20/0.20/0.20 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.20/0.22/0.23  & 0.43/0.47/0.48  & 0.27/0.32/0.37 \\ 
 & L2.0 & 0.22/0.25/0.25  & 0.47/0.50/0.52  & 0.27/0.37/0.42 \\ 
 & L2.1 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.62/0.70/0.70  & 0.72/0.75/0.75  & 0.70/0.70/0.75 \\ 
 & Linf.0 & 0.63/0.70/0.72  & 0.72/0.75/0.78  & 0.70/0.70/0.75 \\ 
 & Linf.1 & 0.12/0.17/0.20  & 0.10/0.18/0.23  & 0.10/0.13/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.00/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.12/0.17/0.20  & 0.10/0.18/0.23  & 0.10/0.13/0.15 \\ 
 & pi.Linf.1 & 0.05/0.05/0.12  & 0.05/0.10/0.13  & 0.00/0.05/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.15)}} & ell.L1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.10/0.15  & 0.10/0.13/0.20  & 0.05/0.05/0.08 \\ 
 & ell.L2.1 & 0.05/0.07/0.10  & 0.05/0.05/0.07  & 0.05/0.07/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.10/0.13/0.15  & 0.15/0.17/0.23  & 0.05/0.12/0.15 \\ 
 & ell.Linf.1 & 0.00/0.05/0.10  & 0.00/0.00/0.10  & 0.00/0.02/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.20/0.20/0.22  & 0.30/0.40/0.40  & 0.25/0.27/0.30 \\ 
 & L1.0 & 0.20/0.20/0.20  & 0.37/0.40/0.40  & 0.27/0.32/0.35 \\ 
 & L1.1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.30/0.30/0.33  & 0.45/0.52/0.57  & 0.35/0.38/0.40 \\ 
 & L2.0 & 0.30/0.32/0.35  & 0.55/0.55/0.55  & 0.40/0.40/0.40 \\ 
 & L2.1 & 0.05/0.10/0.15  & 0.10/0.13/0.20  & 0.05/0.05/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.40/0.48/0.55  & 0.57/0.65/0.68  & 0.42/0.48/0.53 \\ 
 & Linf.0 & 0.35/0.50/0.55  & 0.53/0.65/0.75  & 0.42/0.52/0.58 \\ 
 & Linf.1 & 0.10/0.13/0.15  & 0.15/0.17/0.23  & 0.05/0.12/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.02/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.10/0.15  & 0.10/0.13/0.20  & 0.05/0.05/0.08 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.05/0.07  & 0.00/0.00/0.03 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.10/0.13/0.15  & 0.15/0.17/0.23  & 0.05/0.12/0.15 \\ 
 & pi.Linf.1 & 0.10/0.12/0.15  & 0.05/0.17/0.22  & 0.12/0.15/0.20 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.2)}} & ell.L1 & 0.05/0.08/0.15  & 0.17/0.20/0.23  & 0.05/0.10/0.15 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.15/0.15/0.20  & 0.15/0.23/0.33  & 0.15/0.15/0.20 \\ 
 & ell.L2.1 & 0.05/0.07/0.08  & 0.02/0.05/0.05  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.15/0.22/0.22  & 0.15/0.25/0.25  & 0.15/0.25/0.25 \\ 
 & ell.Linf.1 & 0.02/0.05/0.07  & 0.00/0.05/0.08  & 0.00/0.00/0.07 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.25/0.32/0.33  & 0.60/0.65/0.72  & 0.40/0.50/0.50 \\ 
 & L1.0 & 0.32/0.33/0.38  & 0.65/0.70/0.75  & 0.45/0.50/0.52 \\ 
 & L1.1 & 0.05/0.08/0.15  & 0.17/0.20/0.23  & 0.05/0.10/0.15 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.40/0.40/0.40  & 0.65/0.73/0.75  & 0.45/0.52/0.55 \\ 
 & L2.0 & 0.40/0.40/0.43  & 0.75/0.75/0.75  & 0.50/0.55/0.55 \\ 
 & L2.1 & 0.15/0.15/0.20  & 0.15/0.23/0.33  & 0.15/0.15/0.20 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.33/0.42  & 0.52/0.57/0.63  & 0.32/0.43/0.50 \\ 
 & Linf.0 & 0.27/0.38/0.53  & 0.47/0.52/0.67  & 0.30/0.43/0.48 \\ 
 & Linf.1 & 0.15/0.22/0.22  & 0.15/0.25/0.25  & 0.15/0.25/0.25 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.08/0.15  & 0.17/0.20/0.23  & 0.05/0.10/0.15 \\ 
 & pi.L1.1 & 0.02/0.05/0.07  & 0.00/0.05/0.07  & 0.05/0.05/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.15/0.15/0.20  & 0.15/0.23/0.33  & 0.15/0.15/0.20 \\ 
 & pi.L2.1 & 0.02/0.05/0.05  & 0.00/0.05/0.07  & 0.00/0.03/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.15/0.22/0.22  & 0.15/0.25/0.25  & 0.15/0.25/0.25 \\ 
 & pi.Linf.1 & 0.00/0.03/0.10  & 0.02/0.08/0.10  & 0.00/0.08/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.25)}} & ell.L1 & 0.10/0.10/0.12  & 0.10/0.15/0.18  & 0.05/0.07/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.10/0.15/0.15  & 0.05/0.12/0.15  & 0.08/0.10/0.10 \\ 
 & ell.L2.1 & 0.00/0.03/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.05  & 0.05/0.07/0.10  & 0.05/0.05/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.32/0.37/0.45  & 0.50/0.55/0.55  & 0.30/0.37/0.40 \\ 
 & L1.0 & 0.35/0.45/0.45  & 0.55/0.55/0.55  & 0.35/0.38/0.40 \\ 
 & L1.1 & 0.10/0.10/0.12  & 0.10/0.15/0.18  & 0.05/0.07/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.35/0.35/0.42  & 0.50/0.50/0.52  & 0.30/0.42/0.45 \\ 
 & L2.0 & 0.35/0.47/0.50  & 0.50/0.52/0.55  & 0.40/0.45/0.45 \\ 
 & L2.1 & 0.10/0.15/0.15  & 0.05/0.12/0.15  & 0.08/0.10/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.10/0.17/0.38  & 0.32/0.50/0.58  & 0.17/0.25/0.33 \\ 
 & Linf.0 & 0.05/0.28/0.50  & 0.33/0.55/0.60  & 0.22/0.25/0.40 \\ 
 & Linf.1 & 0.05/0.05/0.05  & 0.05/0.07/0.10  & 0.05/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.10/0.12  & 0.10/0.15/0.18  & 0.05/0.07/0.12 \\ 
 & pi.L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.10/0.15/0.15  & 0.05/0.12/0.15  & 0.08/0.10/0.10 \\ 
 & pi.L2.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.05  & 0.05/0.07/0.10  & 0.05/0.05/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 


==> arXiv submission multiple hypothesis/reject-rates-acyclic-additive-validation.tex <==
\multirow{6}{*}{axis}
& \texttt{L1.0} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{L1.1} & 0.11/0.21/0.55 & 0.00/0.00/0.19 \\ 
& \texttt{L2.0} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{L2.1} & 0.21/0.31/0.42 & 0.00/0.08/0.15 \\ 
& \texttt{Linf.0} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{Linf.1} & 0.00/0.10/0.10 & 0.00/0.08/0.08 \\ 
\midrule\multirow{6}{*}{ball}
& \texttt{L1.0} & 0.00/0.00/0.00 & 0.00/0.02/0.03 \\ 
& \texttt{L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{L2.0} & 0.00/0.00/0.00 & 0.00/0.01/0.01 \\ 
& \texttt{L2.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{Linf.0} & 0.00/0.00/0.00 & 0.00/0.00/0.01 \\ 
& \texttt{Linf.1} & 0.00/0.02/0.02 & 0.01/0.01/0.01 \\ 
\midrule\multirow{6}{*}{cross}
& \texttt{L1.0} & 0.18/0.18/0.18 & 0.13/0.13/0.21 \\ 
& \texttt{L1.1} & 0.00/0.00/0.00 & 0.00/0.22/0.32 \\ 
& \texttt{L2.0} & 0.18/0.18/0.18 & 0.13/0.13/0.21 \\ 
& \texttt{L2.1} & 0.00/0.00/0.00 & 0.00/0.00/0.32 \\ 
& \texttt{Linf.0} & 0.11/0.11/0.19 & 0.13/0.13/0.23 \\ 
& \texttt{Linf.1} & 0.00/0.00/0.00 & 0.00/0.00/0.11 \\ 
\midrule\multirow{6}{*}{random.hull}
& \texttt{L1.0} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{L1.1} & 0.00/0.00/0.00 & 0.10/0.10/0.10 \\ 
& \texttt{L2.0} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{L2.1} & 0.00/0.00/0.00 & 0.10/0.10/0.10 \\ 
& \texttt{Linf.0} & 0.00/0.00/0.02 & 0.00/0.00/0.09 \\ 
& \texttt{Linf.1} & 0.00/0.02/0.02 & 0.01/0.04/0.09 \\ 
\midrule\multirow{6}{*}{random.polytope}
& \texttt{L1.0} & 0.00/0.00/0.00 & 0.02/0.02/0.07 \\ 
& \texttt{L1.1} & 0.00/0.02/0.07 & 0.01/0.03/0.04 \\ 
& \texttt{L2.0} & 0.00/0.00/0.00 & 0.00/0.02/0.07 \\ 
& \texttt{L2.1} & 0.00/0.02/0.04 & 0.01/0.03/0.08 \\ 
& \texttt{Linf.0} & 0.00/0.05/0.05 & 0.04/0.04/0.04 \\ 
& \texttt{Linf.1} & 0.00/0.00/0.05 & 0.00/0.02/0.13 \\ 
\midrule\multirow{6}{*}{simplex}
& \texttt{L1.0} & 0.00/0.00/0.00 & 0.01/0.03/0.09 \\ 
& \texttt{L1.1} & 0.00/0.00/0.00 & 0.00/0.02/0.04 \\ 
& \texttt{L2.0} & 0.00/0.00/0.00 & 0.02/0.03/0.05 \\ 
& \texttt{L2.1} & 0.00/0.00/0.00 & 0.00/0.00/0.02 \\ 
& \texttt{Linf.0} & 0.01/0.02/0.02 & 0.00/0.03/0.11 \\ 
& \texttt{Linf.1} & 0.00/0.00/0.00 & 0.00/0.02/0.03 \\ 
\midrule

==> arXiv submission multiple hypothesis/reject-rates-acyclic-all-validation.tex <==
\texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
\texttt{ell.L2.1} & 0.04/0.09/0.13 & 0.04/0.07/0.12 & 0.04/0.07/0.11 \\ 
\texttt{ell.Linf.1} & 0.00/0.02/0.05 & 0.03/0.03/0.05 & 0.00/0.03/0.08 \\ 
\texttt{pi.L1.1} & 0.08/0.14/0.21 & 0.11/0.17/0.20 & 0.06/0.14/0.20 \\ 
\texttt{pi.L2.1} & 0.10/0.12/0.20 & 0.10/0.14/0.19 & 0.06/0.13/0.18 \\ 
\texttt{pi.Linf.1} & 0.02/0.04/0.06 & 0.03/0.04/0.10 & 0.03/0.07/0.12 \\ 


==> arXiv submission multiple hypothesis/reject-rates-acyclic-combined-validation.tex <==
\texttt{L1.0} & 0.06/0.07/0.08 & 0.09/0.10/0.15 \\ 
\texttt{L1.1} & 0.03/0.05/0.07 & 0.02/0.03/0.06 \\ 
\texttt{L2.0} & 0.08/0.08/0.10 & 0.05/0.11/0.14 \\ 
\texttt{L2.1} & 0.06/0.07/0.09 & 0.02/0.07/0.07 \\ 
\texttt{Linf.0} & 0.07/0.10/0.11 & 0.01/0.03/0.08 \\ 
\texttt{Linf.1} & 0.00/0.02/0.07 & 0.00/0.02/0.04 \\ 


==> arXiv submission multiple hypothesis/reject-rates-acyclic-composite-validation.tex <==
\multirow{12}{*}{axis}
& \texttt{ell} & 0.02/0.05/0.11 & 0.04/0.08/0.13 \\ 
& \texttt{ell.L1} & 0.02/0.05/0.09 & 0.03/0.03/0.10 \\ 
& \texttt{ell.L2} & 0.03/0.04/0.08 & 0.03/0.09/0.10 \\ 
& \texttt{ell.Linf} & 0.01/0.04/0.06 & 0.01/0.07/0.07 \\ 
& \texttt{L} & 0.08/0.14/0.21 & 0.03/0.04/0.16 \\ 
& \texttt{L1} & 0.02/0.08/0.12 & 0.03/0.03/0.10 \\ 
& \texttt{L2} & 0.05/0.11/0.18 & 0.01/0.05/0.12 \\ 
& \texttt{Linf} & 0.06/0.13/0.19 & 0.01/0.06/0.14 \\ 
& \texttt{pi} & 0.02/0.05/0.11 & 0.04/0.08/0.13 \\ 
& \texttt{pi.L1} & 0.02/0.05/0.09 & 0.03/0.03/0.10 \\ 
& \texttt{pi.L2} & 0.03/0.04/0.08 & 0.03/0.09/0.10 \\ 
& \texttt{pi.Linf} & 0.01/0.04/0.06 & 0.01/0.07/0.07 \\ 
\midrule\multirow{12}{*}{ball}
& \texttt{ell} & 0.01/0.03/0.04 & 0.00/0.00/0.03 \\ 
& \texttt{ell.L1} & 0.01/0.01/0.01 & 0.00/0.00/0.01 \\ 
& \texttt{ell.L2} & 0.01/0.01/0.04 & 0.00/0.00/0.01 \\ 
& \texttt{ell.Linf} & 0.00/0.03/0.05 & 0.02/0.02/0.03 \\ 
& \texttt{L} & 0.01/0.03/0.03 & 0.00/0.01/0.03 \\ 
& \texttt{L1} & 0.01/0.01/0.01 & 0.01/0.01/0.05 \\ 
& \texttt{L2} & 0.01/0.01/0.03 & 0.01/0.01/0.02 \\ 
& \texttt{Linf} & 0.00/0.02/0.03 & 0.00/0.02/0.03 \\ 
& \texttt{pi} & 0.01/0.03/0.04 & 0.00/0.00/0.03 \\ 
& \texttt{pi.L1} & 0.01/0.01/0.01 & 0.00/0.00/0.01 \\ 
& \texttt{pi.L2} & 0.01/0.01/0.04 & 0.00/0.00/0.01 \\ 
& \texttt{pi.Linf} & 0.00/0.03/0.05 & 0.02/0.02/0.03 \\ 
\midrule\multirow{12}{*}{cross}
& \texttt{ell} & 0.00/0.00/0.03 & 0.00/0.03/0.05 \\ 
& \texttt{ell.L1} & 0.00/0.01/0.03 & 0.02/0.07/0.08 \\ 
& \texttt{ell.L2} & 0.00/0.01/0.01 & 0.01/0.02/0.04 \\ 
& \texttt{ell.Linf} & 0.00/0.00/0.01 & 0.00/0.01/0.04 \\ 
& \texttt{L} & 0.26/0.32/0.36 & 0.12/0.17/0.25 \\ 
& \texttt{L1} & 0.14/0.14/0.15 & 0.14/0.16/0.18 \\ 
& \texttt{L2} & 0.15/0.16/0.16 & 0.10/0.15/0.19 \\ 
& \texttt{Linf} & 0.25/0.30/0.35 & 0.02/0.08/0.16 \\ 
& \texttt{pi} & 0.00/0.00/0.03 & 0.00/0.03/0.05 \\ 
& \texttt{pi.L1} & 0.00/0.01/0.03 & 0.02/0.07/0.08 \\ 
& \texttt{pi.L2} & 0.00/0.01/0.01 & 0.01/0.02/0.04 \\ 
& \texttt{pi.Linf} & 0.00/0.00/0.01 & 0.00/0.01/0.04 \\ 
\midrule\multirow{12}{*}{random.hull}
& \texttt{ell} & 0.00/0.00/0.01 & 0.02/0.04/0.04 \\ 
& \texttt{ell.L1} & 0.00/0.00/0.02 & 0.02/0.03/0.05 \\ 
& \texttt{ell.L2} & 0.00/0.00/0.01 & 0.03/0.03/0.05 \\ 
& \texttt{ell.Linf} & 0.00/0.01/0.02 & 0.01/0.02/0.03 \\ 
& \texttt{L} & 0.00/0.00/0.00 & 0.01/0.03/0.04 \\ 
& \texttt{L1} & 0.00/0.00/0.00 & 0.02/0.03/0.04 \\ 
& \texttt{L2} & 0.00/0.00/0.00 & 0.02/0.03/0.05 \\ 
& \texttt{Linf} & 0.00/0.00/0.01 & 0.00/0.02/0.03 \\ 
& \texttt{pi} & 0.00/0.00/0.01 & 0.02/0.04/0.04 \\ 
& \texttt{pi.L1} & 0.00/0.00/0.02 & 0.02/0.03/0.05 \\ 
& \texttt{pi.L2} & 0.00/0.00/0.01 & 0.03/0.03/0.05 \\ 
& \texttt{pi.Linf} & 0.00/0.01/0.02 & 0.01/0.02/0.03 \\ 
\midrule\multirow{12}{*}{random.polytope}
& \texttt{ell} & 0.00/0.01/0.03 & 0.00/0.03/0.07 \\ 
& \texttt{ell.L1} & 0.00/0.04/0.06 & 0.01/0.05/0.08 \\ 
& \texttt{ell.L2} & 0.00/0.02/0.05 & 0.01/0.04/0.11 \\ 
& \texttt{ell.Linf} & 0.01/0.01/0.03 & 0.00/0.01/0.04 \\ 
& \texttt{L} & 0.00/0.00/0.02 & 0.04/0.06/0.09 \\ 
& \texttt{L1} & 0.00/0.02/0.05 & 0.01/0.05/0.08 \\ 
& \texttt{L2} & 0.00/0.02/0.03 & 0.00/0.04/0.06 \\ 
& \texttt{Linf} & 0.01/0.02/0.02 & 0.03/0.06/0.08 \\ 
& \texttt{pi} & 0.00/0.01/0.03 & 0.00/0.03/0.07 \\ 
& \texttt{pi.L1} & 0.00/0.04/0.06 & 0.01/0.05/0.08 \\ 
& \texttt{pi.L2} & 0.00/0.02/0.05 & 0.01/0.04/0.11 \\ 
& \texttt{pi.Linf} & 0.01/0.01/0.03 & 0.00/0.01/0.04 \\ 
\midrule\multirow{12}{*}{simplex}
& \texttt{ell} & 0.00/0.00/0.01 & 0.00/0.02/0.08 \\ 
& \texttt{ell.L1} & 0.00/0.01/0.01 & 0.00/0.08/0.12 \\ 
& \texttt{ell.L2} & 0.00/0.00/0.01 & 0.00/0.01/0.05 \\ 
& \texttt{ell.Linf} & 0.00/0.00/0.00 & 0.00/0.03/0.03 \\ 
& \texttt{L} & 0.00/0.01/0.02 & 0.05/0.08/0.15 \\ 
& \texttt{L1} & 0.00/0.01/0.01 & 0.01/0.10/0.14 \\ 
& \texttt{L2} & 0.00/0.00/0.00 & 0.03/0.05/0.07 \\ 
& \texttt{Linf} & 0.00/0.01/0.01 & 0.02/0.05/0.07 \\ 
& \texttt{pi} & 0.00/0.00/0.01 & 0.00/0.02/0.08 \\ 
& \texttt{pi.L1} & 0.00/0.01/0.01 & 0.00/0.08/0.12 \\ 
& \texttt{pi.L2} & 0.00/0.00/0.01 & 0.00/0.01/0.05 \\ 
& \texttt{pi.Linf} & 0.00/0.00/0.00 & 0.00/0.03/0.03 \\ 
\midrule

==> arXiv submission multiple hypothesis/reject-rates-acyclic-fwer-composite-validation.tex <==
ell & 0.06/0.06/0.09  & 0.03/0.08/0.11 \\ 
ell.L1 & 0.05/0.06/0.07  & 0.03/0.08/0.10 \\ 
ell.L2 & 0.04/0.07/0.09  & 0.04/0.08/0.09 \\ 
ell.Linf & 0.01/0.04/0.07  & 0.00/0.03/0.06 \\ 
L & 0.05/0.10/0.12  & 0.05/0.08/0.10 \\ 
L1 & 0.05/0.06/0.06  & 0.04/0.07/0.12 \\ 
L2 & 0.04/0.07/0.09  & 0.04/0.08/0.10 \\ 
Linf & 0.02/0.06/0.11  & 0.02/0.04/0.06 \\ 
pi & 0.06/0.06/0.09  & 0.03/0.08/0.11 \\ 
pi.L1 & 0.05/0.06/0.07  & 0.03/0.08/0.10 \\ 
pi.L2 & 0.04/0.07/0.09  & 0.04/0.08/0.09 \\ 
pi.Linf & 0.01/0.04/0.07  & 0.00/0.03/0.06 \\ 


==> arXiv submission multiple hypothesis/reject-rates-acyclic-fwer-validation.tex <==
ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
ell.L2.1 & 0.00/0.05/0.12  & 0.03/0.12/0.17 \\ 
ell.Linf.1 & 0.05/0.09/0.15  & 0.08/0.12/0.16 \\ 
L1.0 & 0.02/0.04/0.04  & 0.00/0.05/0.12 \\ 
L1.1 & 0.03/0.05/0.07  & 0.00/0.02/0.03 \\ 
L2.0 & 0.02/0.04/0.06  & 0.02/0.05/0.08 \\ 
L2.1 & 0.01/0.02/0.07  & 0.01/0.01/0.02 \\ 
Linf.0 & 0.04/0.10/0.11  & 0.03/0.09/0.14 \\ 
Linf.1 & 0.01/0.02/0.04  & 0.01/0.03/0.06 \\ 
pi.L1.1 & 0.02/0.07/0.16  & 0.05/0.07/0.11 \\ 
pi.L2.1 & 0.02/0.07/0.14  & 0.05/0.06/0.16 \\ 
pi.Linf.1 & 0.01/0.04/0.09  & 0.01/0.06/0.12 \\ 


==> arXiv submission multiple hypothesis/reject-rates-acyclic-multiplicative-validation.tex <==
\multirow{6}{*}{axis}& \texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.L2.1} & 0.21/0.33/0.38 & 0.13/0.13/0.28 & 0.11/0.23/0.32 \\ 
& \texttt{ell.Linf.1} & 0.00/0.00/0.00 & 0.13/0.13/0.13 & 0.00/0.07/0.07 \\ 
& \texttt{pi.L1.1} & 0.11/0.23/0.56 & 0.26/0.34/0.42 & 0.11/0.26/0.41 \\ 
& \texttt{pi.L2.1} & 0.21/0.23/0.43 & 0.26/0.34/0.34 & 0.11/0.26/0.41 \\ 
& \texttt{pi.Linf.1} & 0.00/0.00/0.00 & 0.13/0.13/0.13 & 0.07/0.07/0.07 \\ 
\midrule\multirow{6}{*}{ball}& \texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.L2.1} & 0.02/0.06/0.07 & 0.03/0.08/0.11 & 0.01/0.05/0.06 \\ 
& \texttt{ell.Linf.1} & 0.00/0.00/0.08 & 0.02/0.02/0.09 & 0.00/0.03/0.04 \\ 
& \texttt{pi.L1.1} & 0.01/0.03/0.06 & 0.00/0.02/0.07 & 0.00/0.09/0.18 \\ 
& \texttt{pi.L2.1} & 0.01/0.03/0.05 & 0.00/0.01/0.07 & 0.00/0.05/0.13 \\ 
& \texttt{pi.Linf.1} & 0.00/0.02/0.09 & 0.00/0.02/0.07 & 0.01/0.06/0.08 \\ 
\midrule\multirow{6}{*}{cross}& \texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.L2.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.Linf.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{pi.L1.1} & 0.18/0.31/0.31 & 0.12/0.33/0.33 & 0.11/0.22/0.31 \\ 
& \texttt{pi.L2.1} & 0.18/0.18/0.31 & 0.12/0.24/0.36 & 0.11/0.22/0.22 \\ 
& \texttt{pi.Linf.1} & 0.00/0.00/0.00 & 0.00/0.00/0.12 & 0.00/0.00/0.21 \\ 
\midrule\multirow{6}{*}{random.hull}& \texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.L2.1} & 0.00/0.02/0.11 & 0.02/0.11/0.11 & 0.03/0.03/0.06 \\ 
& \texttt{ell.Linf.1} & 0.00/0.10/0.15 & 0.00/0.01/0.01 & 0.00/0.03/0.24 \\ 
& \texttt{pi.L1.1} & 0.16/0.16/0.16 & 0.18/0.19/0.20 & 0.14/0.14/0.14 \\ 
& \texttt{pi.L2.1} & 0.16/0.16/0.16 & 0.18/0.19/0.20 & 0.14/0.14/0.14 \\ 
& \texttt{pi.Linf.1} & 0.11/0.19/0.20 & 0.04/0.10/0.21 & 0.09/0.15/0.20 \\ 
\midrule\multirow{6}{*}{random.polytope}& \texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.L2.1} & 0.03/0.09/0.15 & 0.02/0.05/0.12 & 0.01/0.01/0.08 \\ 
& \texttt{ell.Linf.1} & 0.00/0.00/0.04 & 0.00/0.00/0.06 & 0.00/0.00/0.02 \\ 
& \texttt{pi.L1.1} & 0.01/0.09/0.13 & 0.07/0.09/0.11 & 0.02/0.06/0.11 \\ 
& \texttt{pi.L2.1} & 0.01/0.09/0.15 & 0.04/0.06/0.11 & 0.01/0.07/0.11 \\ 
& \texttt{pi.Linf.1} & 0.00/0.02/0.02 & 0.00/0.00/0.08 & 0.00/0.06/0.11 \\ 
\midrule\multirow{6}{*}{simplex}& \texttt{ell.L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
& \texttt{ell.L2.1} & 0.01/0.01/0.07 & 0.01/0.03/0.09 & 0.05/0.07/0.14 \\ 
& \texttt{ell.Linf.1} & 0.01/0.01/0.05 & 0.02/0.02/0.02 & 0.00/0.04/0.09 \\ 
& \texttt{pi.L1.1} & 0.02/0.03/0.05 & 0.01/0.02/0.06 & 0.00/0.05/0.07 \\ 
& \texttt{pi.L2.1} & 0.01/0.02/0.07 & 0.01/0.02/0.07 & 0.00/0.05/0.07 \\ 
& \texttt{pi.Linf.1} & 0.01/0.03/0.03 & 0.00/0.00/0.02 & 0.01/0.05/0.05 \\ 
\midrule

==> arXiv submission multiple hypothesis/reject-rates-power-fig8.tex <==
\multirow{9}{*}{axis} & \multirow{3}{*}{L1} & 0.01 & 0.80/0.87/0.97  & 0.80/0.80/0.80  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & & 0.05 & 0.20/0.20/0.20  & 0.20/0.27/0.38  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & & 0.1 & 0.20/0.35/0.40  & 0.00/0.12/0.20  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{L2} & 0.01 & 0.82/0.99/1.00  & 0.80/0.80/0.80  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & & 0.05 & 0.20/0.20/0.21  & 0.60/0.60/0.60  & 0.41/0.53/0.71  & 0.80/0.80/0.80 \\ 
 & & 0.1 & 0.20/0.35/0.40  & 0.02/0.19/0.25  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{Linf} & 0.01 & 0.26/0.60/0.62  & 0.80/0.80/0.80  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & & 0.05 & 0.02/0.02/0.02  & 0.43/0.59/0.60  & 0.49/0.98/1.00  & 1.00/1.00/1.00 \\ 
 & & 0.1 & 0.40/0.40/0.40  & 0.00/0.27/0.60  & 0.00/0.16/0.37  & 0.40/0.41/0.48 \\ 
 \cmidrule(lr){2-7}\midrule
\multirow{9}{*}{unbiased.hull} & \multirow{3}{*}{L1} & 0.01 & 0.62/0.79/0.80  & 0.60/0.74/0.80  & 0.83/0.99/1.00  & 0.00/0.00/0.00 \\ 
 & & 0.05 & 0.20/0.20/0.22  & 0.40/0.46/0.59  & 0.00/0.05/0.19  & 0.00/0.00/0.00 \\ 
 & & 0.1 & 0.20/0.23/0.35  & 0.00/0.12/0.20  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{L2} & 0.01 & 0.80/0.80/0.91  & 0.80/0.80/0.80  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & & 0.05 & 0.20/0.20/0.30  & 0.60/0.60/0.60  & 0.63/0.78/0.80  & 1.00/1.00/1.00 \\ 
 & & 0.1 & 0.20/0.26/0.38  & 0.40/0.40/0.40  & 0.00/0.00/0.10  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{Linf} & 0.01 & 0.40/0.47/0.58  & 0.80/0.80/0.80  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & & 0.05 & 0.20/0.23/0.35  & 0.60/0.60/0.64  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & & 0.1 & 0.06/0.21/0.22  & 0.24/0.52/0.66  & 0.40/0.56/0.63  & 0.42/0.60/0.66 \\ 
 \cmidrule(lr){2-7}

==> arXiv submission multiple hypothesis/reject-rates-power-fwer-composite.tex <==
\multirow{12}{*}{concentric} & ell & 0.48/0.53/0.60  & 0.42/0.55/0.57 \\ 
 & ell.L1 & 0.18/0.29/0.33  & 0.13/0.22/0.26 \\ 
 & ell.L2 & 0.44/0.49/0.54  & 0.43/0.50/0.55 \\ 
 & ell.Linf & 0.45/0.51/0.53  & 0.45/0.51/0.54 \\ 
 & L & 0.48/0.55/0.58  & 0.47/0.61/0.61 \\ 
 & L1 & 0.17/0.28/0.32  & 0.13/0.22/0.26 \\ 
 & L2 & 0.44/0.50/0.54  & 0.42/0.49/0.55 \\ 
 & Linf & 0.46/0.50/0.54  & 0.49/0.59/0.61 \\ 
 & pi & 0.48/0.53/0.60  & 0.42/0.55/0.57 \\ 
 & pi.L1 & 0.18/0.29/0.33  & 0.13/0.22/0.26 \\ 
 & pi.L2 & 0.44/0.49/0.54  & 0.43/0.50/0.55 \\ 
 & pi.Linf & 0.45/0.51/0.53  & 0.45/0.51/0.54 \\ 
\midrule
\multirow{12}{*}{fig8} & ell & 0.63/0.66/0.68  & 0.63/0.65/0.69 \\ 
 & ell.L1 & 0.36/0.42/0.44  & 0.35/0.41/0.45 \\ 
 & ell.L2 & 0.54/0.60/0.65  & 0.57/0.64/0.66 \\ 
 & ell.Linf & 0.57/0.59/0.62  & 0.55/0.61/0.68 \\ 
 & L & 0.60/0.65/0.67  & 0.62/0.66/0.68 \\ 
 & L1 & 0.36/0.41/0.43  & 0.34/0.40/0.45 \\ 
 & L2 & 0.53/0.59/0.64  & 0.57/0.62/0.65 \\ 
 & Linf & 0.54/0.58/0.62  & 0.53/0.61/0.63 \\ 
 & pi & 0.63/0.66/0.68  & 0.63/0.65/0.69 \\ 
 & pi.L1 & 0.36/0.42/0.44  & 0.35/0.41/0.45 \\ 
 & pi.L2 & 0.54/0.60/0.65  & 0.57/0.64/0.66 \\ 
 & pi.Linf & 0.57/0.59/0.62  & 0.55/0.61/0.68 \\ 
\midrule
\multirow{12}{*}{sphere} & ell & 0.26/0.32/0.35  & 0.26/0.28/0.31 \\ 
 & ell.L1 & 0.13/0.14/0.19  & 0.08/0.11/0.15 \\ 
 & ell.L2 & 0.21/0.24/0.30  & 0.23/0.25/0.29 \\ 
 & ell.Linf & 0.25/0.32/0.36  & 0.21/0.25/0.37 \\ 
 & L & 0.24/0.32/0.38  & 0.30/0.39/0.40 \\ 
 & L1 & 0.12/0.14/0.18  & 0.08/0.11/0.16 \\ 
 & L2 & 0.20/0.25/0.29  & 0.23/0.25/0.30 \\ 
 & Linf & 0.23/0.31/0.40  & 0.27/0.35/0.39 \\ 
 & pi & 0.26/0.32/0.35  & 0.26/0.28/0.31 \\ 
 & pi.L1 & 0.13/0.14/0.19  & 0.08/0.11/0.15 \\ 
 & pi.L2 & 0.21/0.24/0.30  & 0.23/0.25/0.29 \\ 
 & pi.Linf & 0.25/0.32/0.36  & 0.21/0.25/0.37 \\ 
\midrule
\multirow{12}{*}{thomas} & ell & 0.10/0.17/0.20  & 0.10/0.16/0.18 \\ 
 & ell.L1 & 0.04/0.08/0.16  & 0.04/0.08/0.11 \\ 
 & ell.L2 & 0.07/0.10/0.13  & 0.09/0.11/0.11 \\ 
 & ell.Linf & 0.12/0.16/0.20  & 0.13/0.17/0.21 \\ 
 & L & 0.56/0.63/0.67  & 0.60/0.64/0.66 \\ 
 & L1 & 0.22/0.24/0.30  & 0.21/0.27/0.32 \\ 
 & L2 & 0.34/0.40/0.42  & 0.36/0.38/0.42 \\ 
 & Linf & 0.47/0.53/0.55  & 0.53/0.59/0.62 \\ 
 & pi & 0.10/0.17/0.20  & 0.10/0.16/0.18 \\ 
 & pi.L1 & 0.04/0.08/0.16  & 0.04/0.08/0.11 \\ 
 & pi.L2 & 0.07/0.10/0.13  & 0.09/0.11/0.11 \\ 
 & pi.Linf & 0.12/0.16/0.20  & 0.13/0.17/0.21 \\ 


==> arXiv submission multiple hypothesis/reject-rates-power-fwer-noise.tex <==
\multirow{12}{*}{0.01} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.07/0.17/0.19  & 0.06/0.14/0.19 \\ 
 & ell.Linf.1 & 0.43/0.51/0.53  & 0.41/0.44/0.51 \\ 
 & L1.0 & 0.00/0.02/0.04  & 0.03/0.06/0.10 \\ 
 & L1.1 & 0.47/0.54/0.55  & 0.41/0.50/0.54 \\ 
 & L2.0 & 0.01/0.02/0.03  & 0.03/0.04/0.08 \\ 
 & L2.1 & 0.76/0.78/0.79  & 0.73/0.75/0.78 \\ 
 & Linf.0 & 0.27/0.31/0.33  & 0.22/0.28/0.31 \\ 
 & Linf.1 & 0.73/0.78/0.79  & 0.70/0.74/0.74 \\ 
 & pi.L1.1 & 0.43/0.53/0.62  & 0.44/0.55/0.62 \\ 
 & pi.L2.1 & 0.63/0.67/0.74  & 0.66/0.69/0.74 \\ 
 & pi.Linf.1 & 0.59/0.65/0.71  & 0.64/0.68/0.69 \\ 
\midrule
\multirow{12}{*}{0.05} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.11/0.15  & 0.05/0.11/0.16 \\ 
 & ell.Linf.1 & 0.32/0.42/0.49  & 0.33/0.45/0.48 \\ 
 & L1.0 & 0.00/0.04/0.05  & 0.03/0.09/0.09 \\ 
 & L1.1 & 0.20/0.31/0.34  & 0.17/0.27/0.32 \\ 
 & L2.0 & 0.01/0.05/0.06  & 0.02/0.05/0.08 \\ 
 & L2.1 & 0.47/0.59/0.63  & 0.53/0.60/0.65 \\ 
 & Linf.0 & 0.21/0.26/0.30  & 0.26/0.30/0.34 \\ 
 & Linf.1 & 0.50/0.60/0.64  & 0.52/0.57/0.62 \\ 
 & pi.L1.1 & 0.14/0.26/0.36  & 0.15/0.30/0.35 \\ 
 & pi.L2.1 & 0.26/0.44/0.50  & 0.26/0.43/0.48 \\ 
 & pi.Linf.1 & 0.43/0.49/0.61  & 0.40/0.50/0.60 \\ 
\midrule
\multirow{12}{*}{0.1} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.06/0.08/0.18  & 0.06/0.11/0.20 \\ 
 & ell.Linf.1 & 0.24/0.32/0.35  & 0.23/0.31/0.40 \\ 
 & L1.0 & 0.01/0.04/0.04  & 0.05/0.10/0.11 \\ 
 & L1.1 & 0.18/0.20/0.28  & 0.16/0.22/0.27 \\ 
 & L2.0 & 0.02/0.05/0.05  & 0.03/0.05/0.08 \\ 
 & L2.1 & 0.32/0.35/0.37  & 0.27/0.37/0.41 \\ 
 & Linf.0 & 0.23/0.28/0.32  & 0.22/0.30/0.39 \\ 
 & Linf.1 & 0.35/0.40/0.40  & 0.35/0.43/0.47 \\ 
 & pi.L1.1 & 0.14/0.21/0.25  & 0.15/0.22/0.25 \\ 
 & pi.L2.1 & 0.21/0.27/0.30  & 0.18/0.27/0.34 \\ 
 & pi.Linf.1 & 0.35/0.45/0.49  & 0.36/0.45/0.51 \\ 


==> arXiv submission multiple hypothesis/reject-rates-power-fwer.tex <==
\multirow{12}{*}{concentric} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.15/0.21  & 0.09/0.14/0.22 \\ 
 & ell.Linf.1 & 0.36/0.43/0.50  & 0.31/0.41/0.47 \\ 
 & L1.0 & 0.02/0.04/0.06  & 0.03/0.05/0.08 \\ 
 & L1.1 & 0.23/0.24/0.29  & 0.17/0.29/0.31 \\ 
 & L2.0 & 0.02/0.09/0.10  & 0.02/0.04/0.07 \\ 
 & L2.1 & 0.44/0.49/0.51  & 0.44/0.48/0.52 \\ 
 & Linf.0 & 0.29/0.33/0.38  & 0.29/0.34/0.35 \\ 
 & Linf.1 & 0.47/0.52/0.57  & 0.44/0.47/0.54 \\ 
 & pi.L1.1 & 0.18/0.25/0.30  & 0.18/0.31/0.37 \\ 
 & pi.L2.1 & 0.30/0.34/0.41  & 0.27/0.37/0.42 \\ 
 & pi.Linf.1 & 0.42/0.48/0.50  & 0.40/0.46/0.51 \\ 
\midrule
\multirow{12}{*}{fig8} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.03/0.10/0.14  & 0.04/0.10/0.15 \\ 
 & ell.Linf.1 & 0.32/0.34/0.37  & 0.28/0.36/0.38 \\ 
 & L1.0 & 0.03/0.05/0.06  & 0.01/0.01/0.01 \\ 
 & L1.1 & 0.42/0.45/0.49  & 0.38/0.42/0.46 \\ 
 & L2.0 & 0.03/0.06/0.07  & 0.01/0.03/0.04 \\ 
 & L2.1 & 0.54/0.62/0.66  & 0.55/0.60/0.64 \\ 
 & Linf.0 & 0.04/0.16/0.23  & 0.14/0.22/0.27 \\ 
 & Linf.1 & 0.59/0.64/0.66  & 0.60/0.65/0.65 \\ 
 & pi.L1.1 & 0.36/0.44/0.53  & 0.38/0.47/0.56 \\ 
 & pi.L2.1 & 0.39/0.51/0.59  & 0.46/0.54/0.63 \\ 
 & pi.Linf.1 & 0.53/0.58/0.60  & 0.54/0.58/0.64 \\ 
\midrule
\multirow{12}{*}{sphere} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.06/0.14/0.18  & 0.04/0.16/0.27 \\ 
 & ell.Linf.1 & 0.19/0.29/0.35  & 0.22/0.31/0.34 \\ 
 & L1.0 & 0.00/0.01/0.02  & 0.06/0.09/0.11 \\ 
 & L1.1 & 0.16/0.19/0.24  & 0.13/0.15/0.20 \\ 
 & L2.0 & 0.01/0.04/0.05  & 0.03/0.05/0.12 \\ 
 & L2.1 & 0.27/0.32/0.36  & 0.26/0.29/0.30 \\ 
 & Linf.0 & 0.08/0.16/0.19  & 0.15/0.18/0.20 \\ 
 & Linf.1 & 0.28/0.32/0.35  & 0.27/0.34/0.36 \\ 
 & pi.L1.1 & 0.16/0.26/0.33  & 0.18/0.28/0.35 \\ 
 & pi.L2.1 & 0.28/0.34/0.40  & 0.25/0.36/0.42 \\ 
 & pi.Linf.1 & 0.30/0.36/0.42  & 0.29/0.40/0.46 \\ 
\midrule
\multirow{12}{*}{thomas} & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.04/0.10  & 0.04/0.08/0.14 \\ 
 & ell.Linf.1 & 0.01/0.05/0.14  & 0.05/0.14/0.17 \\ 
 & L1.0 & 0.18/0.21/0.21  & 0.25/0.29/0.33 \\ 
 & L1.1 & 0.07/0.13/0.16  & 0.07/0.07/0.10 \\ 
 & L2.0 & 0.34/0.35/0.38  & 0.45/0.47/0.48 \\ 
 & L2.1 & 0.07/0.11/0.14  & 0.08/0.09/0.11 \\ 
 & Linf.0 & 0.40/0.47/0.51  & 0.47/0.51/0.57 \\ 
 & Linf.1 & 0.07/0.09/0.12  & 0.05/0.10/0.13 \\ 
 & pi.L1.1 & 0.04/0.08/0.17  & 0.03/0.11/0.17 \\ 
 & pi.L2.1 & 0.04/0.10/0.19  & 0.03/0.09/0.18 \\ 
 & pi.Linf.1 & 0.07/0.14/0.21  & 0.07/0.16/0.22 \\ 


==> arXiv submission multiple hypothesis/reject-rates-power-models-estimator-noise.tex <==
\multirow{9}{*}{axis} & \multirow{3}{*}{L1} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{L2} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{Linf} & 0.01 & 0.57/0.97/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7}\midrule
\multirow{9}{*}{unbiased.hull} & \multirow{3}{*}{L1} & 0.01 & 1.00/1.00/1.00  & 0.55/0.98/1.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{L2} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{Linf} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7}

==> arXiv submission multiple hypothesis/reject-rates-power-models-size.tex <==
\texttt{L1.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 0.57/0.97/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L1.1} & 1.00/1.00/1.00 & 0.55/0.98/1.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L1.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 


==> long-table.tex <==
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1,0.1)}} & ell.L1 & 0.07/0.17/0.22  & 0.18/0.38/0.43  & 0.00/0.05/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.12/0.25/0.27  & 0.00/0.32/0.48  & 0.00/0.05/0.08 \\ 
 & ell.L2.1 & 0.00/0.02/0.10  & 0.00/0.00/0.07  & 0.00/0.05/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.13  & 0.05/0.25/0.42  & 0.00/0.03/0.05 \\ 
 & ell.Linf.1 & 0.00/0.03/0.10  & 0.00/0.00/0.08  & 0.05/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.17/0.22  & 1.00/1.00/1.00  & 0.00/0.03/0.08 \\ 
 & L1.0 & 0.02/0.05/0.17  & 1.00/1.00/1.00  & 0.00/0.08/0.15 \\ 
 & L1.1 & 0.07/0.17/0.22  & 0.18/0.38/0.43  & 0.00/0.05/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.12/0.23/0.28  & 1.00/1.00/1.00  & 0.00/0.00/0.05 \\ 
 & L2.0 & 0.02/0.03/0.12  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.12/0.25/0.27  & 0.00/0.32/0.48  & 0.00/0.05/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.05  & 0.27/0.50/0.68  & 0.00/0.02/0.05 \\ 
 & Linf.0 & 0.00/0.03/0.12  & 0.28/0.57/0.68  & 0.00/0.00/0.08 \\ 
 & Linf.1 & 0.00/0.02/0.13  & 0.05/0.25/0.42  & 0.00/0.03/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.07/0.17/0.22  & 0.18/0.38/0.43  & 0.00/0.05/0.12 \\ 
 & pi.L1.1 & 0.07/0.18/0.30  & 0.02/0.15/0.28  & 0.05/0.15/0.25 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.12/0.25/0.27  & 0.00/0.32/0.48  & 0.00/0.05/0.08 \\ 
 & pi.L2.1 & 0.10/0.15/0.25  & 0.00/0.10/0.27  & 0.05/0.17/0.25 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.13  & 0.05/0.25/0.42  & 0.00/0.03/0.05 \\ 
 & pi.Linf.1 & 0.00/0.05/0.15  & 0.00/0.02/0.08  & 0.00/0.05/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1,1)}} & ell.L1 & 0.00/0.05/0.15  & 0.10/0.17/0.30  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.07/0.18  & 0.05/0.22/0.35  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.02/0.03 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.02/0.07  & 0.95/0.97/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.03  & 0.95/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.05/0.15  & 0.10/0.17/0.30  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.10  & 0.92/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.02/0.05  & 0.95/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.07/0.18  & 0.05/0.22/0.35  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.15/0.15  & 0.02/0.12/0.18  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.05/0.17/0.20  & 0.02/0.13/0.22  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.05/0.15  & 0.10/0.17/0.30  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.10  & 0.00/0.00/0.03  & 0.00/0.00/0.03 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.07/0.18  & 0.05/0.22/0.35  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.02/0.10  & 0.00/0.00/0.03  & 0.00/0.00/0.03 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.13  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.05/0.08  & 0.05/0.05/0.05  & 0.05/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.03/0.05  & 0.00/0.02/0.03  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.02/0.07  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.82/0.97/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.05/0.13  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.07  & 0.33/0.38/0.55  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.05/0.08/0.10  & 0.40/0.40/0.58  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.07/0.13  & 0.00/0.07/0.12  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.05/0.05/0.12  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.02/0.03/0.05  & 0.00/0.02/0.03  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.13  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.03/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.07  & 0.00/0.03/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.03/0.05  & 0.00/0.02/0.03  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.02/0.05/0.05  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,0.1)}} & ell.L1 & 0.00/0.03/0.12  & 0.05/0.10/0.18  & 0.05/0.07/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.05/0.08  & 0.10/0.17/0.18  & 0.00/0.13/0.15 \\ 
 & ell.L2.1 & 0.00/0.00/0.12  & 0.00/0.02/0.12  & 0.10/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.03/0.10 \\ 
 & ell.Linf.1 & 0.05/0.08/0.15  & 0.00/0.02/0.13  & 0.10/0.12/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.03/0.05  & 0.40/0.70/0.82  & 0.05/0.10/0.22 \\ 
 & L1.0 & 0.00/0.00/0.12  & 0.70/0.83/0.90  & 0.05/0.17/0.28 \\ 
 & L1.1 & 0.00/0.03/0.12  & 0.05/0.10/0.18  & 0.05/0.07/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.07/0.10  & 0.45/0.83/0.88  & 0.00/0.10/0.23 \\ 
 & L2.0 & 0.00/0.05/0.08  & 0.85/0.85/0.87  & 0.02/0.10/0.15 \\ 
 & L2.1 & 0.00/0.05/0.08  & 0.10/0.17/0.18  & 0.00/0.13/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.05/0.08  & 0.05/0.10/0.13  & 0.03/0.05/0.07 \\ 
 & Linf.0 & 0.05/0.05/0.10  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & Linf.1 & 0.00/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.03/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.12  & 0.05/0.10/0.18  & 0.05/0.07/0.12 \\ 
 & pi.L1.1 & 0.00/0.03/0.08  & 0.00/0.05/0.08  & 0.00/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.05/0.08  & 0.10/0.17/0.18  & 0.00/0.13/0.15 \\ 
 & pi.L2.1 & 0.00/0.03/0.08  & 0.00/0.07/0.10  & 0.00/0.02/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.03/0.10 \\ 
 & pi.Linf.1 & 0.00/0.00/0.10  & 0.00/0.03/0.07  & 0.00/0.00/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,1,1)}} & ell.L1 & 0.00/0.03/0.15  & 0.05/0.15/0.23  & 0.00/0.00/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.13  & 0.07/0.12/0.15  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.08/0.12  & 0.00/0.03/0.17  & 0.07/0.17/0.20 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.02  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.03/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.07/0.12  & 0.97/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L1.0 & 0.05/0.08/0.17  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.03/0.15  & 0.05/0.15/0.23  & 0.00/0.00/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.05/0.15  & 0.97/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.07/0.15/0.18  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.02/0.13  & 0.07/0.12/0.15  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.08/0.10  & 0.05/0.27/0.35  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.02/0.12/0.15  & 0.03/0.25/0.38  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.02  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.15  & 0.05/0.15/0.23  & 0.00/0.00/0.05 \\ 
 & pi.L1.1 & 0.00/0.03/0.08  & 0.05/0.07/0.12  & 0.05/0.12/0.23 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.13  & 0.07/0.12/0.15  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.02/0.13  & 0.05/0.08/0.13  & 0.05/0.18/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.02  & 0.02/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.00  & 0.00/0.02/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,1,10)}} & ell.L1 & 0.00/0.00/0.02  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.02  & 0.02/0.10/0.15  & 0.02/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.02  & 0.00/0.00/0.07  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.12/0.15  & 0.03/0.15/0.25  & 0.02/0.05/0.05 \\ 
 & ell.Linf.1 & 0.00/0.03/0.05  & 0.02/0.05/0.05  & 0.00/0.02/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.78/1.00/1.00  & 0.00/0.03/0.05 \\ 
 & L1.0 & 0.00/0.00/0.08  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.05/0.07  & 0.65/0.92/0.98  & 0.02/0.05/0.05 \\ 
 & L2.0 & 0.00/0.07/0.12  & 0.80/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.02  & 0.02/0.10/0.15  & 0.02/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.12/0.27  & 0.02/0.10/0.30  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.02/0.15/0.28  & 0.02/0.08/0.20  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.12/0.15  & 0.03/0.15/0.25  & 0.02/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.02  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.20/0.30/0.37 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.02  & 0.02/0.10/0.15  & 0.02/0.05/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.20/0.30/0.37 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.12/0.15  & 0.03/0.15/0.25  & 0.02/0.05/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.03/0.08  & 0.05/0.10/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,1)}} & ell.L1 & 0.00/0.02/0.10  & 0.05/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.12  & 0.05/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & ell.L2.1 & 0.00/0.03/0.17  & 0.02/0.05/0.12  & 0.00/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.02/0.02/0.05  & 0.05/0.05/0.08 \\ 
 & ell.Linf.1 & 0.00/0.05/0.10  & 0.00/0.05/0.08  & 0.00/0.07/0.15 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.07/0.13  & 0.27/0.62/0.83  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.02/0.10/0.17  & 0.50/0.85/0.88  & 0.05/0.05/0.05 \\ 
 & L1.1 & 0.00/0.02/0.10  & 0.05/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.07/0.13/0.18  & 0.18/0.45/0.57  & 0.05/0.05/0.05 \\ 
 & L2.0 & 0.10/0.15/0.15  & 0.33/0.58/0.65  & 0.05/0.05/0.05 \\ 
 & L2.1 & 0.00/0.02/0.12  & 0.05/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.10/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & Linf.0 & 0.05/0.10/0.10  & 0.10/0.10/0.10  & 0.00/0.10/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.02/0.02/0.05  & 0.05/0.05/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.10  & 0.05/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & pi.L1.1 & 0.00/0.03/0.13  & 0.05/0.05/0.05  & 0.00/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.12  & 0.05/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & pi.L2.1 & 0.00/0.03/0.13  & 0.05/0.05/0.07  & 0.00/0.07/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.02/0.02/0.05  & 0.05/0.05/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.03  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,10,10)}} & ell.L1 & 0.10/0.10/0.13  & 0.17/0.30/0.38  & 0.05/0.07/0.20 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.15/0.15/0.18  & 0.12/0.20/0.33  & 0.07/0.15/0.18 \\ 
 & ell.L2.1 & 0.05/0.05/0.07  & 0.05/0.08/0.12  & 0.05/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.08/0.10  & 0.05/0.12/0.20  & 0.00/0.00/0.08 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.05/0.05/0.05  & 0.02/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.15/0.23/0.25  & 0.93/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.10/0.17/0.20  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.10/0.13  & 0.17/0.30/0.38  & 0.05/0.07/0.20 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.17/0.25/0.25  & 0.87/0.97/0.98  & 0.00/0.10/0.15 \\ 
 & L2.0 & 0.10/0.17/0.23  & 0.95/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.15/0.15/0.18  & 0.12/0.20/0.33  & 0.07/0.15/0.18 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.07/0.17/0.20  & 0.17/0.25/0.43  & 0.00/0.03/0.12 \\ 
 & Linf.0 & 0.15/0.15/0.20  & 0.13/0.25/0.42  & 0.02/0.07/0.12 \\ 
 & Linf.1 & 0.02/0.08/0.10  & 0.05/0.12/0.20  & 0.00/0.00/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.10/0.13  & 0.17/0.30/0.38  & 0.05/0.07/0.20 \\ 
 & pi.L1.1 & 0.10/0.10/0.15  & 0.05/0.08/0.17  & 0.12/0.23/0.45 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.15/0.15/0.18  & 0.12/0.20/0.33  & 0.07/0.15/0.18 \\ 
 & pi.L2.1 & 0.10/0.10/0.12  & 0.05/0.10/0.15  & 0.12/0.23/0.42 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.08/0.10  & 0.05/0.12/0.20  & 0.00/0.00/0.08 \\ 
 & pi.Linf.1 & 0.02/0.10/0.10  & 0.05/0.05/0.12  & 0.05/0.10/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(0.1,10)}} & ell.L1 & 0.02/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.02/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.02/0.02/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.02/0.05  & 0.00/0.02/0.05  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.03/0.05  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.05/0.07  & 0.55/0.65/0.77  & 0.00/0.00/0.02 \\ 
 & L1.0 & 0.00/0.02/0.03  & 0.52/0.68/0.80  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.02/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.02/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.07/0.07/0.15  & 0.10/0.17/0.25  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.05/0.05/0.10  & 0.05/0.15/0.20  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.02/0.02/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.13/0.22  & 0.00/0.12/0.18  & 0.00/0.02/0.10 \\ 
 & Linf.0 & 0.05/0.13/0.18  & 0.00/0.12/0.18  & 0.00/0.03/0.10 \\ 
 & Linf.1 & 0.00/0.03/0.05  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.02/0.05/0.10  & 0.05/0.07/0.10  & 0.00/0.02/0.05 \\ 
 & pi.L1.1 & 0.00/0.03/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.02/0.02/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.03/0.10  & 0.05/0.05/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.03/0.05  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,1,1)}} & ell.L1 & 0.02/0.07/0.10  & 0.05/0.22/0.32  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.02/0.07/0.12  & 0.15/0.27/0.38  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.05/0.05/0.05  & 0.00/0.05/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.10/0.12  & 0.10/0.25/0.45  & 0.00/0.05/0.05 \\ 
 & ell.Linf.1 & 0.05/0.05/0.12  & 0.05/0.12/0.15  & 0.05/0.08/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.05/0.07  & 1.00/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L1.0 & 0.00/0.03/0.07  & 1.00/1.00/1.00  & 0.02/0.05/0.05 \\ 
 & L1.1 & 0.02/0.07/0.10  & 0.05/0.22/0.32  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.05/0.08  & 1.00/1.00/1.00  & 0.00/0.00/0.02 \\ 
 & L2.0 & 0.00/0.00/0.02  & 1.00/1.00/1.00  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.02/0.07/0.12  & 0.15/0.27/0.38  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.07/0.13  & 0.23/0.45/0.57  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.05/0.08/0.15  & 0.22/0.40/0.53  & 0.00/0.05/0.05 \\ 
 & Linf.1 & 0.00/0.10/0.12  & 0.10/0.25/0.45  & 0.00/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.02/0.07/0.10  & 0.05/0.22/0.32  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.02/0.05/0.10  & 0.05/0.05/0.05  & 0.00/0.05/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.02/0.07/0.12  & 0.15/0.27/0.38  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.02/0.05/0.12  & 0.05/0.05/0.05  & 0.00/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.10/0.12  & 0.10/0.25/0.45  & 0.00/0.05/0.05 \\ 
 & pi.Linf.1 & 0.05/0.05/0.08  & 0.00/0.10/0.20  & 0.05/0.05/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,1,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.08/0.18  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.00/0.00/0.03  & 0.00/0.00/0.02 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.10/0.15  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.03  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.93/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.05  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.05  & 0.78/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.03/0.07  & 0.85/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.08/0.18  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.10/0.20  & 0.05/0.08/0.22  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.08/0.15  & 0.05/0.10/0.17  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.02/0.10/0.15  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.08/0.18  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.10/0.15  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.02/0.05  & 0.00/0.00/0.03  & 0.00/0.00/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,1)}} & ell.L1 & 0.00/0.00/0.02  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.08/0.12  & 0.00/0.05/0.10  & 0.02/0.08/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.13  & 0.00/0.00/0.08 \\ 
 & ell.Linf.1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 0.62/0.77/0.90  & 0.00/0.08/0.13 \\ 
 & L1.0 & 0.00/0.05/0.10  & 0.70/0.88/0.92  & 0.05/0.12/0.32 \\ 
 & L1.1 & 0.00/0.00/0.02  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.48/0.72/0.83  & 0.00/0.03/0.12 \\ 
 & L2.0 & 0.00/0.02/0.05  & 0.70/0.85/0.88  & 0.05/0.17/0.20 \\ 
 & L2.1 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.08/0.13/0.15  & 0.20/0.22/0.35  & 0.07/0.20/0.22 \\ 
 & Linf.0 & 0.10/0.13/0.18  & 0.22/0.33/0.43  & 0.07/0.23/0.25 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.00/0.05/0.13  & 0.00/0.00/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.02  & 0.00/0.05/0.10  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.03  & 0.00/0.03/0.13  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.13  & 0.00/0.00/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,10,10)}} & ell.L1 & 0.05/0.05/0.05  & 0.05/0.08/0.13  & 0.05/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.05/0.15/0.20  & 0.05/0.05/0.05 \\ 
 & ell.L2.1 & 0.02/0.05/0.12  & 0.05/0.05/0.07  & 0.05/0.08/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.10/0.10  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & ell.Linf.1 & 0.00/0.00/0.05  & 0.05/0.05/0.08  & 0.00/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.07  & 1.00/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.02/0.08  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.05/0.08/0.13  & 0.05/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.08  & 0.95/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L2.0 & 0.00/0.02/0.10  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.05/0.15/0.20  & 0.05/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.05/0.10  & 0.17/0.20/0.27  & 0.00/0.02/0.05 \\ 
 & Linf.0 & 0.00/0.02/0.12  & 0.13/0.18/0.32  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.02/0.10/0.10  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.05/0.08/0.13  & 0.05/0.05/0.05 \\ 
 & pi.L1.1 & 0.02/0.02/0.07  & 0.00/0.05/0.07  & 0.10/0.17/0.20 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.05/0.15/0.20  & 0.05/0.05/0.05 \\ 
 & pi.L2.1 & 0.02/0.02/0.07  & 0.00/0.02/0.08  & 0.10/0.15/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.10/0.10  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & pi.Linf.1 & 0.05/0.05/0.08  & 0.00/0.00/0.07  & 0.05/0.08/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(1,10)}} & ell.L1 & 0.00/0.02/0.08  & 0.00/0.08/0.20  & 0.02/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.05/0.08  & 0.00/0.13/0.17  & 0.00/0.02/0.12 \\ 
 & ell.L2.1 & 0.05/0.15/0.20  & 0.00/0.13/0.20  & 0.10/0.13/0.25 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & ell.Linf.1 & 0.17/0.20/0.25  & 0.00/0.05/0.17  & 0.17/0.20/0.22 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.05  & 0.38/0.55/0.72  & 0.02/0.08/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.55/0.72/0.88  & 0.05/0.08/0.10 \\ 
 & L1.1 & 0.00/0.02/0.08  & 0.00/0.08/0.20  & 0.02/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.03/0.07  & 0.18/0.50/0.62  & 0.00/0.02/0.05 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.37/0.60/0.77  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.00/0.05/0.08  & 0.00/0.13/0.17  & 0.00/0.02/0.12 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.07/0.13  & 0.08/0.12/0.17  & 0.00/0.03/0.08 \\ 
 & Linf.0 & 0.00/0.02/0.10  & 0.00/0.02/0.12  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.05/0.05/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.08  & 0.00/0.08/0.20  & 0.02/0.05/0.07 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.07/0.15  & 0.05/0.10/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.05/0.08  & 0.00/0.13/0.17  & 0.00/0.02/0.12 \\ 
 & pi.L2.1 & 0.00/0.02/0.07  & 0.00/0.03/0.18  & 0.05/0.10/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.10  & 0.10/0.12/0.12  & 0.05/0.10/0.15 \\ 
 & pi.Linf.1 & 0.05/0.05/0.07  & 0.00/0.03/0.12  & 0.02/0.05/0.08 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(10,10,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.17/0.32  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.05  & 0.07/0.23/0.40  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.12/0.17  & 0.05/0.08/0.17  & 0.07/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.03/0.18  & 0.12/0.30/0.48  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.05/0.10/0.13  & 0.05/0.08/0.13  & 0.05/0.10/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.05/0.05  & 0.97/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.05/0.07/0.10  & 1.00/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.17/0.32  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.07  & 0.98/1.00/1.00  & 0.02/0.03/0.05 \\ 
 & L2.0 & 0.00/0.02/0.05  & 1.00/1.00/1.00  & 0.02/0.05/0.05 \\ 
 & L2.1 & 0.00/0.02/0.05  & 0.07/0.23/0.40  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.08/0.12  & 0.12/0.48/0.65  & 0.02/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.05/0.07  & 0.22/0.38/0.57  & 0.05/0.05/0.05 \\ 
 & Linf.1 & 0.00/0.03/0.18  & 0.12/0.30/0.48  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.17/0.32  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.07  & 0.00/0.03/0.05  & 0.00/0.07/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.05  & 0.07/0.23/0.40  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.03/0.08  & 0.00/0.03/0.05  & 0.00/0.05/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.03/0.18  & 0.12/0.30/0.48  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.00/0.02/0.07  & 0.00/0.08/0.10  & 0.00/0.05/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.axis(10,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.08/0.18  & 0.00/0.08/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.12  & 0.07/0.17/0.25  & 0.02/0.13/0.25 \\ 
 & ell.L2.1 & 0.05/0.08/0.15  & 0.05/0.13/0.20  & 0.12/0.15/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.07/0.20/0.33  & 0.13/0.25/0.35  & 0.07/0.20/0.30 \\ 
 & ell.Linf.1 & 0.07/0.15/0.15  & 0.05/0.12/0.22  & 0.00/0.08/0.18 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.30/0.53/0.73  & 0.00/0.08/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.55/0.77/0.87  & 0.05/0.05/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.08/0.18  & 0.00/0.08/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.38/0.62/0.78  & 0.00/0.12/0.17 \\ 
 & L2.0 & 0.00/0.00/0.07  & 0.70/0.78/0.83  & 0.05/0.05/0.18 \\ 
 & L2.1 & 0.00/0.03/0.12  & 0.07/0.17/0.25  & 0.02/0.13/0.25 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.02/0.18/0.30  & 0.10/0.22/0.38  & 0.03/0.12/0.27 \\ 
 & Linf.0 & 0.02/0.10/0.20  & 0.07/0.17/0.28  & 0.00/0.03/0.08 \\ 
 & Linf.1 & 0.07/0.20/0.33  & 0.13/0.25/0.35  & 0.07/0.20/0.30 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.08/0.18  & 0.00/0.08/0.10 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.03/0.15  & 0.02/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.12  & 0.07/0.17/0.25  & 0.02/0.13/0.25 \\ 
 & pi.L2.1 & 0.00/0.05/0.07  & 0.00/0.10/0.18  & 0.07/0.10/0.25 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.07/0.20/0.33  & 0.13/0.25/0.35  & 0.07/0.20/0.30 \\ 
 & pi.Linf.1 & 0.08/0.25/0.28  & 0.08/0.17/0.20  & 0.10/0.20/0.32 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(2)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.12/0.20  & 0.00/0.00/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.02/0.15  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.07/0.12  & 0.00/0.03/0.10  & 0.02/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.03  & 0.07/0.15/0.20  & 0.00/0.02/0.10 \\ 
 & ell.Linf.1 & 0.00/0.00/0.03  & 0.05/0.05/0.05  & 0.00/0.00/0.07 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.67/0.93/1.00  & 0.05/0.05/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.90/1.00/1.00  & 0.05/0.10/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.12/0.20  & 0.00/0.00/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.72/0.88/0.95  & 0.00/0.03/0.08 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.90/0.92/0.95  & 0.00/0.03/0.07 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.02/0.15  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.03/0.17/0.25  & 0.00/0.00/0.03 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.05/0.10/0.18  & 0.00/0.00/0.07 \\ 
 & Linf.1 & 0.00/0.00/0.03  & 0.07/0.15/0.20  & 0.00/0.02/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.12/0.20  & 0.00/0.00/0.05 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.05/0.08  & 0.00/0.07/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.02/0.15  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.10  & 0.00/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.03  & 0.07/0.15/0.20  & 0.00/0.02/0.10 \\ 
 & pi.Linf.1 & 0.03/0.13/0.18  & 0.00/0.18/0.20  & 0.05/0.08/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(3)}} & ell.L1 & 0.05/0.05/0.05  & 0.20/0.40/0.48  & 0.00/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.10  & 0.25/0.43/0.55  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.10  & 0.00/0.05/0.10  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.07/0.12  & 0.10/0.32/0.52  & 0.05/0.10/0.10 \\ 
 & ell.Linf.1 & 0.00/0.00/0.07  & 0.00/0.05/0.10  & 0.05/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.97/1.00/1.00  & 0.00/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.20/0.40/0.48  & 0.00/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.05  & 0.98/1.00/1.00  & 0.00/0.05/0.05 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.10  & 0.25/0.43/0.55  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.08  & 0.27/0.42/0.55  & 0.02/0.05/0.08 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.23/0.38/0.40  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.00/0.07/0.12  & 0.10/0.32/0.52  & 0.05/0.10/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.20/0.40/0.48  & 0.00/0.05/0.05 \\ 
 & pi.L1.1 & 0.05/0.05/0.12  & 0.00/0.10/0.12  & 0.05/0.10/0.17 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.10  & 0.25/0.43/0.55  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.05/0.07/0.18  & 0.00/0.10/0.22  & 0.05/0.05/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.07/0.12  & 0.10/0.32/0.52  & 0.05/0.10/0.10 \\ 
 & pi.Linf.1 & 0.00/0.13/0.23  & 0.05/0.10/0.18  & 0.05/0.12/0.18 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(4)}} & ell.L1 & 0.00/0.00/0.00  & 0.45/0.63/0.83  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.52/0.72/0.88  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.03/0.10/0.12  & 0.05/0.10/0.17  & 0.05/0.10/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.33/0.65/0.78  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.08  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.45/0.63/0.83  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.52/0.72/0.88  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.50/0.80/0.87  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.43/0.75/0.85  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.33/0.65/0.78  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.45/0.63/0.83  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.15  & 0.00/0.00/0.02  & 0.00/0.00/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.52/0.72/0.88  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.00/0.02  & 0.00/0.00/0.03 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.33/0.65/0.78  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.05  & 0.00/0.03/0.12  & 0.00/0.00/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.ball(5)}} & ell.L1 & 0.00/0.02/0.05  & 0.75/0.90/0.98  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.07  & 0.80/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.13  & 0.00/0.02/0.10  & 0.00/0.02/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.05  & 0.57/0.83/0.97  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.07  & 0.00/0.03/0.05  & 0.00/0.02/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.75/0.90/0.98  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.07  & 0.80/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.02  & 0.85/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.92/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.02/0.05  & 0.57/0.83/0.97  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.75/0.90/0.98  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.10/0.13/0.18  & 0.05/0.13/0.17  & 0.02/0.10/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.07  & 0.80/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.10/0.13/0.17  & 0.05/0.15/0.17  & 0.02/0.10/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.05  & 0.57/0.83/0.97  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.08/0.13  & 0.00/0.03/0.10  & 0.02/0.05/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1,0.1)}} & ell.L1 & 0.00/0.00/0.00  & 0.10/0.25/0.35  & 0.00/0.03/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.20/0.27/0.38  & 0.00/0.00/0.02 \\ 
 & ell.L2.1 & 0.02/0.10/0.20  & 0.05/0.07/0.13  & 0.05/0.07/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.07/0.22/0.35  & 0.00/0.00/0.05 \\ 
 & ell.Linf.1 & 0.05/0.12/0.20  & 0.10/0.10/0.18  & 0.00/0.10/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.95/0.97/0.98  & 0.00/0.00/0.02 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/0.97/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.10/0.25/0.35  & 0.00/0.03/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.02 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.20/0.27/0.38  & 0.00/0.00/0.02 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.25/0.45/0.70  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.28/0.52/0.65  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.07/0.22/0.35  & 0.00/0.00/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.10/0.25/0.35  & 0.00/0.03/0.05 \\ 
 & pi.L1.1 & 0.00/0.08/0.13  & 0.00/0.05/0.08  & 0.00/0.03/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.20/0.27/0.38  & 0.00/0.00/0.02 \\ 
 & pi.L2.1 & 0.00/0.07/0.13  & 0.00/0.05/0.08  & 0.00/0.03/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.07/0.22/0.35  & 0.00/0.00/0.05 \\ 
 & pi.Linf.1 & 0.05/0.13/0.15  & 0.03/0.10/0.18  & 0.05/0.08/0.17 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.23/0.38  & 0.00/0.02/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.10/0.28/0.45  & 0.00/0.02/0.08 \\ 
 & ell.L2.1 & 0.00/0.02/0.05  & 0.00/0.02/0.02  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.05/0.05  & 0.10/0.12/0.28  & 0.00/0.02/0.10 \\ 
 & ell.Linf.1 & 0.02/0.05/0.05  & 0.00/0.00/0.05  & 0.00/0.02/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.92/1.00/1.00  & 0.00/0.05/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.05/0.08 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.23/0.38  & 0.00/0.02/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.03/0.05  & 0.77/0.98/1.00  & 0.00/0.02/0.02 \\ 
 & L2.0 & 0.05/0.05/0.05  & 0.90/0.98/1.00  & 0.00/0.02/0.07 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.10/0.28/0.45  & 0.00/0.02/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.32/0.52/0.65  & 0.22/0.33/0.40  & 0.00/0.02/0.20 \\ 
 & Linf.0 & 0.40/0.60/0.60  & 0.17/0.23/0.37  & 0.00/0.17/0.25 \\ 
 & Linf.1 & 0.00/0.05/0.05  & 0.10/0.12/0.28  & 0.00/0.02/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.23/0.38  & 0.00/0.02/0.08 \\ 
 & pi.L1.1 & 0.10/0.12/0.17  & 0.05/0.10/0.18  & 0.05/0.05/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.10/0.28/0.45  & 0.00/0.02/0.08 \\ 
 & pi.L2.1 & 0.10/0.12/0.15  & 0.05/0.10/0.18  & 0.05/0.05/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.05/0.05  & 0.10/0.12/0.28  & 0.00/0.02/0.10 \\ 
 & pi.Linf.1 & 0.08/0.08/0.12  & 0.05/0.08/0.15  & 0.07/0.08/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1,10)}} & ell.L1 & 0.05/0.05/0.05  & 0.12/0.22/0.23  & 0.10/0.15/0.18 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.12/0.18/0.22  & 0.10/0.15/0.18 \\ 
 & ell.L2.1 & 0.05/0.05/0.05  & 0.00/0.02/0.05  & 0.02/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.75/0.75/0.75  & 0.95/0.97/1.00  & 0.55/0.65/0.70 \\ 
 & L1.0 & 0.75/0.75/0.75  & 0.95/0.97/1.00  & 0.62/0.65/0.70 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.12/0.22/0.23  & 0.10/0.15/0.18 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 0.67/0.85/0.93  & 0.38/0.63/0.75 \\ 
 & L2.0 & 1.00/1.00/1.00  & 0.65/0.83/0.97  & 0.42/0.67/0.78 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.12/0.18/0.22  & 0.10/0.15/0.18 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.65/0.80/0.80  & 0.27/0.47/0.55  & 0.12/0.30/0.45 \\ 
 & Linf.0 & 0.65/0.80/0.80  & 0.32/0.50/0.57  & 0.12/0.33/0.45 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.12/0.22/0.23  & 0.10/0.15/0.18 \\ 
 & pi.L1.1 & 0.07/0.22/0.25  & 0.05/0.07/0.17  & 0.00/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.12/0.18/0.22  & 0.10/0.15/0.18 \\ 
 & pi.L2.1 & 0.07/0.18/0.23  & 0.05/0.07/0.13  & 0.00/0.07/0.17 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,0.1)}} & ell.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.03/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.05  & 0.05/0.17/0.22  & 0.00/0.00/0.05 \\ 
 & ell.L2.1 & 0.07/0.08/0.15  & 0.05/0.08/0.13  & 0.05/0.10/0.18 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.05/0.05  & 0.00/0.02/0.08  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.03/0.05  & 0.00/0.05/0.08  & 0.00/0.00/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.33/0.73/0.80  & 0.00/0.12/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.68/0.80/0.90  & 0.10/0.12/0.17 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.03/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.05  & 0.52/0.80/0.87  & 0.00/0.05/0.10 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.82/0.87/0.95  & 0.05/0.12/0.13 \\ 
 & L2.1 & 0.00/0.03/0.05  & 0.05/0.17/0.22  & 0.00/0.00/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.02  & 0.00/0.05/0.15  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.00/0.17/0.27  & 0.00/0.03/0.07 \\ 
 & Linf.1 & 0.00/0.05/0.05  & 0.00/0.02/0.08  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.03/0.07 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.05  & 0.05/0.17/0.22  & 0.00/0.00/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.02 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.05/0.05  & 0.00/0.02/0.08  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.12  & 0.00/0.00/0.07  & 0.00/0.00/0.03 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.13/0.28/0.38  & 0.00/0.03/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.03  & 0.12/0.17/0.30  & 0.00/0.00/0.10 \\ 
 & ell.L2.1 & 0.00/0.05/0.18  & 0.05/0.17/0.27  & 0.05/0.07/0.25 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.15/0.23/0.32  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.08/0.10/0.13  & 0.00/0.15/0.22  & 0.02/0.05/0.18 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.90/0.97/0.98  & 0.00/0.02/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.13/0.28/0.38  & 0.00/0.03/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.90/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.95/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.03  & 0.12/0.17/0.30  & 0.00/0.00/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.02  & 0.15/0.28/0.37  & 0.02/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.03/0.05  & 0.12/0.22/0.37  & 0.02/0.05/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.15/0.23/0.32  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.13/0.28/0.38  & 0.00/0.03/0.12 \\ 
 & pi.L1.1 & 0.10/0.15/0.15  & 0.02/0.05/0.18  & 0.00/0.10/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.03  & 0.12/0.17/0.30  & 0.00/0.00/0.10 \\ 
 & pi.L2.1 & 0.10/0.13/0.15  & 0.00/0.07/0.13  & 0.00/0.05/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.15/0.23/0.32  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.03/0.15  & 0.00/0.00/0.07 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,1,10)}} & ell.L1 & 0.05/0.05/0.05  & 0.07/0.12/0.25  & 0.05/0.10/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & ell.L2.1 & 0.02/0.12/0.18  & 0.10/0.12/0.15  & 0.07/0.13/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.07  & 0.05/0.07/0.10  & 0.05/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.95/1.00/1.00  & 0.15/0.20/0.22 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.10/0.17/0.23 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.07/0.12/0.25  & 0.05/0.10/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.15/0.18/0.23  & 0.80/0.88/0.97  & 0.22/0.30/0.40 \\ 
 & L2.0 & 0.15/0.18/0.23  & 0.80/0.92/1.00  & 0.17/0.35/0.40 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.45/0.45/0.45  & 0.17/0.27/0.43  & 0.03/0.18/0.25 \\ 
 & Linf.0 & 0.45/0.45/0.45  & 0.18/0.30/0.52  & 0.05/0.23/0.27 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.07/0.12/0.25  & 0.05/0.10/0.12 \\ 
 & pi.L1.1 & 0.05/0.08/0.10  & 0.05/0.08/0.10  & 0.05/0.05/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.05/0.08/0.18  & 0.05/0.05/0.07 \\ 
 & pi.L2.1 & 0.05/0.08/0.10  & 0.05/0.08/0.10  & 0.05/0.05/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.03/0.05  & 0.05/0.05/0.07  & 0.00/0.03/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,1)}} & ell.L1 & 0.00/0.02/0.05  & 0.00/0.10/0.17  & 0.02/0.07/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.03  & 0.00/0.02/0.12  & 0.00/0.00/0.08 \\ 
 & ell.L2.1 & 0.05/0.07/0.10  & 0.00/0.07/0.10  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.05  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.37/0.62/0.73  & 0.02/0.10/0.18 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.70/0.72/0.80  & 0.05/0.12/0.22 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.00/0.10/0.17  & 0.02/0.07/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.03/0.22/0.50  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.20/0.52/0.82  & 0.00/0.00/0.05 \\ 
 & L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.12  & 0.00/0.00/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.20/0.25/0.25  & 0.05/0.12/0.12  & 0.00/0.02/0.10 \\ 
 & Linf.0 & 0.22/0.25/0.25  & 0.05/0.12/0.13  & 0.00/0.03/0.13 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.00/0.10/0.17  & 0.02/0.07/0.12 \\ 
 & pi.L1.1 & 0.02/0.05/0.07  & 0.00/0.05/0.10  & 0.02/0.07/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.03  & 0.00/0.02/0.12  & 0.00/0.00/0.08 \\ 
 & pi.L2.1 & 0.02/0.05/0.07  & 0.00/0.05/0.10  & 0.00/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.02/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,10,10)}} & ell.L1 & 0.00/0.00/0.05  & 0.07/0.27/0.40  & 0.05/0.07/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.12/0.23/0.38  & 0.00/0.05/0.10 \\ 
 & ell.L2.1 & 0.05/0.05/0.08  & 0.02/0.07/0.17  & 0.07/0.12/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & ell.Linf.1 & 0.00/0.08/0.10  & 0.00/0.00/0.05  & 0.00/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.80/0.95/0.98  & 0.10/0.15/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.05/0.10/0.15 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.07/0.27/0.40  & 0.05/0.07/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.85/1.00/1.00  & 0.12/0.22/0.27 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.15/0.23/0.33 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.12/0.23/0.38  & 0.00/0.05/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.08/0.10/0.10  & 0.20/0.42/0.47  & 0.05/0.12/0.12 \\ 
 & Linf.0 & 0.10/0.10/0.12  & 0.25/0.42/0.53  & 0.05/0.12/0.18 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.07/0.27/0.40  & 0.05/0.07/0.13 \\ 
 & pi.L1.1 & 0.00/0.05/0.10  & 0.02/0.05/0.10  & 0.05/0.07/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.12/0.23/0.38  & 0.00/0.05/0.10 \\ 
 & pi.L2.1 & 0.00/0.03/0.08  & 0.02/0.05/0.08  & 0.02/0.07/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.03 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(0.1,10)}} & ell.L1 & 0.05/0.08/0.10  & 0.05/0.05/0.10  & 0.00/0.13/0.20 \\ 
 & ell.L1.1 & 0.00/0.03/0.03  & 0.00/0.00/0.00  & 0.00/0.02/0.05 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.08/0.10  & 0.05/0.05/0.07  & 0.00/0.10/0.13 \\ 
 & ell.L2.1 & 0.02/0.05/0.08  & 0.00/0.05/0.05  & 0.00/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.97/1.00/1.00  & 0.80/0.80/0.82  & 0.68/0.80/0.80 \\ 
 & L1.0 & 1.00/1.00/1.00  & 0.80/0.85/0.88  & 0.77/0.80/0.80 \\ 
 & L1.1 & 0.05/0.08/0.10  & 0.05/0.05/0.10  & 0.00/0.13/0.20 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.83/0.97/1.00  & 0.55/0.68/0.78  & 0.35/0.55/0.78 \\ 
 & L2.0 & 0.83/0.97/1.00  & 0.55/0.72/0.82  & 0.37/0.62/0.85 \\ 
 & L2.1 & 0.05/0.08/0.10  & 0.05/0.05/0.07  & 0.00/0.10/0.13 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.55/0.60/0.63  & 0.17/0.37/0.45  & 0.15/0.25/0.38 \\ 
 & Linf.0 & 0.55/0.60/0.63  & 0.17/0.38/0.48  & 0.15/0.28/0.45 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.08/0.10  & 0.05/0.05/0.10  & 0.00/0.13/0.20 \\ 
 & pi.L1.1 & 0.10/0.13/0.17  & 0.05/0.05/0.10  & 0.05/0.15/0.17 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.08/0.10  & 0.05/0.05/0.07  & 0.00/0.10/0.13 \\ 
 & pi.L2.1 & 0.10/0.13/0.17  & 0.05/0.05/0.10  & 0.05/0.15/0.17 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.00/0.02/0.03  & 0.00/0.02/0.02  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.07/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.08  & 0.00/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.12/0.18/0.28  & 0.00/0.00/0.03 \\ 
 & ell.Linf.1 & 0.00/0.00/0.02  & 0.05/0.05/0.07  & 0.03/0.05/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.02/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.07/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.32/0.45/0.55  & 0.00/0.02/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.32/0.50/0.60  & 0.00/0.03/0.07 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.12/0.18/0.28  & 0.00/0.00/0.03 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.07/0.17/0.28  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.12/0.18/0.28  & 0.00/0.00/0.03 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.07  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,1,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.20  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.13/0.25  & 0.05/0.18/0.23  & 0.07/0.10/0.27 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.08/0.15  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.05/0.10/0.10  & 0.00/0.00/0.03  & 0.00/0.02/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.87/0.95/1.00  & 0.00/0.00/0.02 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.87/1.00/1.00  & 0.00/0.02/0.17 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.10/0.20  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.40/0.52/0.62  & 0.20/0.43/0.58  & 0.00/0.03/0.07 \\ 
 & Linf.0 & 0.40/0.55/0.63  & 0.20/0.47/0.63  & 0.00/0.03/0.13 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.08/0.15  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.10/0.18  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.02/0.05/0.05  & 0.00/0.00/0.05  & 0.00/0.03/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.20  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.02/0.05/0.05  & 0.00/0.00/0.05  & 0.00/0.02/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.08/0.15  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.00/0.02/0.05  & 0.00/0.02/0.05  & 0.00/0.00/0.03 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,1)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.07/0.13  & 0.00/0.05/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.17  & 0.00/0.05/0.10 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.13/0.15  & 0.00/0.02/0.08 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.45/0.65/0.77  & 0.05/0.15/0.17 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.67/0.73/0.85  & 0.05/0.13/0.22 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.07/0.13  & 0.00/0.05/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.58/0.87/0.97  & 0.00/0.07/0.12 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/0.95/0.98  & 0.00/0.07/0.25 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.05/0.13/0.17  & 0.00/0.05/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.05/0.22/0.40  & 0.00/0.05/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.05/0.18/0.33  & 0.00/0.12/0.15 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.13/0.15  & 0.00/0.02/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.07/0.13  & 0.00/0.05/0.08 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.02/0.08  & 0.00/0.03/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.17  & 0.00/0.05/0.10 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.05/0.12  & 0.00/0.05/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.13/0.15  & 0.00/0.02/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.07  & 0.00/0.02/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,10,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.25/0.35  & 0.05/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.10/0.23/0.33  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.02/0.05/0.10  & 0.00/0.03/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.05/0.10/0.17  & 0.05/0.05/0.05 \\ 
 & ell.Linf.1 & 0.02/0.05/0.07  & 0.05/0.05/0.05  & 0.05/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.03/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.25/0.35  & 0.05/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.93/0.97/1.00  & 0.00/0.08/0.10 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.00/0.05/0.05 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.10/0.23/0.33  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.08/0.12  & 0.23/0.33/0.43  & 0.05/0.15/0.20 \\ 
 & Linf.0 & 0.02/0.13/0.18  & 0.30/0.45/0.52  & 0.07/0.12/0.25 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.05/0.10/0.17  & 0.05/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.25/0.35  & 0.05/0.05/0.05 \\ 
 & pi.L1.1 & 0.02/0.08/0.15  & 0.00/0.05/0.13  & 0.05/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.10/0.23/0.33  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.02/0.10/0.15  & 0.00/0.10/0.13  & 0.05/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.05/0.10/0.17  & 0.05/0.05/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.07  & 0.00/0.02/0.10  & 0.00/0.05/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(1,10)}} & ell.L1 & 0.00/0.03/0.05  & 0.00/0.02/0.15  & 0.00/0.00/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.05  & 0.00/0.03/0.15  & 0.00/0.05/0.15 \\ 
 & ell.L2.1 & 0.05/0.20/0.27  & 0.12/0.18/0.20  & 0.08/0.15/0.27 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.00/0.02/0.10  & 0.03/0.08/0.13 \\ 
 & ell.Linf.1 & 0.02/0.08/0.10  & 0.02/0.03/0.05  & 0.10/0.10/0.13 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.43/0.73/0.75  & 0.05/0.07/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.70/0.75/0.77  & 0.05/0.10/0.18 \\ 
 & L1.1 & 0.00/0.03/0.05  & 0.00/0.02/0.15  & 0.00/0.00/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.07/0.08  & 0.13/0.38/0.58  & 0.02/0.03/0.10 \\ 
 & L2.0 & 0.05/0.05/0.05  & 0.18/0.53/0.73  & 0.02/0.05/0.17 \\ 
 & L2.1 & 0.00/0.03/0.05  & 0.00/0.03/0.15  & 0.00/0.05/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.20/0.27/0.35  & 0.07/0.18/0.28  & 0.03/0.10/0.20 \\ 
 & Linf.0 & 0.20/0.30/0.35  & 0.07/0.22/0.28  & 0.00/0.05/0.17 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.00/0.02/0.10  & 0.03/0.08/0.13 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.05  & 0.00/0.02/0.15  & 0.00/0.00/0.08 \\ 
 & pi.L1.1 & 0.08/0.10/0.13  & 0.00/0.00/0.12  & 0.00/0.08/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.05  & 0.00/0.03/0.15  & 0.00/0.05/0.15 \\ 
 & pi.L2.1 & 0.05/0.07/0.12  & 0.00/0.02/0.07  & 0.00/0.07/0.18 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.00/0.02/0.10  & 0.03/0.08/0.13 \\ 
 & pi.Linf.1 & 0.00/0.07/0.10  & 0.05/0.07/0.10  & 0.10/0.10/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(10,10,10)}} & ell.L1 & 0.00/0.00/0.03  & 0.15/0.27/0.33  & 0.00/0.00/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.17/0.27/0.37  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.03/0.10/0.10  & 0.00/0.07/0.10  & 0.00/0.08/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.10/0.17/0.32  & 0.00/0.00/0.02 \\ 
 & ell.Linf.1 & 0.00/0.05/0.05  & 0.00/0.03/0.05  & 0.00/0.05/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.95/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.03  & 0.15/0.27/0.33  & 0.00/0.00/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.17/0.27/0.37  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.12/0.37/0.57  & 0.00/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.15/0.43/0.58  & 0.00/0.05/0.07 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.10/0.17/0.32  & 0.00/0.00/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.03  & 0.15/0.27/0.33  & 0.00/0.00/0.07 \\ 
 & pi.L1.1 & 0.00/0.08/0.10  & 0.00/0.02/0.05  & 0.00/0.05/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.17/0.27/0.37  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.05/0.10  & 0.00/0.02/0.07  & 0.00/0.05/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.10/0.17/0.32  & 0.00/0.00/0.02 \\ 
 & pi.Linf.1 & 0.02/0.05/0.13  & 0.00/0.08/0.13  & 0.00/0.05/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.cross(10,10)}} & ell.L1 & 0.00/0.00/0.03  & 0.05/0.08/0.12  & 0.00/0.02/0.03 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.03  & 0.05/0.08/0.10  & 0.00/0.03/0.08 \\ 
 & ell.L2.1 & 0.05/0.05/0.07  & 0.05/0.05/0.07  & 0.05/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.05/0.12/0.15  & 0.00/0.07/0.08 \\ 
 & ell.Linf.1 & 0.02/0.10/0.10  & 0.10/0.10/0.10  & 0.05/0.07/0.15 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.37/0.67/0.77  & 0.00/0.02/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.58/0.80/0.87  & 0.00/0.05/0.20 \\ 
 & L1.1 & 0.00/0.00/0.03  & 0.05/0.08/0.12  & 0.00/0.02/0.03 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.40/0.68/0.78  & 0.03/0.10/0.17 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.63/0.80/0.88  & 0.10/0.10/0.13 \\ 
 & L2.1 & 0.00/0.02/0.03  & 0.05/0.08/0.10  & 0.00/0.03/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.08/0.17/0.25  & 0.00/0.08/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.03/0.15/0.27  & 0.02/0.08/0.17 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.05/0.12/0.15  & 0.00/0.07/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.03  & 0.05/0.08/0.12  & 0.00/0.02/0.03 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.05/0.07/0.12  & 0.00/0.02/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.03  & 0.05/0.08/0.10  & 0.00/0.03/0.08 \\ 
 & pi.L2.1 & 0.00/0.03/0.07  & 0.05/0.07/0.10  & 0.05/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.05/0.12/0.15  & 0.00/0.07/0.08 \\ 
 & pi.Linf.1 & 0.00/0.05/0.10  & 0.00/0.07/0.12  & 0.05/0.05/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(10,5,25)}} & ell.L1 & 0.00/0.02/0.05  & 0.67/0.90/0.97  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.05/0.05  & 0.67/0.88/1.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.02/0.05/0.05  & 0.02/0.05/0.07  & 0.00/0.00/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.48/0.80/0.85  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.08/0.17  & 0.00/0.02/0.05  & 0.00/0.00/0.02 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.67/0.90/0.97  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.02/0.02  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.05/0.05  & 0.67/0.88/1.00  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.02  & 0.88/0.93/0.97  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.02/0.05  & 0.85/0.92/0.98  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.48/0.80/0.85  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.67/0.90/0.97  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.07/0.13  & 0.05/0.10/0.10  & 0.00/0.07/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.05/0.05  & 0.67/0.88/1.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.12/0.15  & 0.05/0.10/0.12  & 0.00/0.07/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.48/0.80/0.85  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.07/0.13  & 0.00/0.12/0.15  & 0.00/0.07/0.17 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(3,3,75)}} & ell.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.38  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.27/0.48  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.02  & 0.00/0.05/0.05  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.07/0.10  & 0.10/0.23/0.32  & 0.07/0.10/0.10 \\ 
 & ell.Linf.1 & 0.02/0.05/0.10  & 0.02/0.05/0.07  & 0.02/0.10/0.12 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.02/0.17/0.38  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.27/0.48  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.05/0.08  & 0.35/0.57/0.60  & 0.03/0.07/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.28/0.52/0.70  & 0.00/0.02/0.07 \\ 
 & Linf.1 & 0.00/0.07/0.10  & 0.10/0.23/0.32  & 0.07/0.10/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.02/0.17/0.38  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.27/0.48  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.07/0.10  & 0.10/0.23/0.32  & 0.07/0.10/0.10 \\ 
 & pi.Linf.1 & 0.00/0.02/0.17  & 0.05/0.10/0.12  & 0.07/0.13/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(4,4,25)}} & ell.L1 & 0.05/0.05/0.05  & 0.63/0.77/0.87  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.57/0.83/0.87  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.05/0.12  & 0.00/0.05/0.13  & 0.00/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.02  & 0.35/0.45/0.53  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.02/0.03/0.08  & 0.00/0.02/0.07  & 0.00/0.00/0.07 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.03/0.05/0.05  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.05/0.05/0.05  & 0.63/0.77/0.87  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.02/0.05/0.05  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.57/0.83/0.87  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.77/0.88/0.95  & 0.00/0.00/0.02 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.78/0.90/0.95  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.02  & 0.35/0.45/0.53  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.05  & 0.63/0.77/0.87  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.07/0.10/0.12  & 0.05/0.07/0.12  & 0.02/0.05/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.57/0.83/0.87  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.05/0.10/0.15  & 0.05/0.10/0.12  & 0.02/0.05/0.08 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.02  & 0.35/0.45/0.53  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.00/0.15/0.23  & 0.00/0.03/0.13  & 0.00/0.10/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(5,2,25)}} & ell.L1 & 0.05/0.05/0.07  & 0.10/0.17/0.18  & 0.05/0.10/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.10  & 0.10/0.13/0.17  & 0.10/0.12/0.20 \\ 
 & ell.L2.1 & 0.00/0.05/0.05  & 0.00/0.03/0.07  & 0.05/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.13  & 0.10/0.12/0.13  & 0.05/0.05/0.10 \\ 
 & ell.Linf.1 & 0.05/0.05/0.07  & 0.00/0.05/0.12  & 0.02/0.05/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.52/0.85/0.90  & 0.05/0.07/0.12 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.77/0.90/0.92  & 0.00/0.02/0.08 \\ 
 & L1.1 & 0.05/0.05/0.07  & 0.10/0.17/0.18  & 0.05/0.10/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.07  & 0.78/0.88/0.98  & 0.05/0.10/0.13 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/0.92/0.98  & 0.00/0.02/0.07 \\ 
 & L2.1 & 0.05/0.05/0.10  & 0.10/0.13/0.17  & 0.10/0.12/0.20 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.05/0.05  & 0.10/0.17/0.28  & 0.00/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.05  & 0.05/0.20/0.37  & 0.00/0.00/0.08 \\ 
 & Linf.1 & 0.05/0.05/0.13  & 0.10/0.12/0.13  & 0.05/0.05/0.10 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.07  & 0.10/0.17/0.18  & 0.05/0.10/0.13 \\ 
 & pi.L1.1 & 0.05/0.05/0.12  & 0.02/0.05/0.12  & 0.00/0.07/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.10  & 0.10/0.13/0.17  & 0.10/0.12/0.20 \\ 
 & pi.L2.1 & 0.05/0.05/0.12  & 0.02/0.07/0.10  & 0.07/0.07/0.18 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.13  & 0.10/0.12/0.13  & 0.05/0.05/0.10 \\ 
 & pi.Linf.1 & 0.05/0.10/0.10  & 0.02/0.05/0.10  & 0.00/0.07/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(6,4,25)}} & ell.L1 & 0.00/0.00/0.00  & 0.35/0.52/0.67  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.40/0.53/0.67  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.03/0.05  & 0.00/0.05/0.17  & 0.00/0.02/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.10/0.30/0.43  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.07  & 0.00/0.02/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.35/0.52/0.67  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.40/0.53/0.67  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.62/0.72/0.83  & 0.00/0.00/0.02 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.65/0.82/0.93  & 0.00/0.02/0.05 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.10/0.30/0.43  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.35/0.52/0.67  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.05/0.05/0.05  & 0.05/0.05/0.05  & 0.05/0.05/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.40/0.53/0.67  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.05/0.05/0.05  & 0.05/0.05/0.05  & 0.05/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.10/0.30/0.43  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.07  & 0.00/0.05/0.07  & 0.00/0.02/0.10 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.hull(8,3,100)}} & ell.L1 & 0.00/0.02/0.05  & 0.20/0.40/0.55  & 0.05/0.05/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.05  & 0.17/0.35/0.50  & 0.05/0.07/0.10 \\ 
 & ell.L2.1 & 0.00/0.00/0.07  & 0.00/0.00/0.03  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.03  & 0.13/0.25/0.38  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.00/0.05/0.13  & 0.00/0.00/0.00  & 0.00/0.00/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 0.97/1.00/1.00  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.02/0.05  & 0.20/0.40/0.55  & 0.05/0.05/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.02/0.05/0.05  & 1.00/1.00/1.00  & 0.05/0.05/0.08 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.05/0.05  & 0.17/0.35/0.50  & 0.05/0.07/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.23/0.47/0.63  & 0.00/0.00/0.02 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.28/0.45/0.63  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.00/0.02/0.03  & 0.13/0.25/0.38  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.05  & 0.20/0.40/0.55  & 0.05/0.05/0.10 \\ 
 & pi.L1.1 & 0.10/0.12/0.15  & 0.10/0.13/0.18  & 0.10/0.15/0.17 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.05  & 0.17/0.35/0.50  & 0.05/0.07/0.10 \\ 
 & pi.L2.1 & 0.10/0.15/0.15  & 0.10/0.12/0.17  & 0.10/0.15/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.03  & 0.13/0.25/0.38  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.05/0.05/0.10  & 0.00/0.03/0.08  & 0.05/0.10/0.12 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(1,2,100)}} & ell.L1 & 0.00/0.00/0.05  & 0.03/0.10/0.23  & 0.02/0.08/0.15 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.07/0.13 \\ 
 & ell.L2.1 & 0.00/0.02/0.05  & 0.00/0.10/0.13  & 0.00/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & ell.Linf.1 & 0.00/0.05/0.10  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.63/0.90/1.00  & 0.02/0.05/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.85/0.98/1.00  & 0.00/0.00/0.12 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.03/0.10/0.23  & 0.02/0.08/0.15 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.53/0.93/1.00  & 0.00/0.05/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/1.00/1.00  & 0.05/0.15/0.22 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.07/0.13 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.07  & 0.07/0.13/0.23  & 0.00/0.10/0.12 \\ 
 & Linf.0 & 0.00/0.07/0.12  & 0.10/0.20/0.38  & 0.10/0.10/0.15 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.03/0.10/0.23  & 0.02/0.08/0.15 \\ 
 & pi.L1.1 & 0.05/0.05/0.05  & 0.00/0.05/0.10  & 0.00/0.05/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.07/0.13 \\ 
 & pi.L2.1 & 0.05/0.05/0.05  & 0.00/0.08/0.10  & 0.00/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & pi.Linf.1 & 0.00/0.05/0.10  & 0.00/0.02/0.02  & 0.00/0.02/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(10,4,75)}} & ell.L1 & 0.00/0.00/0.00  & 0.30/0.42/0.55  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.27/0.48/0.63  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.02/0.07/0.23  & 0.00/0.00/0.15  & 0.00/0.02/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.10/0.23/0.47  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.05/0.07/0.13  & 0.05/0.07/0.10  & 0.05/0.10/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.30/0.42/0.55  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.27/0.48/0.63  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.47/0.77/0.90  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.50/0.83/0.90  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.10/0.23/0.47  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.30/0.42/0.55  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.12  & 0.03/0.13/0.15  & 0.03/0.10/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.27/0.48/0.63  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.07/0.13  & 0.02/0.13/0.15  & 0.03/0.12/0.13 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.10/0.23/0.47  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.02/0.05  & 0.00/0.02/0.12  & 0.00/0.10/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(2,2,10)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.08  & 0.00/0.05/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.08 \\ 
 & ell.L2.1 & 0.00/0.05/0.13  & 0.00/0.07/0.22  & 0.00/0.05/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.02  & 0.03/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & ell.Linf.1 & 0.00/0.03/0.10  & 0.00/0.07/0.10  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.32/0.65/0.92  & 0.00/0.12/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.63/0.93/0.95  & 0.05/0.10/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.07/0.08  & 0.00/0.05/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.38/0.85/0.88  & 0.00/0.03/0.08 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.82/0.90/0.95  & 0.05/0.10/0.15 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.02/0.12/0.22  & 0.05/0.07/0.12 \\ 
 & Linf.0 & 0.00/0.00/0.05  & 0.05/0.15/0.32  & 0.07/0.10/0.12 \\ 
 & Linf.1 & 0.00/0.00/0.02  & 0.03/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.08  & 0.00/0.05/0.10 \\ 
 & pi.L1.1 & 0.02/0.05/0.15  & 0.00/0.05/0.13  & 0.05/0.05/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.08 \\ 
 & pi.L2.1 & 0.02/0.07/0.12  & 0.00/0.05/0.10  & 0.05/0.07/0.08 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.02  & 0.03/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & pi.Linf.1 & 0.00/0.05/0.05  & 0.02/0.05/0.10  & 0.00/0.03/0.08 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(3,3,75)}} & ell.L1 & 0.00/0.00/0.00  & 0.15/0.27/0.32  & 0.00/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.12/0.27/0.32  & 0.00/0.02/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.13  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.02/0.03 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.15/0.27/0.32  & 0.00/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.12/0.27/0.32  & 0.00/0.02/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.22/0.38/0.50  & 0.00/0.03/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.27/0.45/0.57  & 0.00/0.05/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.02/0.13  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.15/0.27/0.32  & 0.00/0.05/0.05 \\ 
 & pi.L1.1 & 0.00/0.10/0.15  & 0.00/0.07/0.12  & 0.00/0.13/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.12/0.27/0.32  & 0.00/0.02/0.05 \\ 
 & pi.L2.1 & 0.00/0.07/0.15  & 0.05/0.05/0.10  & 0.02/0.08/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.02/0.13  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(4,3,25)}} & ell.L1 & 0.02/0.07/0.12  & 0.25/0.28/0.42  & 0.00/0.07/0.15 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.08/0.13  & 0.25/0.28/0.40  & 0.05/0.10/0.10 \\ 
 & ell.L2.1 & 0.05/0.08/0.15  & 0.05/0.07/0.08  & 0.05/0.05/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.10/0.12  & 0.18/0.25/0.32  & 0.10/0.15/0.15 \\ 
 & ell.Linf.1 & 0.02/0.03/0.05  & 0.00/0.05/0.05  & 0.00/0.03/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.02/0.05/0.07  & 1.00/1.00/1.00  & 0.00/0.03/0.08 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.02/0.07/0.12  & 0.25/0.28/0.42  & 0.00/0.07/0.15 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.08/0.10  & 1.00/1.00/1.00  & 0.05/0.08/0.10 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.05/0.08/0.13  & 0.25/0.28/0.40  & 0.05/0.10/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.08/0.08  & 0.37/0.45/0.53  & 0.05/0.12/0.15 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.22/0.33/0.53  & 0.00/0.00/0.03 \\ 
 & Linf.1 & 0.05/0.10/0.12  & 0.18/0.25/0.32  & 0.10/0.15/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.02/0.07/0.12  & 0.25/0.28/0.42  & 0.00/0.07/0.15 \\ 
 & pi.L1.1 & 0.17/0.20/0.20  & 0.10/0.17/0.23  & 0.12/0.20/0.30 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.08/0.13  & 0.25/0.28/0.40  & 0.05/0.10/0.10 \\ 
 & pi.L2.1 & 0.17/0.20/0.22  & 0.10/0.17/0.23  & 0.12/0.20/0.30 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.10/0.12  & 0.18/0.25/0.32  & 0.10/0.15/0.15 \\ 
 & pi.Linf.1 & 0.10/0.13/0.15  & 0.10/0.12/0.15  & 0.05/0.12/0.15 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(5,2,75)}} & ell.L1 & 0.00/0.05/0.10  & 0.12/0.22/0.33  & 0.05/0.08/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.13  & 0.20/0.22/0.28  & 0.05/0.08/0.17 \\ 
 & ell.L2.1 & 0.00/0.05/0.08  & 0.00/0.05/0.07  & 0.00/0.05/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.07/0.12/0.13  & 0.07/0.10/0.15  & 0.02/0.05/0.17 \\ 
 & ell.Linf.1 & 0.00/0.05/0.23  & 0.05/0.07/0.15  & 0.00/0.08/0.12 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.02/0.07  & 0.70/0.95/0.98  & 0.08/0.18/0.22 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.90/0.98/1.00  & 0.05/0.12/0.17 \\ 
 & L1.1 & 0.00/0.05/0.10  & 0.12/0.22/0.33  & 0.05/0.08/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.07  & 0.87/0.95/0.95  & 0.05/0.10/0.20 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.92/0.95/0.98  & 0.05/0.12/0.20 \\ 
 & L2.1 & 0.00/0.03/0.13  & 0.20/0.22/0.28  & 0.05/0.08/0.17 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.05/0.12/0.18  & 0.15/0.22/0.22  & 0.05/0.05/0.17 \\ 
 & Linf.0 & 0.00/0.07/0.10  & 0.10/0.13/0.32  & 0.05/0.07/0.13 \\ 
 & Linf.1 & 0.07/0.12/0.13  & 0.07/0.10/0.15  & 0.02/0.05/0.17 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.05/0.10  & 0.12/0.22/0.33  & 0.05/0.08/0.13 \\ 
 & pi.L1.1 & 0.00/0.13/0.22  & 0.10/0.15/0.23  & 0.05/0.07/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.13  & 0.20/0.22/0.28  & 0.05/0.08/0.17 \\ 
 & pi.L2.1 & 0.05/0.12/0.27  & 0.12/0.18/0.25  & 0.05/0.08/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.07/0.12/0.13  & 0.07/0.10/0.15  & 0.02/0.05/0.17 \\ 
 & pi.Linf.1 & 0.10/0.13/0.18  & 0.05/0.05/0.12  & 0.05/0.12/0.17 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(6,2,100)}} & ell.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.05  & 0.00/0.08/0.12  & 0.00/0.00/0.05 \\ 
 & ell.L2.1 & 0.00/0.07/0.10  & 0.00/0.05/0.10  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.02/0.05/0.05  & 0.05/0.08/0.12  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.02  & 0.55/0.87/0.92  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.85/0.95/0.95  & 0.00/0.00/0.13 \\ 
 & L1.1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.02  & 0.48/0.83/0.92  & 0.00/0.02/0.03 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.72/0.90/1.00  & 0.00/0.02/0.17 \\ 
 & L2.1 & 0.00/0.00/0.05  & 0.00/0.08/0.12  & 0.00/0.00/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.03/0.05  & 0.02/0.08/0.18  & 0.00/0.00/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.02/0.10/0.18  & 0.00/0.02/0.05 \\ 
 & Linf.1 & 0.02/0.05/0.05  & 0.05/0.08/0.12  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.05  & 0.00/0.13/0.17  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.02/0.05  & 0.00/0.00/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.05  & 0.00/0.08/0.12  & 0.00/0.00/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.00/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.02/0.05/0.05  & 0.05/0.08/0.12  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.00/0.02/0.03  & 0.00/0.00/0.02  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(8,3,50)}} & ell.L1 & 0.00/0.00/0.00  & 0.25/0.38/0.57  & 0.00/0.00/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.25/0.47/0.52  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.05/0.10/0.10  & 0.08/0.15/0.18  & 0.05/0.07/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.07  & 0.10/0.17/0.23  & 0.00/0.03/0.05 \\ 
 & ell.Linf.1 & 0.05/0.05/0.05  & 0.05/0.05/0.05  & 0.00/0.03/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.98/1.00/1.00  & 0.00/0.02/0.03 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.02/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.25/0.38/0.57  & 0.00/0.00/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.03 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.25/0.47/0.52  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.33/0.43/0.68  & 0.00/0.00/0.00 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.25/0.53/0.75  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.00/0.00/0.07  & 0.10/0.17/0.23  & 0.00/0.03/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.25/0.38/0.57  & 0.00/0.00/0.05 \\ 
 & pi.L1.1 & 0.00/0.10/0.25  & 0.05/0.10/0.25  & 0.07/0.17/0.22 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.25/0.47/0.52  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.05/0.10/0.23  & 0.00/0.07/0.18  & 0.02/0.17/0.18 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.07  & 0.10/0.17/0.23  & 0.00/0.03/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.08  & 0.00/0.02/0.10  & 0.00/0.05/0.07 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.random.polytope(9,2,10)}} & ell.L1 & 0.00/0.05/0.05  & 0.07/0.13/0.22  & 0.02/0.02/0.08 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.02/0.07/0.23  & 0.00/0.00/0.12 \\ 
 & ell.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.07  & 0.00/0.02/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.05/0.08/0.17  & 0.00/0.02/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.03  & 0.00/0.00/0.03  & 0.00/0.05/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.05  & 0.50/0.77/0.88  & 0.07/0.07/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.77/0.90/1.00  & 0.05/0.12/0.15 \\ 
 & L1.1 & 0.00/0.05/0.05  & 0.07/0.13/0.22  & 0.02/0.02/0.08 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.47/0.85/0.95  & 0.03/0.05/0.12 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.90/0.93/0.95  & 0.05/0.15/0.20 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.02/0.07/0.23  & 0.00/0.00/0.12 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.05/0.15/0.17  & 0.00/0.02/0.07 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.10/0.15/0.25  & 0.00/0.02/0.12 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.05/0.08/0.17  & 0.00/0.02/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.05/0.05  & 0.07/0.13/0.22  & 0.02/0.02/0.08 \\ 
 & pi.L1.1 & 0.00/0.07/0.07  & 0.00/0.02/0.10  & 0.00/0.02/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.02/0.07/0.23  & 0.00/0.00/0.12 \\ 
 & pi.L2.1 & 0.00/0.02/0.10  & 0.00/0.03/0.10  & 0.00/0.03/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.05/0.08/0.17  & 0.00/0.02/0.05 \\ 
 & pi.Linf.1 & 0.00/0.05/0.05  & 0.00/0.05/0.12  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.simplex(unit,2)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.05/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.03/0.18  & 0.02/0.03/0.10 \\ 
 & ell.L2.1 & 0.00/0.05/0.13  & 0.07/0.10/0.18  & 0.05/0.13/0.23 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.03/0.07 \\ 
 & ell.Linf.1 & 0.07/0.10/0.13  & 0.05/0.10/0.10  & 0.00/0.08/0.15 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.32/0.63/0.80  & 0.00/0.07/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.62/0.82/0.88  & 0.00/0.10/0.17 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.05/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.48/0.72/0.80  & 0.05/0.08/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.70/0.80/0.92  & 0.05/0.08/0.23 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.03/0.18  & 0.02/0.03/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.02/0.05  & 0.07/0.20/0.43  & 0.00/0.05/0.10 \\ 
 & Linf.0 & 0.00/0.05/0.07  & 0.10/0.25/0.43  & 0.00/0.07/0.13 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.03/0.07 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.05/0.05 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.03/0.05  & 0.02/0.05/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.03/0.18  & 0.02/0.03/0.10 \\ 
 & pi.L2.1 & 0.00/0.00/0.02  & 0.00/0.03/0.05  & 0.02/0.05/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.00/0.07/0.15  & 0.02/0.03/0.07 \\ 
 & pi.Linf.1 & 0.00/0.03/0.03  & 0.00/0.02/0.05  & 0.00/0.03/0.05 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.simplex(unit,3)}} & ell.L1 & 0.00/0.00/0.00  & 0.05/0.18/0.30  & 0.00/0.03/0.05 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.30  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.03/0.07  & 0.00/0.05/0.08  & 0.05/0.10/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.07/0.08/0.10  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.03/0.05  & 0.05/0.05/0.08  & 0.02/0.07/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.90/0.98/1.00  & 0.03/0.07/0.15 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.05/0.10/0.15 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.05/0.18/0.30  & 0.00/0.03/0.05 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.02 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.02/0.07 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.05/0.13/0.30  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.15/0.20/0.25  & 0.05/0.05/0.05 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.12/0.22/0.32  & 0.05/0.05/0.05 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.07/0.08/0.10  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.05/0.18/0.30  & 0.00/0.03/0.05 \\ 
 & pi.L1.1 & 0.05/0.05/0.05  & 0.05/0.05/0.10  & 0.02/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.05/0.13/0.30  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.02/0.03/0.05  & 0.05/0.05/0.05  & 0.02/0.05/0.05 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.07/0.08/0.10  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{null.simplex(unit,4)}} & ell.L1 & 0.00/0.00/0.00  & 0.27/0.40/0.55  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.25/0.35/0.58  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.03/0.05  & 0.00/0.00/0.08  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.00  & 0.05/0.05/0.18  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.05/0.08  & 0.00/0.00/0.05  & 0.02/0.07/0.08 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.27/0.40/0.55  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.25/0.35/0.58  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.00  & 0.37/0.47/0.60  & 0.05/0.05/0.07 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.37/0.53/0.70  & 0.05/0.07/0.10 \\ 
 & Linf.1 & 0.00/0.00/0.00  & 0.05/0.05/0.18  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.27/0.40/0.55  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.02/0.07  & 0.00/0.03/0.17  & 0.00/0.07/0.22 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.25/0.35/0.58  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.17  & 0.00/0.10/0.23 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.00  & 0.05/0.05/0.18  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.05/0.07  & 0.00/0.02/0.05  & 0.00/0.02/0.07 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(1.25).mvn.0.01}} & ell.L1 & 0.62/0.65/0.67  & 0.60/0.73/0.75  & 0.57/0.68/0.72 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & ell.L2.1 & 0.00/0.00/0.05  & 0.00/0.10/0.10  & 0.00/0.00/0.00 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.90/0.95/0.95  & 1.00/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & ell.Linf.1 & 0.48/0.50/0.58  & 0.45/0.52/0.60  & 0.42/0.47/0.58 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.60/0.62/0.65  & 0.60/0.70/0.73  & 0.57/0.68/0.68 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.17/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.62/0.65/0.67  & 0.60/0.73/0.75  & 0.57/0.68/0.72 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.17/0.22  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.90/0.95/0.95  & 0.97/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & Linf.0 & 0.05/0.05/0.05  & 0.05/0.10/0.22  & 0.05/0.07/0.08 \\ 
 & Linf.1 & 0.90/0.95/0.95  & 1.00/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.62/0.65/0.67  & 0.60/0.73/0.75  & 0.57/0.68/0.72 \\ 
 & pi.L1.1 & 0.70/0.87/0.90  & 0.62/0.88/0.95  & 0.63/0.88/0.97 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.95/0.95/0.95  & 0.95/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & pi.L2.1 & 0.85/0.88/0.93  & 0.87/0.95/0.95  & 0.82/0.93/0.98 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.90/0.95/0.95  & 1.00/1.00/1.00  & 0.95/0.95/0.95 \\ 
 & pi.Linf.1 & 0.80/0.88/0.93  & 0.90/0.90/0.95  & 0.85/0.90/0.90 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(1.25).mvn.0.05}} & ell.L1 & 0.22/0.32/0.38  & 0.32/0.45/0.57  & 0.30/0.32/0.40 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.53/0.62/0.82  & 0.85/0.93/0.95  & 0.80/0.85/0.88 \\ 
 & ell.L2.1 & 0.10/0.12/0.20  & 0.02/0.12/0.15  & 0.05/0.13/0.18 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.65/0.73/0.83  & 0.85/0.85/0.85  & 0.70/0.90/0.92 \\ 
 & ell.Linf.1 & 0.43/0.45/0.50  & 0.40/0.45/0.52  & 0.45/0.48/0.52 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.22/0.32/0.33  & 0.33/0.43/0.58  & 0.30/0.30/0.33 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.25/0.33/0.45  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.22/0.32/0.38  & 0.32/0.45/0.57  & 0.30/0.32/0.40 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.52/0.60/0.68  & 0.85/0.95/0.97  & 0.80/0.83/0.83 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.30/0.45  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.53/0.62/0.82  & 0.85/0.93/0.95  & 0.80/0.85/0.88 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.60/0.68/0.77  & 0.80/0.83/0.85  & 0.70/0.78/0.90 \\ 
 & Linf.0 & 0.15/0.18/0.20  & 0.20/0.25/0.33  & 0.20/0.20/0.30 \\ 
 & Linf.1 & 0.65/0.73/0.83  & 0.85/0.85/0.85  & 0.70/0.90/0.92 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.22/0.32/0.38  & 0.32/0.45/0.57  & 0.30/0.32/0.40 \\ 
 & pi.L1.1 & 0.22/0.35/0.40  & 0.27/0.38/0.47  & 0.30/0.33/0.38 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.53/0.62/0.82  & 0.85/0.93/0.95  & 0.80/0.85/0.88 \\ 
 & pi.L2.1 & 0.33/0.63/0.78  & 0.45/0.68/0.77  & 0.35/0.57/0.80 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.65/0.73/0.83  & 0.85/0.85/0.85  & 0.70/0.90/0.92 \\ 
 & pi.Linf.1 & 0.68/0.77/0.80  & 0.70/0.73/0.77  & 0.65/0.75/0.85 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(1.25).mvn.0.1}} & ell.L1 & 0.05/0.10/0.15  & 0.00/0.20/0.25  & 0.10/0.12/0.18 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.13/0.23  & 0.10/0.32/0.35  & 0.10/0.18/0.27 \\ 
 & ell.L2.1 & 0.07/0.08/0.10  & 0.00/0.10/0.13  & 0.00/0.08/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.35/0.48/0.62  & 0.47/0.63/0.70  & 0.32/0.47/0.53 \\ 
 & ell.Linf.1 & 0.25/0.38/0.42  & 0.35/0.37/0.43  & 0.35/0.38/0.40 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.08/0.12  & 0.17/0.63/0.67  & 0.10/0.15/0.18 \\ 
 & L1.0 & 0.00/0.02/0.05  & 0.55/0.60/0.65  & 0.02/0.05/0.07 \\ 
 & L1.1 & 0.05/0.10/0.15  & 0.00/0.20/0.25  & 0.10/0.12/0.18 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.10/0.17  & 0.37/0.67/0.75  & 0.10/0.17/0.25 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.50/0.67/0.78  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.05/0.13/0.23  & 0.10/0.32/0.35  & 0.10/0.18/0.27 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.35/0.40/0.45  & 0.48/0.67/0.75  & 0.27/0.47/0.53 \\ 
 & Linf.0 & 0.20/0.27/0.30  & 0.35/0.35/0.38  & 0.30/0.32/0.35 \\ 
 & Linf.1 & 0.35/0.48/0.62  & 0.47/0.63/0.70  & 0.32/0.47/0.53 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.10/0.15  & 0.00/0.20/0.25  & 0.10/0.12/0.18 \\ 
 & pi.L1.1 & 0.05/0.15/0.23  & 0.00/0.17/0.20  & 0.10/0.10/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.13/0.23  & 0.10/0.32/0.35  & 0.10/0.18/0.27 \\ 
 & pi.L2.1 & 0.05/0.18/0.25  & 0.00/0.13/0.22  & 0.10/0.13/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.35/0.48/0.62  & 0.47/0.63/0.70  & 0.32/0.47/0.53 \\ 
 & pi.Linf.1 & 0.35/0.53/0.63  & 0.37/0.52/0.65  & 0.27/0.43/0.50 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(10).mvn.0.01}} & ell.L1 & 0.60/0.60/0.62  & 0.68/0.72/0.75  & 0.42/0.50/0.57 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.65/0.65/0.68  & 0.70/0.73/0.80  & 0.58/0.65/0.65 \\ 
 & ell.L2.1 & 0.38/0.70/0.80  & 0.40/0.53/0.77  & 0.47/0.65/0.72 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.60/0.63/0.67  & 0.68/0.73/0.78  & 0.55/0.60/0.65 \\ 
 & ell.Linf.1 & 0.70/0.70/0.75  & 0.70/0.70/0.77  & 0.62/0.68/0.72 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.60/0.60/0.60  & 0.67/0.75/0.80  & 0.42/0.50/0.50 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.02/0.15/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.60/0.60/0.62  & 0.68/0.72/0.75  & 0.42/0.50/0.57 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.65/0.65/0.65  & 0.88/0.95/1.00  & 0.58/0.65/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.45/0.50/0.50  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.65/0.65/0.68  & 0.70/0.73/0.80  & 0.58/0.65/0.65 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.78/0.95/0.98  & 1.00/1.00/1.00  & 0.75/0.75/0.75 \\ 
 & Linf.0 & 0.90/0.98/1.00  & 1.00/1.00/1.00  & 0.70/0.75/0.75 \\ 
 & Linf.1 & 0.60/0.63/0.67  & 0.68/0.73/0.78  & 0.55/0.60/0.65 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.60/0.60/0.62  & 0.68/0.72/0.75  & 0.42/0.50/0.57 \\ 
 & pi.L1.1 & 0.50/0.57/0.60  & 0.55/0.60/0.65  & 0.47/0.60/0.60 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.65/0.65/0.68  & 0.70/0.73/0.80  & 0.58/0.65/0.65 \\ 
 & pi.L2.1 & 0.60/0.60/0.60  & 0.60/0.65/0.67  & 0.57/0.60/0.63 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.60/0.63/0.67  & 0.68/0.73/0.78  & 0.55/0.60/0.65 \\ 
 & pi.Linf.1 & 0.52/0.58/0.60  & 0.60/0.60/0.63  & 0.55/0.58/0.63 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(10).mvn.0.05}} & ell.L1 & 0.25/0.37/0.55  & 0.35/0.47/0.53  & 0.22/0.30/0.40 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.70/0.73/0.77  & 0.75/0.80/0.87  & 0.60/0.63/0.70 \\ 
 & ell.L2.1 & 0.22/0.40/0.50  & 0.40/0.45/0.47  & 0.32/0.45/0.53 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.60/0.65/0.75  & 0.70/0.80/0.80  & 0.60/0.62/0.65 \\ 
 & ell.Linf.1 & 0.50/0.55/0.63  & 0.50/0.57/0.65  & 0.52/0.55/0.60 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.25/0.33/0.40  & 0.40/0.58/0.68  & 0.18/0.28/0.35 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.23/0.25  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.25/0.37/0.55  & 0.35/0.47/0.53  & 0.22/0.30/0.40 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.70/0.73/0.73  & 0.93/1.00/1.00  & 0.60/0.63/0.65 \\ 
 & L2.0 & 0.00/0.00/0.03  & 0.37/0.38/0.45  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.70/0.73/0.77  & 0.75/0.80/0.87  & 0.60/0.63/0.70 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.75/0.92/0.93  & 1.00/1.00/1.00  & 0.75/0.75/0.75 \\ 
 & Linf.0 & 0.85/0.95/1.00  & 1.00/1.00/1.00  & 0.75/0.75/0.75 \\ 
 & Linf.1 & 0.60/0.65/0.75  & 0.70/0.80/0.80  & 0.60/0.62/0.65 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.25/0.37/0.55  & 0.35/0.47/0.53  & 0.22/0.30/0.40 \\ 
 & pi.L1.1 & 0.15/0.20/0.37  & 0.10/0.27/0.40  & 0.12/0.23/0.30 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.70/0.73/0.77  & 0.75/0.80/0.87  & 0.60/0.63/0.70 \\ 
 & pi.L2.1 & 0.50/0.57/0.67  & 0.42/0.58/0.65  & 0.42/0.60/0.60 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.60/0.65/0.75  & 0.70/0.80/0.80  & 0.60/0.62/0.65 \\ 
 & pi.Linf.1 & 0.50/0.58/0.63  & 0.50/0.55/0.70  & 0.45/0.62/0.67 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(10).mvn.0.1}} & ell.L1 & 0.30/0.38/0.40  & 0.35/0.40/0.42  & 0.30/0.37/0.40 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.60/0.63/0.65  & 0.65/0.65/0.72  & 0.62/0.65/0.65 \\ 
 & ell.L2.1 & 0.00/0.05/0.15  & 0.05/0.10/0.12  & 0.00/0.05/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.60/0.63/0.65  & 0.65/0.65/0.67  & 0.62/0.65/0.65 \\ 
 & ell.Linf.1 & 0.40/0.50/0.50  & 0.43/0.55/0.55  & 0.50/0.53/0.55 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.30/0.37/0.38  & 0.35/0.42/0.52  & 0.30/0.37/0.37 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.05/0.12/0.18  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.30/0.38/0.40  & 0.35/0.40/0.42  & 0.30/0.37/0.40 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.60/0.67/0.70  & 0.73/0.92/0.97  & 0.62/0.65/0.65 \\ 
 & L2.0 & 0.05/0.05/0.05  & 0.37/0.45/0.50  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.60/0.63/0.65  & 0.65/0.65/0.72  & 0.62/0.65/0.65 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.83/0.85/0.87  & 1.00/1.00/1.00  & 0.75/0.75/0.80 \\ 
 & Linf.0 & 0.85/0.88/0.98  & 1.00/1.00/1.00  & 0.70/0.75/0.80 \\ 
 & Linf.1 & 0.60/0.63/0.65  & 0.65/0.65/0.67  & 0.62/0.65/0.65 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.30/0.38/0.40  & 0.35/0.40/0.42  & 0.30/0.37/0.40 \\ 
 & pi.L1.1 & 0.17/0.30/0.35  & 0.20/0.32/0.35  & 0.25/0.27/0.32 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.60/0.63/0.65  & 0.65/0.65/0.72  & 0.62/0.65/0.65 \\ 
 & pi.L2.1 & 0.50/0.58/0.62  & 0.50/0.57/0.60  & 0.50/0.58/0.62 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.60/0.63/0.65  & 0.65/0.65/0.67  & 0.62/0.65/0.65 \\ 
 & pi.Linf.1 & 0.55/0.55/0.55  & 0.52/0.58/0.60  & 0.55/0.60/0.60 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(2).mvn.0.01}} & ell.L1 & 0.20/0.20/0.30  & 0.17/0.42/0.58  & 0.20/0.25/0.33 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.50/0.55/0.67  & 0.52/0.68/0.83  & 0.45/0.52/0.67 \\ 
 & ell.L2.1 & 0.00/0.05/0.15  & 0.00/0.02/0.10  & 0.00/0.07/0.18 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.47/0.65/0.70  & 0.70/0.78/0.82  & 0.45/0.53/0.70 \\ 
 & ell.Linf.1 & 0.40/0.40/0.40  & 0.30/0.43/0.45  & 0.35/0.42/0.43 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.20/0.20/0.25  & 0.35/0.57/0.70  & 0.20/0.25/0.25 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.32/0.48/0.50  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.20/0.20/0.30  & 0.17/0.42/0.58  & 0.20/0.25/0.33 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.50/0.55/0.57  & 0.87/1.00/1.00  & 0.45/0.52/0.53 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.50/0.50/0.50  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.50/0.55/0.67  & 0.52/0.68/0.83  & 0.45/0.52/0.67 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.42/0.52/0.60  & 0.62/0.70/0.80  & 0.42/0.47/0.57 \\ 
 & Linf.0 & 0.25/0.25/0.25  & 0.27/0.33/0.57  & 0.25/0.28/0.30 \\ 
 & Linf.1 & 0.47/0.65/0.70  & 0.70/0.78/0.82  & 0.45/0.53/0.70 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.20/0.20/0.30  & 0.17/0.42/0.58  & 0.20/0.25/0.33 \\ 
 & pi.L1.1 & 0.05/0.08/0.17  & 0.07/0.10/0.12  & 0.05/0.10/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.50/0.55/0.67  & 0.52/0.68/0.83  & 0.45/0.52/0.67 \\ 
 & pi.L2.1 & 0.25/0.40/0.45  & 0.22/0.38/0.40  & 0.22/0.33/0.43 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.47/0.65/0.70  & 0.70/0.78/0.82  & 0.45/0.53/0.70 \\ 
 & pi.Linf.1 & 0.35/0.45/0.58  & 0.47/0.53/0.57  & 0.37/0.50/0.67 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(2).mvn.0.05}} & ell.L1 & 0.00/0.10/0.17  & 0.08/0.23/0.40  & 0.05/0.13/0.33 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.25/0.27/0.30  & 0.32/0.43/0.57  & 0.20/0.35/0.38 \\ 
 & ell.L2.1 & 0.00/0.07/0.13  & 0.05/0.05/0.12  & 0.05/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.30/0.30/0.33  & 0.37/0.37/0.40  & 0.25/0.32/0.38 \\ 
 & ell.Linf.1 & 0.25/0.25/0.30  & 0.22/0.28/0.30  & 0.20/0.27/0.30 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.07/0.12  & 0.32/0.62/0.72  & 0.00/0.10/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.55/0.70/0.73  & 0.00/0.00/0.05 \\ 
 & L1.1 & 0.00/0.10/0.17  & 0.08/0.23/0.40  & 0.05/0.13/0.33 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.20/0.25/0.28  & 0.52/0.88/1.00  & 0.20/0.33/0.37 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.65/0.72/0.75  & 0.00/0.00/0.02 \\ 
 & L2.1 & 0.25/0.27/0.30  & 0.32/0.43/0.57  & 0.20/0.35/0.38 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.30/0.30/0.30  & 0.32/0.32/0.40  & 0.25/0.28/0.32 \\ 
 & Linf.0 & 0.00/0.00/0.00  & 0.00/0.08/0.25  & 0.00/0.10/0.22 \\ 
 & Linf.1 & 0.30/0.30/0.33  & 0.37/0.37/0.40  & 0.25/0.32/0.38 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.10/0.17  & 0.08/0.23/0.40  & 0.05/0.13/0.33 \\ 
 & pi.L1.1 & 0.00/0.17/0.25  & 0.00/0.02/0.10  & 0.00/0.15/0.27 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.25/0.27/0.30  & 0.32/0.43/0.57  & 0.20/0.35/0.38 \\ 
 & pi.L2.1 & 0.10/0.28/0.35  & 0.15/0.20/0.25  & 0.05/0.23/0.32 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.30/0.30/0.33  & 0.37/0.37/0.40  & 0.25/0.32/0.38 \\ 
 & pi.Linf.1 & 0.25/0.30/0.30  & 0.25/0.25/0.27  & 0.25/0.27/0.30 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(2).mvn.0.1}} & ell.L1 & 0.05/0.05/0.07  & 0.05/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.05/0.10  & 0.05/0.10/0.17  & 0.05/0.08/0.15 \\ 
 & ell.L2.1 & 0.00/0.10/0.13  & 0.00/0.10/0.20  & 0.05/0.07/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.07/0.22  & 0.07/0.23/0.38  & 0.08/0.23/0.33 \\ 
 & ell.Linf.1 & 0.10/0.12/0.17  & 0.10/0.10/0.15  & 0.10/0.10/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.05  & 0.40/0.57/0.67  & 0.05/0.10/0.10 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.62/0.65/0.70  & 0.05/0.05/0.12 \\ 
 & L1.1 & 0.05/0.05/0.07  & 0.05/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.05/0.07  & 0.57/0.77/0.90  & 0.05/0.08/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.80/0.95/0.95  & 0.00/0.03/0.15 \\ 
 & L2.1 & 0.05/0.05/0.10  & 0.05/0.10/0.17  & 0.05/0.08/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.08/0.18/0.33  & 0.37/0.58/0.70  & 0.18/0.40/0.47 \\ 
 & Linf.0 & 0.15/0.25/0.32  & 0.43/0.57/0.62  & 0.18/0.33/0.40 \\ 
 & Linf.1 & 0.00/0.07/0.22  & 0.07/0.23/0.38  & 0.08/0.23/0.33 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.05/0.07  & 0.05/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & pi.L1.1 & 0.05/0.05/0.10  & 0.05/0.05/0.05  & 0.00/0.03/0.07 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.05/0.10  & 0.05/0.10/0.17  & 0.05/0.08/0.15 \\ 
 & pi.L2.1 & 0.05/0.08/0.15  & 0.05/0.07/0.07  & 0.05/0.08/0.12 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.07/0.22  & 0.07/0.23/0.38  & 0.08/0.23/0.33 \\ 
 & pi.Linf.1 & 0.10/0.22/0.32  & 0.15/0.20/0.25  & 0.08/0.22/0.25 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(5).mvn.0.01}} & ell.L1 & 0.25/0.25/0.30  & 0.30/0.40/0.40  & 0.25/0.30/0.38 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.50/0.50/0.52  & 0.55/0.55/0.57  & 0.50/0.50/0.52 \\ 
 & ell.L2.1 & 0.17/0.30/0.35  & 0.25/0.25/0.33  & 0.20/0.22/0.25 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.50/0.52/0.55  & 0.55/0.55/0.55  & 0.52/0.55/0.55 \\ 
 & ell.Linf.1 & 0.47/0.53/0.60  & 0.55/0.58/0.60  & 0.43/0.52/0.58 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.25/0.25/0.27  & 0.32/0.50/0.58  & 0.25/0.30/0.32 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.15/0.18/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.25/0.25/0.30  & 0.30/0.40/0.40  & 0.25/0.30/0.38 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.50/0.50/0.50  & 0.78/0.88/0.90  & 0.50/0.50/0.50 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.40/0.40/0.40  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.50/0.50/0.52  & 0.55/0.55/0.57  & 0.50/0.50/0.52 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.75/0.78/0.82  & 0.95/1.00/1.00  & 0.68/0.73/0.75 \\ 
 & Linf.0 & 0.75/0.83/0.92  & 0.95/1.00/1.00  & 0.72/0.75/0.75 \\ 
 & Linf.1 & 0.50/0.52/0.55  & 0.55/0.55/0.55  & 0.52/0.55/0.55 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.25/0.25/0.30  & 0.30/0.40/0.40  & 0.25/0.30/0.38 \\ 
 & pi.L1.1 & 0.30/0.30/0.30  & 0.25/0.27/0.30  & 0.25/0.25/0.27 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.50/0.50/0.52  & 0.55/0.55/0.57  & 0.50/0.50/0.52 \\ 
 & pi.L2.1 & 0.45/0.45/0.45  & 0.45/0.45/0.47  & 0.37/0.45/0.45 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.50/0.52/0.55  & 0.55/0.55/0.55  & 0.52/0.55/0.55 \\ 
 & pi.Linf.1 & 0.45/0.50/0.53  & 0.48/0.52/0.55  & 0.45/0.45/0.48 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(5).mvn.0.05}} & ell.L1 & 0.10/0.15/0.23  & 0.15/0.30/0.38  & 0.10/0.20/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.55/0.62/0.65  & 0.55/0.65/0.70  & 0.60/0.60/0.65 \\ 
 & ell.L2.1 & 0.00/0.02/0.07  & 0.00/0.02/0.10  & 0.00/0.02/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.53/0.60/0.67  & 0.60/0.67/0.70  & 0.50/0.57/0.63 \\ 
 & ell.Linf.1 & 0.52/0.55/0.63  & 0.50/0.50/0.55  & 0.50/0.52/0.57 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.15/0.17  & 0.20/0.40/0.52  & 0.10/0.15/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.20/0.22  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.15/0.23  & 0.15/0.30/0.38  & 0.10/0.20/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.53/0.62/0.65  & 0.73/0.90/0.95  & 0.60/0.60/0.60 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.30/0.37/0.42  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.55/0.62/0.65  & 0.55/0.65/0.70  & 0.60/0.60/0.65 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.65/0.72/0.78  & 0.77/0.90/0.93  & 0.63/0.67/0.75 \\ 
 & Linf.0 & 0.65/0.78/0.83  & 0.80/0.90/1.00  & 0.65/0.70/0.75 \\ 
 & Linf.1 & 0.53/0.60/0.67  & 0.60/0.67/0.70  & 0.50/0.57/0.63 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.15/0.23  & 0.15/0.30/0.38  & 0.10/0.20/0.25 \\ 
 & pi.L1.1 & 0.05/0.08/0.12  & 0.00/0.05/0.10  & 0.05/0.05/0.12 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.55/0.62/0.65  & 0.55/0.65/0.70  & 0.60/0.60/0.65 \\ 
 & pi.L2.1 & 0.25/0.33/0.45  & 0.22/0.40/0.53  & 0.20/0.35/0.48 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.53/0.60/0.67  & 0.60/0.67/0.70  & 0.50/0.57/0.63 \\ 
 & pi.Linf.1 & 0.35/0.50/0.58  & 0.45/0.50/0.53  & 0.37/0.48/0.53 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.concentric(5).mvn.0.1}} & ell.L1 & 0.07/0.13/0.22  & 0.25/0.25/0.33  & 0.17/0.23/0.27 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.53/0.53/0.60  & 0.55/0.58/0.63  & 0.55/0.55/0.60 \\ 
 & ell.L2.1 & 0.05/0.07/0.20  & 0.05/0.12/0.20  & 0.05/0.13/0.17 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.48/0.52/0.55  & 0.55/0.60/0.67  & 0.45/0.50/0.58 \\ 
 & ell.Linf.1 & 0.50/0.52/0.57  & 0.50/0.52/0.55  & 0.45/0.55/0.55 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.07/0.10/0.12  & 0.27/0.40/0.52  & 0.13/0.20/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.07/0.13/0.22  & 0.25/0.25/0.33  & 0.17/0.23/0.27 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.53/0.53/0.55  & 0.68/0.85/0.90  & 0.55/0.55/0.55 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.25/0.35/0.45  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.53/0.53/0.60  & 0.55/0.58/0.63  & 0.55/0.55/0.60 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.53/0.60/0.60  & 0.82/0.92/0.95  & 0.57/0.60/0.65 \\ 
 & Linf.0 & 0.55/0.58/0.67  & 0.90/0.93/0.95  & 0.60/0.65/0.77 \\ 
 & Linf.1 & 0.48/0.52/0.55  & 0.55/0.60/0.67  & 0.45/0.50/0.58 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.07/0.13/0.22  & 0.25/0.25/0.33  & 0.17/0.23/0.27 \\ 
 & pi.L1.1 & 0.00/0.08/0.10  & 0.05/0.10/0.10  & 0.02/0.10/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.53/0.53/0.60  & 0.55/0.58/0.63  & 0.55/0.55/0.60 \\ 
 & pi.L2.1 & 0.15/0.22/0.32  & 0.10/0.18/0.23  & 0.12/0.25/0.25 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.48/0.52/0.55  & 0.55/0.60/0.67  & 0.45/0.50/0.58 \\ 
 & pi.Linf.1 & 0.40/0.42/0.45  & 0.40/0.40/0.43  & 0.35/0.37/0.47 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.25).mvn.0.01}} & ell.L1 & 0.65/0.67/0.70  & 0.62/0.68/0.72  & 0.52/0.63/0.65 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.90/0.95/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & ell.L2.1 & 0.00/0.05/0.12  & 0.00/0.05/0.07  & 0.05/0.05/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.77/0.85/0.85  & 0.90/0.95/1.00  & 0.80/0.80/0.85 \\ 
 & ell.Linf.1 & 0.45/0.52/0.55  & 0.50/0.55/0.55  & 0.47/0.53/0.55 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.62/0.65/0.67  & 0.62/0.68/0.70  & 0.52/0.63/0.65 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.05/0.10/0.15  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.65/0.67/0.70  & 0.62/0.68/0.72  & 0.52/0.63/0.65 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.90/0.92/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.18/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.90/0.95/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.73/0.82/0.83  & 0.90/0.95/0.97  & 0.80/0.80/0.80 \\ 
 & Linf.0 & 0.00/0.00/0.05  & 0.12/0.25/0.40  & 0.02/0.10/0.10 \\ 
 & Linf.1 & 0.77/0.85/0.85  & 0.90/0.95/1.00  & 0.80/0.80/0.85 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.65/0.67/0.70  & 0.62/0.68/0.72  & 0.52/0.63/0.65 \\ 
 & pi.L1.1 & 0.50/0.52/0.58  & 0.37/0.50/0.58  & 0.40/0.55/0.60 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.90/0.95/0.95  & 0.87/0.95/1.00  & 0.90/0.90/0.92 \\ 
 & pi.L2.1 & 0.75/0.77/0.80  & 0.70/0.77/0.80  & 0.70/0.77/0.80 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.77/0.85/0.85  & 0.90/0.95/1.00  & 0.80/0.80/0.85 \\ 
 & pi.Linf.1 & 0.70/0.70/0.75  & 0.63/0.77/0.80  & 0.70/0.72/0.77 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.25).mvn.0.05}} & ell.L1 & 0.10/0.10/0.17  & 0.20/0.25/0.30  & 0.15/0.17/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.50/0.53/0.55  & 0.60/0.75/0.85  & 0.62/0.67/0.68 \\ 
 & ell.L2.1 & 0.00/0.02/0.03  & 0.00/0.02/0.03  & 0.00/0.05/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.50/0.65/0.67  & 0.70/0.70/0.80  & 0.70/0.72/0.75 \\ 
 & ell.Linf.1 & 0.30/0.37/0.50  & 0.30/0.42/0.58  & 0.40/0.48/0.53 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.10/0.10  & 0.30/0.38/0.40  & 0.15/0.15/0.17 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.30/0.38  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.10/0.17  & 0.20/0.25/0.30  & 0.15/0.17/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.50/0.53/0.53  & 0.70/0.80/0.92  & 0.62/0.65/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.35/0.43/0.55  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.50/0.53/0.55  & 0.60/0.75/0.85  & 0.62/0.67/0.68 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.47/0.63/0.67  & 0.73/0.78/0.82  & 0.55/0.70/0.73 \\ 
 & Linf.0 & 0.15/0.23/0.25  & 0.35/0.43/0.47  & 0.25/0.27/0.30 \\ 
 & Linf.1 & 0.50/0.65/0.67  & 0.70/0.70/0.80  & 0.70/0.72/0.75 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.10/0.17  & 0.20/0.25/0.30  & 0.15/0.17/0.25 \\ 
 & pi.L1.1 & 0.10/0.23/0.30  & 0.05/0.15/0.23  & 0.10/0.13/0.28 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.50/0.53/0.55  & 0.60/0.75/0.85  & 0.62/0.67/0.68 \\ 
 & pi.L2.1 & 0.30/0.45/0.57  & 0.22/0.37/0.52  & 0.30/0.47/0.62 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.50/0.65/0.67  & 0.70/0.70/0.80  & 0.70/0.72/0.75 \\ 
 & pi.Linf.1 & 0.50/0.65/0.67  & 0.53/0.65/0.70  & 0.55/0.65/0.73 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.25).mvn.0.1}} & ell.L1 & 0.05/0.10/0.13  & 0.10/0.13/0.17  & 0.05/0.10/0.13 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.10/0.17  & 0.13/0.30/0.33  & 0.15/0.15/0.22 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.00/0.02/0.08  & 0.00/0.00/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.20/0.32/0.48  & 0.32/0.48/0.67  & 0.25/0.48/0.55 \\ 
 & ell.Linf.1 & 0.10/0.22/0.32  & 0.15/0.25/0.28  & 0.17/0.23/0.33 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.08/0.10  & 0.33/0.48/0.53  & 0.05/0.10/0.10 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.43/0.47/0.55  & 0.00/0.02/0.12 \\ 
 & L1.1 & 0.05/0.10/0.13  & 0.10/0.13/0.17  & 0.05/0.10/0.13 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.05/0.08/0.13  & 0.47/0.68/0.77  & 0.15/0.17/0.22 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.65/0.75/0.82  & 0.00/0.05/0.08 \\ 
 & L2.1 & 0.05/0.10/0.17  & 0.13/0.30/0.33  & 0.15/0.15/0.22 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.30/0.40/0.43  & 0.42/0.55/0.70  & 0.30/0.43/0.55 \\ 
 & Linf.0 & 0.25/0.27/0.30  & 0.30/0.38/0.45  & 0.25/0.30/0.37 \\ 
 & Linf.1 & 0.20/0.32/0.48  & 0.32/0.48/0.67  & 0.25/0.48/0.55 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.10/0.13  & 0.10/0.13/0.17  & 0.05/0.10/0.13 \\ 
 & pi.L1.1 & 0.07/0.12/0.15  & 0.05/0.10/0.10  & 0.05/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.10/0.17  & 0.13/0.30/0.33  & 0.15/0.15/0.22 \\ 
 & pi.L2.1 & 0.07/0.12/0.17  & 0.05/0.12/0.15  & 0.05/0.15/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.20/0.32/0.48  & 0.32/0.48/0.67  & 0.25/0.48/0.55 \\ 
 & pi.Linf.1 & 0.32/0.37/0.40  & 0.22/0.28/0.35  & 0.15/0.25/0.27 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.5).mvn.0.01}} & ell.L1 & 0.60/0.65/0.65  & 0.70/0.75/0.75  & 0.70/0.73/0.75 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.90/0.90/0.90  & 0.90/0.90/0.92  & 0.90/0.90/0.90 \\ 
 & ell.L2.1 & 0.00/0.02/0.08  & 0.00/0.07/0.10  & 0.02/0.05/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.90/0.90/0.90  & 0.87/0.87/0.88  & 0.83/0.83/0.83 \\ 
 & ell.Linf.1 & 0.32/0.45/0.53  & 0.30/0.43/0.55  & 0.37/0.45/0.48 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.60/0.65/0.65  & 0.70/0.78/0.80  & 0.70/0.73/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.07/0.17/0.25  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.60/0.65/0.65  & 0.70/0.75/0.75  & 0.70/0.73/0.75 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.90/0.90/0.90  & 1.00/1.00/1.00  & 0.90/0.90/0.90 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.15/0.20/0.20  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.90/0.90/0.90  & 0.90/0.90/0.92  & 0.90/0.90/0.90 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.92/0.95/0.95  & 0.97/0.97/0.97  & 0.83/0.88/0.90 \\ 
 & Linf.0 & 0.05/0.10/0.15  & 0.32/0.45/0.50  & 0.12/0.23/0.32 \\ 
 & Linf.1 & 0.90/0.90/0.90  & 0.87/0.87/0.88  & 0.83/0.83/0.83 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.60/0.65/0.65  & 0.70/0.75/0.75  & 0.70/0.73/0.75 \\ 
 & pi.L1.1 & 0.70/0.82/0.90  & 0.67/0.78/0.82  & 0.68/0.78/0.87 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.90/0.90/0.90  & 0.90/0.90/0.92  & 0.90/0.90/0.90 \\ 
 & pi.L2.1 & 0.80/0.85/0.90  & 0.83/0.85/0.87  & 0.83/0.85/0.88 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.90/0.90/0.90  & 0.87/0.87/0.88  & 0.83/0.83/0.83 \\ 
 & pi.Linf.1 & 0.58/0.68/0.85  & 0.65/0.72/0.72  & 0.53/0.72/0.78 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.5).mvn.0.05}} & ell.L1 & 0.10/0.17/0.30  & 0.25/0.35/0.40  & 0.05/0.10/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.42/0.55/0.62  & 0.57/0.65/0.72  & 0.47/0.53/0.63 \\ 
 & ell.L2.1 & 0.03/0.05/0.10  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.55/0.55/0.70  & 0.68/0.72/0.72  & 0.53/0.68/0.70 \\ 
 & ell.Linf.1 & 0.25/0.38/0.43  & 0.30/0.35/0.40  & 0.30/0.35/0.40 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.12/0.20  & 0.40/0.45/0.53  & 0.05/0.10/0.10 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.30/0.42/0.47  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.17/0.30  & 0.25/0.35/0.40  & 0.05/0.10/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.37/0.53/0.55  & 0.82/0.85/0.87  & 0.47/0.53/0.62 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.37/0.43/0.50  & 0.00/0.02/0.05 \\ 
 & L2.1 & 0.42/0.55/0.62  & 0.57/0.65/0.72  & 0.47/0.53/0.63 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.53/0.62/0.77  & 0.73/0.97/0.97  & 0.55/0.68/0.73 \\ 
 & Linf.0 & 0.07/0.33/0.42  & 0.38/0.57/0.62  & 0.30/0.32/0.40 \\ 
 & Linf.1 & 0.55/0.55/0.70  & 0.68/0.72/0.72  & 0.53/0.68/0.70 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.17/0.30  & 0.25/0.35/0.40  & 0.05/0.10/0.25 \\ 
 & pi.L1.1 & 0.17/0.28/0.33  & 0.12/0.18/0.33  & 0.05/0.07/0.20 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.42/0.55/0.62  & 0.57/0.65/0.72  & 0.47/0.53/0.63 \\ 
 & pi.L2.1 & 0.22/0.33/0.40  & 0.25/0.37/0.48  & 0.15/0.18/0.33 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.55/0.55/0.70  & 0.68/0.72/0.72  & 0.53/0.68/0.70 \\ 
 & pi.Linf.1 & 0.47/0.60/0.62  & 0.42/0.55/0.57  & 0.45/0.52/0.58 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(0.5).mvn.0.1}} & ell.L1 & 0.00/0.03/0.05  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.03/0.08  & 0.02/0.12/0.18  & 0.05/0.05/0.08 \\ 
 & ell.L2.1 & 0.00/0.00/0.07  & 0.00/0.05/0.07  & 0.05/0.05/0.12 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.17/0.23/0.33  & 0.30/0.37/0.57  & 0.25/0.33/0.37 \\ 
 & ell.Linf.1 & 0.22/0.30/0.33  & 0.20/0.33/0.42  & 0.30/0.35/0.38 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.03  & 0.18/0.50/0.55  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.48/0.52/0.57  & 0.00/0.00/0.05 \\ 
 & L1.1 & 0.00/0.03/0.05  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.03/0.07  & 0.40/0.72/0.77  & 0.05/0.12/0.15 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.70/0.75/0.77  & 0.00/0.08/0.13 \\ 
 & L2.1 & 0.00/0.03/0.08  & 0.02/0.12/0.18  & 0.05/0.05/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.28/0.30  & 0.27/0.37/0.57  & 0.25/0.30/0.37 \\ 
 & Linf.0 & 0.20/0.22/0.25  & 0.25/0.43/0.57  & 0.25/0.28/0.38 \\ 
 & Linf.1 & 0.17/0.23/0.33  & 0.30/0.37/0.57  & 0.25/0.33/0.37 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.03/0.05  & 0.00/0.05/0.10  & 0.05/0.05/0.07 \\ 
 & pi.L1.1 & 0.00/0.08/0.15  & 0.02/0.08/0.10  & 0.05/0.08/0.13 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.03/0.08  & 0.02/0.12/0.18  & 0.05/0.05/0.08 \\ 
 & pi.L2.1 & 0.00/0.08/0.15  & 0.02/0.08/0.10  & 0.05/0.08/0.17 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.17/0.23/0.33  & 0.30/0.37/0.57  & 0.25/0.33/0.37 \\ 
 & pi.Linf.1 & 0.23/0.25/0.37  & 0.25/0.27/0.35  & 0.25/0.27/0.32 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1.5).mvn.0.01}} & ell.L1 & 0.70/0.75/0.78  & 0.80/0.93/0.95  & 0.80/0.80/0.92 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.85/0.93/0.95  & 0.95/0.98/1.00  & 0.85/0.95/0.98 \\ 
 & ell.L2.1 & 0.15/0.25/0.30  & 0.15/0.20/0.32  & 0.13/0.22/0.27 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.85/0.87/0.87  & 0.90/0.93/0.95  & 0.80/0.83/0.85 \\ 
 & ell.Linf.1 & 0.45/0.45/0.47  & 0.45/0.48/0.50  & 0.40/0.43/0.50 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.70/0.75/0.77  & 0.80/0.85/0.90  & 0.80/0.80/0.80 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.13/0.15  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.70/0.75/0.78  & 0.80/0.93/0.95  & 0.80/0.80/0.92 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.85/0.95/1.00  & 1.00/1.00/1.00  & 0.85/0.95/0.95 \\ 
 & L2.0 & 0.00/0.05/0.05  & 0.25/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.85/0.93/0.95  & 0.95/0.98/1.00  & 0.85/0.95/0.98 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.95/0.95/0.95  & 0.98/1.00/1.00  & 0.80/0.88/0.93 \\ 
 & Linf.0 & 0.10/0.12/0.20  & 0.17/0.32/0.45  & 0.07/0.15/0.20 \\ 
 & Linf.1 & 0.85/0.87/0.87  & 0.90/0.93/0.95  & 0.80/0.83/0.85 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.70/0.75/0.78  & 0.80/0.93/0.95  & 0.80/0.80/0.92 \\ 
 & pi.L1.1 & 0.80/0.88/0.90  & 0.80/0.87/0.90  & 0.80/0.85/0.88 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.85/0.93/0.95  & 0.95/0.98/1.00  & 0.85/0.95/0.98 \\ 
 & pi.L2.1 & 0.80/0.88/0.92  & 0.80/0.87/0.95  & 0.75/0.83/0.88 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.85/0.87/0.87  & 0.90/0.93/0.95  & 0.80/0.83/0.85 \\ 
 & pi.Linf.1 & 0.75/0.75/0.80  & 0.77/0.83/0.85  & 0.75/0.75/0.75 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1.5).mvn.0.05}} & ell.L1 & 0.42/0.50/0.55  & 0.50/0.65/0.65  & 0.50/0.57/0.67 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.85/0.85/0.85  & 0.87/0.90/0.93  & 0.75/0.78/0.88 \\ 
 & ell.L2.1 & 0.05/0.05/0.10  & 0.00/0.05/0.08  & 0.00/0.07/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.75/0.75/0.80  & 0.80/0.83/0.83  & 0.55/0.75/0.75 \\ 
 & ell.Linf.1 & 0.43/0.48/0.53  & 0.40/0.48/0.52  & 0.45/0.45/0.50 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.38/0.50/0.50  & 0.60/0.75/0.75  & 0.48/0.52/0.58 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.20/0.28/0.30  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.42/0.50/0.55  & 0.50/0.65/0.65  & 0.50/0.57/0.67 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.85/0.85/0.85  & 0.95/1.00/1.00  & 0.75/0.78/0.82 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.25/0.27/0.27  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.85/0.85/0.85  & 0.87/0.90/0.93  & 0.75/0.78/0.88 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.58/0.75/0.80  & 0.78/0.88/0.88  & 0.55/0.68/0.75 \\ 
 & Linf.0 & 0.05/0.10/0.10  & 0.20/0.25/0.27  & 0.15/0.15/0.15 \\ 
 & Linf.1 & 0.75/0.75/0.80  & 0.80/0.83/0.83  & 0.55/0.75/0.75 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.42/0.50/0.55  & 0.50/0.65/0.65  & 0.50/0.57/0.67 \\ 
 & pi.L1.1 & 0.37/0.50/0.60  & 0.25/0.53/0.58  & 0.42/0.53/0.65 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.85/0.85/0.85  & 0.87/0.90/0.93  & 0.75/0.78/0.88 \\ 
 & pi.L2.1 & 0.62/0.73/0.77  & 0.58/0.73/0.78  & 0.70/0.73/0.82 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.75/0.75/0.80  & 0.80/0.83/0.83  & 0.55/0.75/0.75 \\ 
 & pi.Linf.1 & 0.65/0.65/0.70  & 0.50/0.67/0.68  & 0.50/0.65/0.65 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1.5).mvn.0.1}} & ell.L1 & 0.18/0.27/0.35  & 0.20/0.30/0.38  & 0.10/0.23/0.28 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.57/0.65/0.65  & 0.65/0.75/0.75  & 0.50/0.65/0.68 \\ 
 & ell.L2.1 & 0.05/0.25/0.32  & 0.15/0.22/0.30  & 0.07/0.20/0.30 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.55/0.65/0.68  & 0.57/0.68/0.70  & 0.55/0.65/0.70 \\ 
 & ell.Linf.1 & 0.42/0.48/0.50  & 0.45/0.47/0.53  & 0.45/0.47/0.53 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.17/0.27/0.30  & 0.27/0.55/0.65  & 0.10/0.18/0.27 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.30/0.42/0.45  & 0.00/0.02/0.03 \\ 
 & L1.1 & 0.18/0.27/0.35  & 0.20/0.30/0.38  & 0.10/0.23/0.28 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.57/0.62/0.65  & 0.67/0.93/0.95  & 0.50/0.63/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.32/0.38/0.40  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.57/0.65/0.65  & 0.65/0.75/0.75  & 0.50/0.65/0.68 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.53/0.58/0.67  & 0.62/0.73/0.78  & 0.55/0.58/0.65 \\ 
 & Linf.0 & 0.12/0.15/0.17  & 0.30/0.43/0.53  & 0.15/0.20/0.23 \\ 
 & Linf.1 & 0.55/0.65/0.68  & 0.57/0.68/0.70  & 0.55/0.65/0.70 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.18/0.27/0.35  & 0.20/0.30/0.38  & 0.10/0.23/0.28 \\ 
 & pi.L1.1 & 0.12/0.20/0.20  & 0.10/0.20/0.22  & 0.08/0.20/0.22 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.57/0.65/0.65  & 0.65/0.75/0.75  & 0.50/0.65/0.68 \\ 
 & pi.L2.1 & 0.37/0.45/0.50  & 0.20/0.47/0.50  & 0.25/0.40/0.50 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.55/0.65/0.68  & 0.57/0.68/0.70  & 0.55/0.65/0.70 \\ 
 & pi.Linf.1 & 0.47/0.50/0.58  & 0.40/0.50/0.55  & 0.45/0.53/0.58 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1).mvn.0.01}} & ell.L1 & 0.65/0.68/0.72  & 0.65/0.70/0.90  & 0.60/0.67/0.72 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.85/0.92/0.95  & 0.88/0.92/1.00  & 0.80/0.92/0.95 \\ 
 & ell.L2.1 & 0.10/0.15/0.28  & 0.12/0.18/0.20  & 0.05/0.12/0.22 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.78/0.80/0.82  & 0.83/0.88/0.90  & 0.70/0.78/0.82 \\ 
 & ell.Linf.1 & 0.40/0.45/0.53  & 0.45/0.47/0.50  & 0.42/0.47/0.48 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.65/0.67/0.70  & 0.65/0.73/0.82  & 0.60/0.67/0.67 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.10/0.20/0.20  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.65/0.68/0.72  & 0.65/0.70/0.90  & 0.60/0.67/0.72 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.85/0.90/0.93  & 0.98/1.00/1.00  & 0.80/0.88/0.92 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.25/0.25/0.25  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.85/0.92/0.95  & 0.88/0.92/1.00  & 0.80/0.92/0.95 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.77/0.80/0.87  & 0.88/0.93/0.95  & 0.65/0.73/0.83 \\ 
 & Linf.0 & 0.15/0.20/0.23  & 0.15/0.30/0.45  & 0.02/0.10/0.17 \\ 
 & Linf.1 & 0.78/0.80/0.82  & 0.83/0.88/0.90  & 0.70/0.78/0.82 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.65/0.68/0.72  & 0.65/0.70/0.90  & 0.60/0.67/0.72 \\ 
 & pi.L1.1 & 0.75/0.78/0.80  & 0.75/0.80/0.80  & 0.70/0.82/0.87 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.85/0.92/0.95  & 0.88/0.92/1.00  & 0.80/0.92/0.95 \\ 
 & pi.L2.1 & 0.80/0.83/0.85  & 0.80/0.82/0.85  & 0.75/0.85/0.87 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.78/0.80/0.82  & 0.83/0.88/0.90  & 0.70/0.78/0.82 \\ 
 & pi.Linf.1 & 0.55/0.60/0.73  & 0.62/0.70/0.72  & 0.50/0.68/0.75 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1).mvn.0.05}} & ell.L1 & 0.32/0.40/0.42  & 0.42/0.52/0.58  & 0.37/0.45/0.52 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.62/0.70/0.70  & 0.77/0.80/0.88  & 0.63/0.78/0.83 \\ 
 & ell.L2.1 & 0.02/0.10/0.15  & 0.05/0.07/0.10  & 0.05/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.47/0.63/0.73  & 0.62/0.73/0.77  & 0.43/0.67/0.80 \\ 
 & ell.Linf.1 & 0.30/0.30/0.30  & 0.30/0.30/0.30  & 0.35/0.35/0.37 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.27/0.35/0.40  & 0.45/0.57/0.63  & 0.35/0.45/0.45 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.25/0.30/0.35  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.32/0.40/0.42  & 0.42/0.52/0.58  & 0.37/0.45/0.52 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.62/0.68/0.70  & 0.85/0.93/0.95  & 0.63/0.77/0.82 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.32/0.40/0.40  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.62/0.70/0.70  & 0.77/0.80/0.88  & 0.63/0.78/0.83 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.38/0.53/0.62  & 0.55/0.80/0.88  & 0.42/0.55/0.67 \\ 
 & Linf.0 & 0.00/0.10/0.15  & 0.10/0.28/0.37  & 0.15/0.15/0.18 \\ 
 & Linf.1 & 0.47/0.63/0.73  & 0.62/0.73/0.77  & 0.43/0.67/0.80 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.32/0.40/0.42  & 0.42/0.52/0.58  & 0.37/0.45/0.52 \\ 
 & pi.L1.1 & 0.15/0.30/0.42  & 0.20/0.30/0.47  & 0.17/0.35/0.47 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.62/0.70/0.70  & 0.77/0.80/0.88  & 0.63/0.78/0.83 \\ 
 & pi.L2.1 & 0.38/0.52/0.65  & 0.43/0.65/0.70  & 0.38/0.62/0.72 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.47/0.63/0.73  & 0.62/0.73/0.77  & 0.43/0.67/0.80 \\ 
 & pi.Linf.1 & 0.40/0.52/0.60  & 0.45/0.50/0.53  & 0.42/0.52/0.60 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(1).mvn.0.1}} & ell.L1 & 0.00/0.07/0.17  & 0.02/0.18/0.23  & 0.00/0.03/0.10 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.03/0.12/0.18  & 0.08/0.28/0.33  & 0.00/0.17/0.23 \\ 
 & ell.L2.1 & 0.05/0.20/0.28  & 0.12/0.17/0.18  & 0.00/0.00/0.20 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.23/0.37/0.37  & 0.35/0.37/0.42  & 0.27/0.37/0.37 \\ 
 & ell.Linf.1 & 0.17/0.27/0.38  & 0.20/0.20/0.33  & 0.20/0.23/0.30 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.05/0.12  & 0.18/0.38/0.50  & 0.00/0.03/0.13 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.33/0.53/0.58  & 0.02/0.05/0.05 \\ 
 & L1.1 & 0.00/0.07/0.17  & 0.02/0.18/0.23  & 0.00/0.03/0.10 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.03/0.10/0.13  & 0.42/0.65/0.73  & 0.00/0.17/0.18 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.50/0.60/0.62  & 0.00/0.00/0.05 \\ 
 & L2.1 & 0.03/0.12/0.18  & 0.08/0.28/0.33  & 0.00/0.17/0.23 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.43/0.50  & 0.50/0.67/0.70  & 0.28/0.37/0.45 \\ 
 & Linf.0 & 0.20/0.20/0.38  & 0.52/0.62/0.67  & 0.20/0.28/0.45 \\ 
 & Linf.1 & 0.23/0.37/0.37  & 0.35/0.37/0.42  & 0.27/0.37/0.37 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.07/0.17  & 0.02/0.18/0.23  & 0.00/0.03/0.10 \\ 
 & pi.L1.1 & 0.00/0.05/0.17  & 0.00/0.08/0.17  & 0.02/0.07/0.15 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.03/0.12/0.18  & 0.08/0.28/0.33  & 0.00/0.17/0.23 \\ 
 & pi.L2.1 & 0.02/0.17/0.25  & 0.05/0.17/0.25  & 0.05/0.08/0.20 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.23/0.37/0.37  & 0.35/0.37/0.42  & 0.27/0.37/0.37 \\ 
 & pi.Linf.1 & 0.25/0.32/0.35  & 0.25/0.27/0.32  & 0.27/0.32/0.35 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(5).mvn.0.01}} & ell.L1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & ell.L2.1 & 0.10/0.10/0.15  & 0.10/0.10/0.10  & 0.05/0.10/0.10 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.92/0.95/0.95  & 0.87/0.90/0.90  & 0.85/0.85/0.88 \\ 
 & ell.Linf.1 & 0.30/0.32/0.35  & 0.30/0.30/0.30  & 0.30/0.33/0.35 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.10/0.15  & 0.00/0.00/0.00 \\ 
 & L2.1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.95/0.95/0.95  & 0.93/1.00/1.00  & 0.82/0.85/0.85 \\ 
 & Linf.0 & 0.05/0.07/0.15  & 0.25/0.38/0.48  & 0.00/0.00/0.05 \\ 
 & Linf.1 & 0.92/0.95/0.95  & 0.87/0.90/0.90  & 0.85/0.85/0.88 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.90/0.98/0.98 \\ 
 & pi.L1.1 & 0.88/1.00/1.00  & 0.87/0.93/1.00  & 0.92/0.97/1.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 1.00/1.00/1.00  & 0.93/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & pi.L2.1 & 0.87/0.98/1.00  & 0.87/0.93/1.00  & 0.92/0.95/1.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.92/0.95/0.95  & 0.87/0.90/0.90  & 0.85/0.85/0.88 \\ 
 & pi.Linf.1 & 0.77/0.82/0.82  & 0.80/0.80/0.80  & 0.80/0.80/0.80 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(5).mvn.0.05}} & ell.L1 & 0.70/0.70/0.70  & 0.72/0.83/0.87  & 0.70/0.73/0.82 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & ell.L2.1 & 0.12/0.23/0.25  & 0.20/0.23/0.27  & 0.20/0.27/0.32 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.95/0.95/0.95  & 0.95/0.95/0.95  & 0.90/0.90/0.90 \\ 
 & ell.Linf.1 & 0.35/0.38/0.40  & 0.40/0.43/0.47  & 0.45/0.45/0.45 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.70/0.70/0.70  & 0.72/0.83/0.83  & 0.70/0.72/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.70/0.70/0.70  & 0.72/0.83/0.87  & 0.70/0.73/0.82 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.02/0.12/0.13  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.92/0.95/0.95  & 0.95/0.95/0.98  & 0.90/0.90/0.90 \\ 
 & Linf.0 & 0.00/0.02/0.07  & 0.10/0.15/0.30  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.95/0.95/0.95  & 0.95/0.95/0.95  & 0.90/0.90/0.90 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.70/0.70/0.70  & 0.72/0.83/0.87  & 0.70/0.73/0.82 \\ 
 & pi.L1.1 & 0.90/0.95/0.95  & 0.88/0.95/0.95  & 0.95/0.95/0.95 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.95/0.95/0.95  & 0.95/0.95/0.98  & 0.95/0.95/0.95 \\ 
 & pi.L2.1 & 0.92/0.95/0.95  & 0.88/0.95/0.95  & 0.95/0.95/0.95 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.95/0.95/0.95  & 0.95/0.95/0.95  & 0.90/0.90/0.90 \\ 
 & pi.Linf.1 & 0.85/0.90/0.95  & 0.82/0.87/0.95  & 0.80/0.85/0.85 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.fig8(5).mvn.0.1}} & ell.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & ell.L2.1 & 0.00/0.07/0.15  & 0.00/0.05/0.12  & 0.00/0.03/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.87/0.90/0.95  & 0.83/0.87/0.88  & 0.85/0.88/0.97 \\ 
 & ell.Linf.1 & 0.40/0.42/0.45  & 0.37/0.43/0.50  & 0.35/0.40/0.47 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.00/0.05/0.05  & 0.00/0.00/0.00 \\ 
 & L2.1 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.80/0.83/0.90  & 0.85/0.93/0.97  & 0.80/0.88/0.92 \\ 
 & Linf.0 & 0.00/0.00/0.02  & 0.07/0.23/0.30  & 0.00/0.00/0.02 \\ 
 & Linf.1 & 0.87/0.90/0.95  & 0.83/0.87/0.88  & 0.85/0.88/0.97 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.70/0.75/0.75 \\ 
 & pi.L1.1 & 0.72/0.75/0.83  & 0.75/0.77/0.83  & 0.70/0.82/0.88 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.92/0.98/1.00 \\ 
 & pi.L2.1 & 0.82/0.83/0.92  & 0.85/0.87/0.90  & 0.80/0.88/0.98 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.87/0.90/0.95  & 0.83/0.87/0.88  & 0.85/0.88/0.97 \\ 
 & pi.Linf.1 & 0.80/0.80/0.82  & 0.75/0.75/0.75  & 0.75/0.78/0.80 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(2).mvn.0.01}} & ell.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & ell.L2.1 & 0.00/0.05/0.18  & 0.05/0.13/0.25  & 0.03/0.10/0.23 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 1.00/1.00/1.00  & 0.85/0.85/0.85  & 0.90/0.93/0.95 \\ 
 & ell.Linf.1 & 0.52/0.60/0.60  & 0.55/0.60/0.60  & 0.50/0.55/0.60 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.05/0.12/0.17  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.10/0.17/0.20  & 0.00/0.00/0.00 \\ 
 & L2.1 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 1.00/1.00/1.00  & 0.90/0.90/0.93  & 0.90/0.93/0.95 \\ 
 & Linf.0 & 0.02/0.10/0.10  & 0.10/0.15/0.20  & 0.05/0.07/0.12 \\ 
 & Linf.1 & 1.00/1.00/1.00  & 0.85/0.85/0.85  & 0.90/0.93/0.95 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.75/0.75/0.75  & 0.75/0.75/0.75  & 0.68/0.73/0.75 \\ 
 & pi.L1.1 & 0.70/0.83/0.85  & 0.80/0.80/0.80  & 0.70/0.77/0.80 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 & pi.L2.1 & 0.95/1.00/1.00  & 1.00/1.00/1.00  & 0.95/1.00/1.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 1.00/1.00/1.00  & 0.85/0.85/0.85  & 0.90/0.93/0.95 \\ 
 & pi.Linf.1 & 0.90/0.95/1.00  & 0.80/0.80/0.85  & 0.85/0.88/0.93 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(2).mvn.0.05}} & ell.L1 & 0.10/0.17/0.20  & 0.13/0.27/0.32  & 0.10/0.18/0.28 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.40/0.52/0.58  & 0.67/0.75/0.78  & 0.55/0.63/0.77 \\ 
 & ell.L2.1 & 0.05/0.10/0.15  & 0.05/0.05/0.10  & 0.00/0.03/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.57/0.70/0.72  & 0.72/0.78/0.80  & 0.68/0.80/0.80 \\ 
 & ell.Linf.1 & 0.30/0.38/0.43  & 0.35/0.40/0.47  & 0.30/0.43/0.48 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.13/0.17  & 0.17/0.28/0.40  & 0.10/0.15/0.17 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.25/0.37/0.47  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.17/0.20  & 0.13/0.27/0.32  & 0.10/0.18/0.28 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.38/0.50/0.57  & 0.67/0.82/0.88  & 0.55/0.60/0.65 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.23/0.37/0.52  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.40/0.52/0.58  & 0.67/0.75/0.78  & 0.55/0.63/0.77 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.52/0.67/0.72  & 0.73/0.82/0.87  & 0.68/0.80/0.83 \\ 
 & Linf.0 & 0.10/0.17/0.23  & 0.30/0.33/0.48  & 0.22/0.28/0.35 \\ 
 & Linf.1 & 0.57/0.70/0.72  & 0.72/0.78/0.80  & 0.68/0.80/0.80 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.17/0.20  & 0.13/0.27/0.32  & 0.10/0.18/0.28 \\ 
 & pi.L1.1 & 0.10/0.25/0.33  & 0.20/0.23/0.32  & 0.22/0.25/0.27 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.40/0.52/0.58  & 0.67/0.75/0.78  & 0.55/0.63/0.77 \\ 
 & pi.L2.1 & 0.30/0.42/0.53  & 0.30/0.43/0.60  & 0.35/0.43/0.58 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.57/0.70/0.72  & 0.72/0.78/0.80  & 0.68/0.80/0.80 \\ 
 & pi.Linf.1 & 0.55/0.65/0.65  & 0.60/0.70/0.70  & 0.65/0.65/0.70 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(2).mvn.0.1}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.02/0.08  & 0.15/0.18/0.30  & 0.05/0.13/0.22 \\ 
 & ell.L2.1 & 0.07/0.13/0.20  & 0.00/0.02/0.10  & 0.00/0.12/0.20 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.12/0.17/0.27  & 0.28/0.53/0.58  & 0.28/0.37/0.47 \\ 
 & ell.Linf.1 & 0.27/0.32/0.38  & 0.25/0.30/0.33  & 0.20/0.25/0.38 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.38/0.62/0.65  & 0.00/0.00/0.00 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.58/0.67/0.70  & 0.00/0.00/0.03 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.02  & 0.75/0.87/0.90  & 0.08/0.15/0.30 \\ 
 & L2.0 & 0.00/0.02/0.05  & 0.70/0.85/0.85  & 0.05/0.20/0.27 \\ 
 & L2.1 & 0.00/0.02/0.08  & 0.15/0.18/0.30  & 0.05/0.13/0.22 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.37/0.37  & 0.50/0.63/0.75  & 0.28/0.38/0.57 \\ 
 & Linf.0 & 0.23/0.32/0.37  & 0.40/0.53/0.67  & 0.25/0.37/0.50 \\ 
 & Linf.1 & 0.12/0.17/0.27  & 0.28/0.53/0.58  & 0.28/0.37/0.47 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.08  & 0.00/0.00/0.03 \\ 
 & pi.L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.00/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.02/0.08  & 0.15/0.18/0.30  & 0.05/0.13/0.22 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.00/0.05  & 0.00/0.02/0.15 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.12/0.17/0.27  & 0.28/0.53/0.58  & 0.28/0.37/0.47 \\ 
 & pi.Linf.1 & 0.25/0.40/0.43  & 0.25/0.35/0.42  & 0.27/0.33/0.40 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(3).mvn.0.01}} & ell.L1 & 0.25/0.38/0.53  & 0.53/0.62/0.75  & 0.05/0.22/0.25 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.18/0.38/0.57  & 0.63/0.68/0.82  & 0.05/0.13/0.23 \\ 
 & ell.L2.1 & 0.02/0.12/0.15  & 0.05/0.10/0.15  & 0.07/0.13/0.15 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.12/0.23/0.40  & 0.58/0.77/0.95  & 0.10/0.17/0.22 \\ 
 & ell.Linf.1 & 0.05/0.12/0.20  & 0.07/0.15/0.20  & 0.08/0.08/0.18 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.20/0.33/0.47  & 0.75/0.75/0.75  & 0.03/0.13/0.20 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.75/0.75/0.75  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.25/0.38/0.53  & 0.53/0.62/0.75  & 0.05/0.22/0.25 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.13/0.28/0.47  & 0.75/0.75/0.75  & 0.05/0.10/0.13 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.75/0.75/0.75  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.18/0.38/0.57  & 0.63/0.68/0.82  & 0.05/0.13/0.23 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.12/0.22/0.30  & 0.62/0.68/0.82  & 0.10/0.10/0.18 \\ 
 & Linf.0 & 0.02/0.05/0.05  & 0.33/0.43/0.48  & 0.00/0.00/0.00 \\ 
 & Linf.1 & 0.12/0.23/0.40  & 0.58/0.77/0.95  & 0.10/0.17/0.22 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.25/0.38/0.53  & 0.53/0.62/0.75  & 0.05/0.22/0.25 \\ 
 & pi.L1.1 & 0.40/0.45/0.58  & 0.20/0.48/0.58  & 0.48/0.53/0.60 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.18/0.38/0.57  & 0.63/0.68/0.82  & 0.05/0.13/0.23 \\ 
 & pi.L2.1 & 0.35/0.45/0.58  & 0.20/0.43/0.58  & 0.48/0.53/0.60 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.12/0.23/0.40  & 0.58/0.77/0.95  & 0.10/0.17/0.22 \\ 
 & pi.Linf.1 & 0.13/0.40/0.58  & 0.17/0.37/0.52  & 0.25/0.37/0.57 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(3).mvn.0.05}} & ell.L1 & 0.10/0.15/0.15  & 0.45/0.47/0.58  & 0.03/0.10/0.18 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.08/0.10/0.13  & 0.43/0.53/0.62  & 0.00/0.08/0.15 \\ 
 & ell.L2.1 & 0.05/0.07/0.17  & 0.07/0.12/0.17  & 0.10/0.10/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.07  & 0.33/0.42/0.45  & 0.00/0.00/0.03 \\ 
 & ell.Linf.1 & 0.05/0.08/0.15  & 0.05/0.08/0.10  & 0.00/0.07/0.12 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.10/0.10/0.10  & 0.92/0.93/0.95  & 0.02/0.05/0.12 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.95/0.95/0.97  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.10/0.15/0.15  & 0.45/0.47/0.58  & 0.03/0.10/0.18 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.08/0.10/0.10  & 0.95/1.00/1.00  & 0.00/0.02/0.07 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.97/1.00/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.08/0.10/0.13  & 0.43/0.53/0.62  & 0.00/0.08/0.15 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.03/0.07/0.10  & 0.45/0.70/0.88  & 0.10/0.10/0.18 \\ 
 & Linf.0 & 0.05/0.05/0.05  & 0.38/0.63/0.80  & 0.12/0.18/0.23 \\ 
 & Linf.1 & 0.05/0.05/0.07  & 0.33/0.42/0.45  & 0.00/0.00/0.03 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.15/0.15  & 0.45/0.47/0.58  & 0.03/0.10/0.18 \\ 
 & pi.L1.1 & 0.15/0.27/0.37  & 0.12/0.18/0.37  & 0.15/0.28/0.38 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.08/0.10/0.13  & 0.43/0.53/0.62  & 0.00/0.08/0.15 \\ 
 & pi.L2.1 & 0.15/0.25/0.38  & 0.13/0.25/0.35  & 0.15/0.25/0.38 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.07  & 0.33/0.42/0.45  & 0.00/0.00/0.03 \\ 
 & pi.Linf.1 & 0.05/0.07/0.28  & 0.05/0.12/0.32  & 0.10/0.15/0.28 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.sphere(3).mvn.0.1}} & ell.L1 & 0.00/0.00/0.02  & 0.02/0.13/0.30  & 0.00/0.05/0.07 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.05  & 0.07/0.18/0.35  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.02/0.05/0.08  & 0.00/0.03/0.05  & 0.00/0.05/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.02/0.05  & 0.07/0.20/0.32  & 0.00/0.00/0.00 \\ 
 & ell.Linf.1 & 0.00/0.02/0.08  & 0.00/0.02/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.80/0.90/0.95  & 0.00/0.00/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.85/0.95/0.95  & 0.00/0.00/0.00 \\ 
 & L1.1 & 0.00/0.00/0.02  & 0.02/0.13/0.30  & 0.00/0.05/0.07 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.00/0.00/0.00  & 0.95/0.95/0.98  & 0.00/0.00/0.00 \\ 
 & L2.0 & 0.00/0.00/0.00  & 0.97/0.98/1.00  & 0.00/0.00/0.00 \\ 
 & L2.1 & 0.00/0.00/0.05  & 0.07/0.18/0.35  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.00/0.00/0.03  & 0.53/0.80/0.85  & 0.23/0.30/0.33 \\ 
 & Linf.0 & 0.00/0.02/0.07  & 0.60/0.80/0.95  & 0.25/0.33/0.33 \\ 
 & Linf.1 & 0.00/0.02/0.05  & 0.07/0.20/0.32  & 0.00/0.00/0.00 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.02  & 0.02/0.13/0.30  & 0.00/0.05/0.07 \\ 
 & pi.L1.1 & 0.00/0.00/0.05  & 0.00/0.05/0.08  & 0.05/0.05/0.10 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.05  & 0.07/0.18/0.35  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.05/0.08  & 0.05/0.05/0.10 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.02/0.05  & 0.07/0.20/0.32  & 0.00/0.00/0.00 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.03/0.12  & 0.00/0.02/0.08 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.05)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2.1 & 0.00/0.02/0.07  & 0.00/0.00/0.03  & 0.00/0.03/0.08 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.08 \\ 
 & ell.Linf.1 & 0.00/0.02/0.05  & 0.02/0.03/0.05  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.00/0.00/0.00  & 0.12/0.20/0.20  & 0.05/0.05/0.05 \\ 
 & L1.0 & 0.00/0.00/0.00  & 0.17/0.20/0.20  & 0.05/0.05/0.05 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.30/0.30/0.30  & 0.55/0.63/0.68  & 0.45/0.45/0.48 \\ 
 & L2.0 & 0.30/0.30/0.30  & 0.57/0.68/0.70  & 0.45/0.50/0.50 \\ 
 & L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.82/0.82/0.85  & 0.95/0.97/0.98  & 0.85/0.90/0.95 \\ 
 & Linf.0 & 0.82/0.90/0.95  & 0.95/0.98/1.00  & 0.90/0.92/1.00 \\ 
 & Linf.1 & 0.00/0.00/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.08 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2.1 & 0.00/0.00/0.00  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.00/0.00/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.08 \\ 
 & pi.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.1)}} & ell.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.05/0.05 \\ 
 & ell.L2.1 & 0.00/0.00/0.03  & 0.02/0.05/0.05  & 0.05/0.05/0.07 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.12/0.17/0.20  & 0.10/0.18/0.23  & 0.10/0.13/0.15 \\ 
 & ell.Linf.1 & 0.03/0.05/0.08  & 0.02/0.10/0.10  & 0.00/0.03/0.10 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.05/0.05/0.08  & 0.25/0.27/0.28  & 0.10/0.17/0.20 \\ 
 & L1.0 & 0.07/0.08/0.10  & 0.25/0.27/0.37  & 0.20/0.20/0.20 \\ 
 & L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.20/0.22/0.23  & 0.43/0.47/0.48  & 0.27/0.32/0.37 \\ 
 & L2.0 & 0.22/0.25/0.25  & 0.47/0.50/0.52  & 0.27/0.37/0.42 \\ 
 & L2.1 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.05/0.05 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.62/0.70/0.70  & 0.72/0.75/0.75  & 0.70/0.70/0.75 \\ 
 & Linf.0 & 0.63/0.70/0.72  & 0.72/0.75/0.78  & 0.70/0.70/0.75 \\ 
 & Linf.1 & 0.12/0.17/0.20  & 0.10/0.18/0.23  & 0.10/0.13/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.00/0.07  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.00/0.00/0.02  & 0.00/0.00/0.02  & 0.00/0.05/0.05 \\ 
 & pi.L2.1 & 0.00/0.00/0.03  & 0.00/0.00/0.05  & 0.00/0.00/0.00 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.12/0.17/0.20  & 0.10/0.18/0.23  & 0.10/0.13/0.15 \\ 
 & pi.Linf.1 & 0.05/0.05/0.12  & 0.05/0.10/0.13  & 0.00/0.05/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.15)}} & ell.L1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.00 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.05/0.10/0.15  & 0.10/0.13/0.20  & 0.05/0.05/0.08 \\ 
 & ell.L2.1 & 0.05/0.07/0.10  & 0.05/0.05/0.07  & 0.05/0.07/0.13 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.10/0.13/0.15  & 0.15/0.17/0.23  & 0.05/0.12/0.15 \\ 
 & ell.Linf.1 & 0.00/0.05/0.10  & 0.00/0.00/0.10  & 0.00/0.02/0.05 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.20/0.20/0.22  & 0.30/0.40/0.40  & 0.25/0.27/0.30 \\ 
 & L1.0 & 0.20/0.20/0.20  & 0.37/0.40/0.40  & 0.27/0.32/0.35 \\ 
 & L1.1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.00 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.30/0.30/0.33  & 0.45/0.52/0.57  & 0.35/0.38/0.40 \\ 
 & L2.0 & 0.30/0.32/0.35  & 0.55/0.55/0.55  & 0.40/0.40/0.40 \\ 
 & L2.1 & 0.05/0.10/0.15  & 0.10/0.13/0.20  & 0.05/0.05/0.08 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.40/0.48/0.55  & 0.57/0.65/0.68  & 0.42/0.48/0.53 \\ 
 & Linf.0 & 0.35/0.50/0.55  & 0.53/0.65/0.75  & 0.42/0.52/0.58 \\ 
 & Linf.1 & 0.10/0.13/0.15  & 0.15/0.17/0.23  & 0.05/0.12/0.15 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.00/0.02/0.02  & 0.00/0.00/0.03  & 0.00/0.00/0.00 \\ 
 & pi.L1.1 & 0.00/0.00/0.03  & 0.00/0.02/0.05  & 0.00/0.02/0.05 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.05/0.10/0.15  & 0.10/0.13/0.20  & 0.05/0.05/0.08 \\ 
 & pi.L2.1 & 0.00/0.00/0.05  & 0.00/0.05/0.07  & 0.00/0.00/0.03 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.10/0.13/0.15  & 0.15/0.17/0.23  & 0.05/0.12/0.15 \\ 
 & pi.Linf.1 & 0.10/0.12/0.15  & 0.05/0.17/0.22  & 0.12/0.15/0.20 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.2)}} & ell.L1 & 0.05/0.08/0.15  & 0.17/0.20/0.23  & 0.05/0.10/0.15 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.15/0.15/0.20  & 0.15/0.23/0.33  & 0.15/0.15/0.20 \\ 
 & ell.L2.1 & 0.05/0.07/0.08  & 0.02/0.05/0.05  & 0.00/0.03/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.15/0.22/0.22  & 0.15/0.25/0.25  & 0.15/0.25/0.25 \\ 
 & ell.Linf.1 & 0.02/0.05/0.07  & 0.00/0.05/0.08  & 0.00/0.00/0.07 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.25/0.32/0.33  & 0.60/0.65/0.72  & 0.40/0.50/0.50 \\ 
 & L1.0 & 0.32/0.33/0.38  & 0.65/0.70/0.75  & 0.45/0.50/0.52 \\ 
 & L1.1 & 0.05/0.08/0.15  & 0.17/0.20/0.23  & 0.05/0.10/0.15 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.40/0.40/0.40  & 0.65/0.73/0.75  & 0.45/0.52/0.55 \\ 
 & L2.0 & 0.40/0.40/0.43  & 0.75/0.75/0.75  & 0.50/0.55/0.55 \\ 
 & L2.1 & 0.15/0.15/0.20  & 0.15/0.23/0.33  & 0.15/0.15/0.20 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.27/0.33/0.42  & 0.52/0.57/0.63  & 0.32/0.43/0.50 \\ 
 & Linf.0 & 0.27/0.38/0.53  & 0.47/0.52/0.67  & 0.30/0.43/0.48 \\ 
 & Linf.1 & 0.15/0.22/0.22  & 0.15/0.25/0.25  & 0.15/0.25/0.25 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.05/0.08/0.15  & 0.17/0.20/0.23  & 0.05/0.10/0.15 \\ 
 & pi.L1.1 & 0.02/0.05/0.07  & 0.00/0.05/0.07  & 0.05/0.05/0.08 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.15/0.15/0.20  & 0.15/0.23/0.33  & 0.15/0.15/0.20 \\ 
 & pi.L2.1 & 0.02/0.05/0.05  & 0.00/0.05/0.07  & 0.00/0.03/0.07 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.15/0.22/0.22  & 0.15/0.25/0.25  & 0.15/0.25/0.25 \\ 
 & pi.Linf.1 & 0.00/0.03/0.10  & 0.02/0.08/0.10  & 0.00/0.08/0.13 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
\hline
\multirow{30}{*}{\texttt{power.thomas(0.25)}} & ell.L1 & 0.10/0.10/0.12  & 0.10/0.15/0.18  & 0.05/0.07/0.12 \\ 
 & ell.L1.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.L2 & 0.10/0.15/0.15  & 0.05/0.12/0.15  & 0.08/0.10/0.10 \\ 
 & ell.L2.1 & 0.00/0.03/0.05  & 0.00/0.05/0.05  & 0.00/0.05/0.05 \\ 
 & ell.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf & 0.05/0.05/0.05  & 0.05/0.07/0.10  & 0.05/0.05/0.05 \\ 
 & ell.Linf.1 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & ell.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L1 & 0.32/0.37/0.45  & 0.50/0.55/0.55  & 0.30/0.37/0.40 \\ 
 & L1.0 & 0.35/0.45/0.45  & 0.55/0.55/0.55  & 0.35/0.38/0.40 \\ 
 & L1.1 & 0.10/0.10/0.12  & 0.10/0.15/0.18  & 0.05/0.07/0.12 \\ 
 & L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & L2 & 0.35/0.35/0.42  & 0.50/0.50/0.52  & 0.30/0.42/0.45 \\ 
 & L2.0 & 0.35/0.47/0.50  & 0.50/0.52/0.55  & 0.40/0.45/0.45 \\ 
 & L2.1 & 0.10/0.15/0.15  & 0.05/0.12/0.15  & 0.08/0.10/0.10 \\ 
 & L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & Linf & 0.10/0.17/0.38  & 0.32/0.50/0.58  & 0.17/0.25/0.33 \\ 
 & Linf.0 & 0.05/0.28/0.50  & 0.33/0.55/0.60  & 0.22/0.25/0.40 \\ 
 & Linf.1 & 0.05/0.05/0.05  & 0.05/0.07/0.10  & 0.05/0.05/0.05 \\ 
 & Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1 & 0.10/0.10/0.12  & 0.10/0.15/0.18  & 0.05/0.07/0.12 \\ 
 & pi.L1.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L1.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.L2 & 0.10/0.15/0.15  & 0.05/0.12/0.15  & 0.08/0.10/0.10 \\ 
 & pi.L2.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.00/0.02 \\ 
 & pi.L2.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf & 0.05/0.05/0.05  & 0.05/0.07/0.10  & 0.05/0.05/0.05 \\ 
 & pi.Linf.1 & 0.00/0.00/0.02  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 
 & pi.Linf.2 & 0.00/0.00/0.00  & 0.00/0.00/0.00  & 0.00/0.00/0.00 \\ 


==> reject-rates-power-models-estimator-noise.tex <==
\multirow{9}{*}{axis} & \multirow{3}{*}{L1} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{L2} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{Linf} & 0.01 & 0.57/0.97/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7}\midrule
\multirow{9}{*}{unbiased.hull} & \multirow{3}{*}{L1} & 0.01 & 1.00/1.00/1.00  & 0.55/0.98/1.00  & 1.00/1.00/1.00  & 0.00/0.00/0.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{L2} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7} & \multirow{3}{*}{Linf} & 0.01 & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00  & 1.00/1.00/1.00 \\ 
 \cmidrule(lr){2-7}

==> reject-rates-power-models-size.tex <==
\texttt{L1.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 0.57/0.97/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L1.1} & 1.00/1.00/1.00 & 0.55/0.98/1.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L1.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{L1.1} & 0.00/0.00/0.00 & 0.00/0.00/0.00 \\ 
\texttt{L2.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 
\texttt{Linf.1} & 1.00/1.00/1.00 & 1.00/1.00/1.00 \\ 

